Feature Generation by Convolutional Neural Network for Click-Through Rate Prediction

Click-Through Rate prediction is an important task in recommender systems, which aims to estimate the probability of a user to click on a given item. Recently, many deep models have been proposed to learn low-order and high-order feature interactions from original features. However, since useful interactions are always sparse, it is difficult for DNN to learn them effectively under a large number of parameters. In real scenarios, artificial features are able to improve the performance of deep models (such as Wide & Deep Learning), but feature engineering is expensive and requires domain knowledge, making it impractical in different scenarios. Therefore, it is necessary to augment feature space automatically. In this paper, We propose a novel Feature Generation by Convolutional Neural Network (FGCNN) model with two components: Feature Generation and Deep Classifier. Feature Generation leverages the strength of CNN to generate local patterns and recombine them to generate new features. Deep Classifier adopts the structure of IPNN to learn interactions from the augmented feature space. Experimental results on three large-scale datasets show that FGCNN significantly outperforms nine state-of-the-art models. Moreover, when applying some state-of-the-art models as Deep Classifier, better performance is always achieved, showing the great compatibility of our FGCNN model. This work explores a novel direction for CTR predictions: it is quite useful to reduce the learning difficulties of DNN by automatically identifying important features.

==> experiments.tex <==
\section{Experiments}
In this section, we conduct extensive experiments to answer the following questions:
\begin{itemize}
       \item \textbf{(Q1)} Is it true that identifying important features first by CNN can boost the performance of DNN models?
       \item \textbf{(Q2)} How does each component in FGCNN affect the final performance?
       \item \textbf{(Q3)} How does the key parameters of  FGCNN impact its performance?
\end{itemize}
\subsection{Experiment Setup}
\subsubsection{Datasets} we conduct extensive experiments in the following three datasets:

\textit{Criteo}: Criteo\footnote{http://labs.criteo.com/downloads/download-terabyte-click-logs/} contains one month of click logs with billions of data samples. A small subset of Criteo was published in Criteo Display Advertising Challenge, 2013 and FFM was the winning solution~\cite{pin, ffm}. 'Day 6-12' is selected for training while 'day 13' is selected for evaluation. Due to the enormous data volume and serious imbalance(only 3\% samples is positive), negative sampling is applied to keep the imbalance ratio close to 1:1. We convert 13 numerical fields into one-hot features through bucketing. And the features in a certain field appearing less than 20 times are set as a dummy feature "other".

\textit{Avazu}: Avazu\footnote{http://www.kaggle.com/c/avazu-ctr-prediction} was published in the contest of Avazu Click-Through Rate Prediction, 2014. The publich dataset is randomly splitted into training and test sets at 4:1. Meanwhile, we remove the features appearing less than 20 times to reduce dimensionality.

\textit{Company}: In order to verify the performance of FGCNN in real  industrial CTR prediction, we conduct experiment on Company* Dataset. we collect  users' click logs record from the game center of Company* App Store while logs from 20180617 to 20180623 is used for training and logs in 20180624 is used for testing. The datasets contains app, user and context features. 

\begin{table}[]
\caption{Dataset statistics}
\label{dataset}
\begin{tabular}{l|llll}
Dataset & \#instances & \#features & \#fields & pos ratio \\ \hline
Criteo & 1$\times$10\textasciicircum{}8 & 1$\times$10\textasciicircum{}6 & 39 & 0.5 \\
Avazu & 4$\times$10\textasciicircum{}7 & 6$\times$10\textasciicircum{}5 & 24 & 0.17 \\
Company & 2.3$\times$10\textasciicircum{}8 & 1.6$\times$10\textasciicircum{}5 & 29 & 0.05
\end{tabular}
\end{table}

Table \ref{dataset} summarizes the statistics of 4 datasets.
\subsubsection{Baselines} 
Eight baseline models is selected for comparison, including LR~\cite{lr}, GBDT~\cite{gbdt}, FM~\cite{fm}, FFM~\cite{ffm}, CCPM~\cite{ccpm}, DeepFM~\cite{deepfm}, xDeepFM~\cite{xdeepfm}, IPNN~\cite{pin} and PIN~\cite{pin}. And since Wide\&Deep model needs feature engineering, it is not compared here. We use XGBoost~\cite{gbdt} and libFFM\footnote{https://github.com/guestwalk/libffm} as GBDT and libFFM in our experiments. Other models are implemented with Tensorflow.
\subsubsection{Evaluation Metrics} The evaluation metics are \textbf{AUC} and \textbf{log loss}.
\subsubsection{Parameter Settings}

\begin{table}[]
\caption{Parameter Settings Pooling not added}
\label{parameter}
\scriptsize
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
 & Criteo & Avazu & Company \\ \hline
General & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=1000\\ opt=Adam\\ lr=1e-4\\ l2=1e-6\end{tabular} \\ \hline
LR & - & - & - \\ \hline
GBDT & \begin{tabular}[c]{@{}l@{}}depth=25\\ \#tree=1300\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=18\\ \#tree=1000\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=10\\ \#tree=1400\end{tabular} \\ \hline
FM & k=20 & k=40 & k=40 \\ \hline
FFM & k=4 & k=4 & k=12 \\ \hline
CCPM & \begin{tabular}[c]{@{}l@{}}k=20\\     conv= 7*1\\    kernel={[}256{]}\\     net={[}256*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv: 7*1\\     kernel = {[}128{]}\\     net= {[}128*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv= 2*1\\     kernel= {[}8,16,32,64{]}\\     net={[}512,256,128,1{]}\\     drop= 0.8\end{tabular} \\ \hline
DeepFM & \begin{tabular}[c]{@{}l@{}}k=20, LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\end{tabular} \\ \hline
XdeepFM & \begin{tabular}[c]{@{}l@{}}k=20\\     net={[}400*3,1{]}\\     CIN={[}100*4{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}700*5,1{]}\\     CIN:{[}100*2{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\\     CIN:{[}100{]}\end{tabular} \\ \hline
IPNN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     \end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\    \end{tabular} \\ \hline
PIN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\\     subnet={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     sub-net={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\     sub-net={[}40,10{]}\end{tabular} \\ \hline
FGCNN & \begin{tabular}[c]{@{}l@{}}k=20\\     conv=9*1\\  pool=2*1\\     kernel={[}38,40,42,44{]}\\     new={[}3,3,3,3{]}\\     BN=True\\     net={[}4096,2048,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=7*1\\ pool=2*1\\    kernel={[}6,8,10,14{]}\\     new={[}3,3,3,3{]}\\     BN=T\\     net={[}4096,2048,1024,\\ 512,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=13*1\\  pool=2*1 \\   kernel={[}6-8-10-12{]}\\     new={[}2,2,2,2{]}\\     BN=T\\     net={[}2048,1024,\\ 512,256,128,1{]}\\     drop=0.8\end{tabular} \\ \hline
\end{tabular}
}
Notice: bs=Batch Size, opt=Optimizer, lr=Learning Rate, l2=L2 Regularization on Embedding Layer, k = Embedding size, conv= Convolution Kernel shape, kernel = Convolution kernels(Feature map),pool=max-pooling shape, net= DNN Structure, sub-net = Micro Network, drop = dropout rate, LN= Layer Normalization, BN= batch normalization, new = new feature map num for each feature generation.
\end{table}
Table~\ref{parameter} summerizes the hyperparameters for each model.
For \textit{Criteo} and \textit{Avazu} Datasets, the same hyperparameters as ~\cite{pin} is used to reproduce their results. In the FGCNN model, to simplify the parameter of the number of generated feature, we introduce parameter \textit{new} which works as the kernel in the convolution layer. The number of generated features can be calculated as $\sum_{i=1}^l \#fields/2^i*new_i$.

\begin{table*}[t]
\caption{Overall Performances\\
$\star: p<0.0001$}
\label{overall}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lllllll}
        & \multicolumn{2}{c}{Criteo}                                    & \multicolumn{2}{c}{Avazu}                                              & \multicolumn{2}{c}{Company}                        \\ \hline
Model   & AUC                 & \multicolumn{1}{l|}{Log Loss}           & AUC(\%)                  & \multicolumn{1}{l|}{Log Loss}               & AUC                      & Log Loss                \\ \hline
LR      & 78.00\%             & \multicolumn{1}{l|}{0.5631}             & 76.76\%                  & \multicolumn{1}{l|}{0.3868}                 & 90.12\%                  & 0.1371                  \\
GBDT    & 78.62\%             & \multicolumn{1}{l|}{0.5560}             & 77.53\%                  & \multicolumn{1}{l|}{0.3824}                 & 92.68\%                  & 0.1227                  \\
FM      & 79.09\%             & \multicolumn{1}{l|}{0.5500}             & 77.93\%                  & \multicolumn{1}{l|}{0.3805}                 & 93.26\%                  & 0.1191                  \\
FFM     & 79.80\%             & \multicolumn{1}{l|}{0.5438}             & 78.31\%                  & \multicolumn{1}{l|}{0.3781}                 & 93.58\%                  & 0.1170                  \\
CCPM    & 79.55\%             & \multicolumn{1}{l|}{0.5469}             & 78.12\%                  & \multicolumn{1}{l|}{0.3800}                 & 93.68\%                  & 0.1162                  \\
DeepFM  & 79.91\%             & \multicolumn{1}{l|}{0.5423}             & 78.30\%                  & \multicolumn{1}{l|}{0.3778}                 & 93.84\%                  & 0.1149                  \\
xDeepfm & 80.06\%             & \multicolumn{1}{l|}{0.5408}             & 78.55\%                  & \multicolumn{1}{l|}{0.3766}                 & 93.82\%                  & 0.1152                  \\
IPNN    & 80.13\%             & \multicolumn{1}{l|}{0.5399}             & 78.68\%                  & \multicolumn{1}{l|}{0.3757}                 & 93.87\%                  & 0.1148                  \\
PIN     & \underline{80.21\%} & \multicolumn{1}{l|}{\underline{0.5390}} & \underline{78.72\%}      & \multicolumn{1}{l|}{\underline{0.3755}}     & \underline{93.89\%}      & \underline{0.1146}      \\ \hline
FGCNN   & \textbf{80.22\%}    & \multicolumn{1}{l|}{\textbf{0.5388}}    & $\mathbf{78.83\%^\star}$ & \multicolumn{1}{l|}{$\mathbf{0.3746^\star}$} & $\mathbf{94.05\%^\star}$ & $\mathbf{0.1135^\star}$
\end{tabular}
}

\end{table*}
\subsubsection{Significance Test} To show whether the improvements is significant, we repeat the experiments for 5 times on FGCNN and the best baseline model. Then, two-tailed pairwise t-test is performed to detect significant differences between FGCNN and the best baseline model.
\begin{table*}[t]
\caption{Performances after removing the component in FGCNN}
\label{remove}
\begin{tabular}{l|ll|ll|ll}
       & \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c}{Company} \\ \hline
Method & AUC          & Log Loss     & Auc         & Log Loss     & Auc          & Log Loss     \\ \hline
FGCNN  & \textbf{80.22\%}      & \textbf{0.5388}      & \textbf{78.83\%}     & \textbf{0.3746}       & \textbf{94.05\%}      & \textbf{0.1135}       \\
Without Raw Features   & 80.21\%      & 0.5390       & 78.66\%     & 0.3757        & 93.98\%      &0.1141       \\
Without New Features   & 80.13\%      & 0.5399       & 78.68\%     & 0.3757       & 93.87\%      & 0.1148       \\
Replacing Convolution by MLP   & 80.12\%      & 0.5402       & 78.58\%     & 0.3761       & 94.04\%             &0.1135              \\
Removing Recombination Layer    & 80.11\%      & 0.5403       & 78.74\%     & 0.3753       & 94.04\%             & 0.1135             \\
Removing Factorization Machine    & 80.09\%      & 0.5402       & 78.55\%     & 0.3764       &  94.00\%            &   0.1139           \\
Using One Embedding Matrix   & 80.17\%      & 0.5394       & 78.68\%     & 0.3755       &     94.04\%        &  0.1136           
\end{tabular}
\end{table*}

\subsection{Overall Performance(Q1)}
Table ~\ref{overall} shows the overall performances, where underline numbers are the best results of baseline models and bold numbers are the best results of all. There are several oberservations:

Firstly, among all basline models, PIN is the best baseline model in three datasets. while xDeepFM(the third best model) tries to learn explicit and implicit low and high order feature interactions, PIN uses a micro network to learn pairwised feature interaction which demonstrates the effectiveness of order-2 cross features. In all baseline models, LR achives worst performance in the three datasets, which demonstrates that factorization-based models are essential for modeling sparse feature in the CTR prediction task. Moreover, CCPM is the worst deep learning model, which shows that it is unsatisfactory to directly using traditional Convolutional Neural Network to make predictions for click-through rate predictions. The main reason is that the arrangement of features in the CTR prediction does not have the different meaning like images and sentences, which makes traditional CNN model difficult to find useful neighboring information on a random feature arrangement. 

Secondly, FGCNN achieves the best performance on all datasets. In Company dataset, our prposed FGCNN model beats competitors by more than 0.16\% in AUC and 0.11\% in log loss. In fact, a small improvement in offline AUC evaluation is likely lead to a significant increase in online CTR.
As shown in ~\cite{cheng2016wide}, 0.275\% improvements in AUC lead to 3.8\% improvement in online CTR. The daily turnover of Company's APP store is millions of dollars, therefore even several percents increase in CTR can bring extra millions of dollars a year.
Recall that we only use inner product to learn explict feature interactions between generated features and old features, which is quite simple than PIN(using Micro Network for each feature pair). It can demonstrate that our FGCNN model do extract important cross features and the generated features do reduce the optimization difficulties of DNNs thus yielding better performances. Despite the significant improvements on \textit{Avazu} and \textit{Company} datasets, the FGCNN model can not achieve significant improvements than PIN on \textit{Criteo} Dataset. The possible reason is that pairwised feature interactions play an important role on the final performance and Micro-Network learns the interactions better than Inner Product. 

\subsection{Component Importances(Q2)}

To investigate how each component contributes to the actual performances, we conduct several experiments by removing some component on our FGCNN model:
\begin{itemize}
\item \textbf{Without Raw Features}: raw features are disregarded in the second part of FGCNN. Only generated features is fed to FM and Deep component.
 \item \textbf{Without New Features}: the feature generation process is removed in FGCNN. Only the raw features is fed to FM and Deep component.
 \item \textbf{Replacing Convolution by MLP}: Convolution layer is replaced by multi-layer  of full connections, hidden neurons in such layer is used as new features. The distribution of generated new features in MLP is exactly same as it in the Recombination Layer.
 \item \textbf{Removing Recombination Layer}: removes the recombination layer in FGCNN and uses the results of pooling layer as new features.
 \item \textbf{Removing Factorization Machine}: removes the factorization machine Layer in the model.
 \item \textbf{Using One Embedding Matrix}: use the same embedding matrix for feature generation and DNN.
\end{itemize}


%\textcolor{red}{adding the Replacing Convolution by Full Connection model picture}

Table ~\ref{remove} summerizes the performances after removing the components in FGCNN. As it shows, removing any components in FGCNN can lead to a drop in the performance.

Firstly, Only using raw features or new features rarely results in an optimal model, which demonstrate that the generated features are a good supplementary for the original feature space. Secondly, the decrease of performance after \textit{Replacing Convolution with MLP} shows it is difficult for Multi-Layer Perceptrons to identify important feature combinations in the large combinational space while CNN+Pooling+Recombination simplifies the its difficulties. 
Thirdly, if we remove the recombination layer, FGCNN is restricted by the feature interactions of neighbor features. Since the arragement order has no actual meaning in CTR prediction and it is usually quite randomized, it is necessary to recombine the neighboring information to generate global feature interactions.
Fourthly, \textit{Removing Factorization Machine} has the greatest impact on the performance, which shows the usefullness of Factorization Machine to capture explicit low-order feature interactions.
Finally, if we only use the same embedding matrix for both feature generation part and Deep Predictive Learning part, the direction gradients from feature generation part and  DNN part may contradict which hinders the learning of FGCNN model. Therefore, using double embedding matrixs can be a good choice.


%Finally, the results of \textit{Replacing the convolution by Full Connection}
 %shows that although DNN can approximate any functions ideally, due to the large parameter space, it is usually hard to optimize. Therefore, the performance of \textit{Replacing the convolution by Full Connection} is relatively poor.  And it is even worse than \textit{Without New Features}, which shows new features generated by Full Connection are actually data noises.  We also have further experiments in the next section to show how the height of convolution kernel impacts(the bigger in height, the closer to Full Connection) the final performances, and it also demonstrates bigger heights often result in worse performances.
\subsection{Compatibility with Other Models}
In the FGCNN model,  the generated features in the first layers can be viewed as an augmentation of original features. Therefore, many models can be used in our second component. FM, DeepFM, IPNN is compared in Table~\ref{integrete} to show FGCNN's Compatibilities. 
\begin{table*}[]
\caption{Integreting FGCNN with other models}
\label{tab:integrete}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
             & \multicolumn{2}{c|}{Criteo}                              & \multicolumn{2}{c|}{Avazu}                               & \multicolumn{2}{c|}{Company}                             \\ \hline
             & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} \\ \hline
IPNN         & 80.13\%                  & 0.5399                        & 78.68\%                  & 0.3757                        & 93.87\%                  & 0.1148                        \\
FGCNN+IPNN   & 80.22\%                  & 0.5388                        & 78.83\%                  & 0.3746                        & 94.05\%                  & 0.1135                        \\ \hline
FM           & 79.09\%                  & 0.5500                        & 77.93\%                  & 0.3805                        & 93.26\%                  & 0.1191                        \\
FGCNN+FM     &  79.67\%                        &  0.5455                             & 78.13\%                  & 0.3794                        & 93.66\%                         &  0.1165                             \\ \hline
DeepFM       & 79.91\%                  & 0.5423                        & 78.36\%                  & 0.3777                        & 93.84\%                  & 0.1149                        \\
FGCNN+DeepFM &                          &                               &                          &                               &   93.93\%                 &  0.1145                         \\ \hline
DNN       & 79.87\%                  & 0.5428                        & 78.30\%                  & 0.3778                        &  \%                  &                         \\
FGCNN+DNN &       80.09\%             &0.5402                               &   78.55\%                       &  0.3764                             &       94.00\%                   &        0.1139                      \\ \hline
\end{tabular}
}
\end{table*}
 \subsection{Parameter Analysis}
 We analyse some key parameters in FGCNN, to show how the parameters affect the performance of FGCNN.
 \subsubsection{Convolution Height}
 The first parameter is convolution height, which controls the percetion range of convolution layer. We try to increase the height from 2 to the number of features in each datasets. As shown in Figure ~\ref{height}, AUC often increases as the initial height increases.  After a critical point, AUC starts to decreases as the height continue increasing. The main reason is that the optimization difficuties is much higher when using bigger convolution heights, which is also the reason why full connections layers can not work well in identifying important patterns.
 \subsubsection{Convolution Layers}
 Experiments on different convolution layers show that as more convolution layers are used, performance is always better, which shows high-order feature interactions are very useful. \textcolor{red}{higher convolution layers}
 \subsubsection{Convolution Kernels}
 Convolution kernels is the second studied parameters. As Figure~\ref{layers} shows, AUC seems to increase with the increase of the number of used kernels in Criteo while AUC has a unstable correlations with the number of kernels. The possible reason is that the number of fields in criteo(39) is much more than it in Avazu(24). Therefore, the combination space in Criteo is much bigger than Avazu. So, more kernels are needed to generate important features. 
 \subsubsection{Number of Generated Features}
 We also studied how the number of new feature map after each pooling layer affect the performance. As Figure~\ref{new} shows, with the inrease of new feature map num, AUC in criteo is improved, and in Avazu the biggest new feature map num lead to the best AUC. it demonstrates that the generated new features have a great impact on final performance.
 
 \subsection{Will the arrangement order of raw features affect FGCNN?}
 Since CNN  will be affected by the arrangement of features, we wonder that if the order of features affects the performance of FGCNN. To study it, we shuffled the order of features before feeding it into \textit{feature generation} part. Recall that the major difference between \textit{feature generation} and traditional CNN structure is that \textit{feature generation} has a recombination layer which is designed to combine the neighboring interactions from CNN and generate global feature interactions. The recombination layer has the potential to break the limitation of CNN to learn effective combinations in any given inpute orders. To verify it, we compare models in two settings: without Recombination and with Recombination. The experiments are repeated in ten times and same model settings are applied here.  Figure ~\ref{shuffle} and Table~\ref{tab:shuffle} summerize such experiments. 
 
 As shown in Table ~\ref{tab:shuffle}, the setting with recombination achieve more stable(low standard deviation) and better performance(high average AUC) than it without recombination Layer. It demonstrates that FGCNN is more robust than traditional CNN. Due to that our best model in the original setting can be also viewed as a random arrangement of features, it is highly likely to achieve better performance based on better parameter settings in any randomized arragements.
 
 
 \begin{table}[]
\caption{AUCs after shuffling features' arrangement order}
\label{tab:shuffle}
\begin{tabular}{|l|l|l|l|l|}
\hline
        & \multicolumn{2}{l|}{Without Recombination} & \multicolumn{2}{l|}{With Recombination} \\ \hline
        & average              & std                 & average             & std               \\ \hline
Criteo  & 80.08\%              & 0.01\%              & \textbf{80.20\% }            & \textbf{0.01\%  }          \\ \hline
Avazu   & 78.75\%              & 0.05\%              & \textbf{78.76\% }            &\textbf{0.03\% }           \\ \hline
Company & 94.01\%              & 0.01\%              & \textbf{94.02\%}             & \textbf{0.01\% }           \\ \hline
\end{tabular}
\end{table}
 \begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{height.jpg}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Convolutional Height}
 \label{height}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{layers.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Convolutional Layers}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{kernel.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Convolutional Kernel}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{new.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{New feature map nums}
 \label{new}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{shuffle.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Shuffling the feature order}
 \label{shuffle}
\end{figure*}




==> experiments_1025_ruiming.tex <==
\section{Experiments}

In this section, we conduct extensive experiments to answer the following questions. 
\begin{itemize}
       \item \textbf{(Q1)} How does FCGNN perform, compared to the state-of-the-art models for CTR prediction task?
       \item \textbf{(Q2)} How does each key structure in FGCNN boost the prediction performance?
       \item \textbf{(Q3)} How is the compatibility of FGCNN, i.e., applying different network structures as its \emph{deep predictive learning} part.
       \item \textbf{(Q4)} How do the key hyper-parameters of FGCNN (i.e., size and number of convolution kernels, number of generated features) impact its performance?
       \item \textbf{(Q5)} How does the \emph{feature generation} part perform when the order of raw features are random shuffled.
\end{itemize}

Note that when studying questions other than \textbf{Q3}, we adpot IPNN as the \emph{deep predictive learning} of FGCNN.

\subsection{Experimental Setup}

\subsubsection{Datasets} we conduct the experiment with the following three datasets:

\textit{Criteo}: Criteo\footnote{http://labs.criteo.com/downloads/download-terabyte-click-logs/} contains one month of click logs with billions of data samples. A small subset of Criteo was published in Criteo Display Advertising Challenge, 2013 and FFM was the winning solution~\cite{pin, ffm}. We select ``day 6-12'' as training set while select ``day 13'' for evaluation. Due to the enormous data volume and serious class imbalance (i.e., only 3\% samples are positive), negative sampling is applied to keep the positive and negative ratio close to 1:1. We convert 13 numerical fields into one-hot features through bucketing, where the features in a certain field appearing less than 20 times are set as a dummy feature ``other".

\textit{Avazu}: Avazu\footnote{http://www.kaggle.com/c/avazu-ctr-prediction} was published in the contest of Avazu Click-Through Rate Prediction, 2014. The publich dataset is randomly splitted into training and test sets at 4:1. Meanwhile, we remove the features appearing less than 20 times to reduce dimensionality.

\textit{Company}: In order to verify the performance of FGCNN in real industrial CTR prediction, we conduct experiment on Company Dataset. We collect users' click logs from Company App Store while logs from 20180617 to 20180623 is used for training and logs of 20180624 is used for test. Negative sampling is applied to reduce data amount and to balance the positive and negative ratio. The datasets contains app features (e.g., identification, category, etc), user features (e.g., user's behavior history, etc) and context features (e.g., operation time, etc). 

\begin{table}[]
\caption{Dataset statistics}
\label{table:dataset}
\begin{tabular}{l|llll}
Dataset & \#instances & \#features & \#fields & pos ratio \\ \hline
Criteo & $1\times 10^{8}$ & $1\times 10^{6}$ & 39 & 0.5 \\
Avazu & $4\times 10^{7}$ & $6\times 10^{5}$ & 24 & 0.17 \\
Company & $2.3\times 10^{8}$ & $1.6\times 10^{5}$ & 29 & 0.05
\end{tabular}
\end{table}

Table~\ref{table:dataset} summarizes the statistics of the three datasets.

\subsubsection{Baselines} 

We compare eight baseline models in our experiment, including LR~\cite{lr}, GBDT~\cite{gbdt}, FM~\cite{fm}, FFM~\cite{ffm}, CCPM~\cite{ccpm}, DeepFM~\cite{deepfm}, xDeepFM~\cite{xdeepfm}, IPNN and PIN~\cite{pin}. We use XGBoost~\cite{gbdt} and libFFM\footnote{https://github.com/guestwalk/libffm} as the implementation of GBDT and libFFM in our experiments, and the other baseline models are implemented with Tensorflow\footnote{https://www.tensorflow.org/}.

\subsubsection{Evaluation Metrics} The evaluation metics are \textbf{AUC} (Area Under ROC) and \textbf{log loss} (cross entropy).

\subsubsection{Parameter Settings}

\begin{table}[]
\caption{Parameter Settings}
\label{table:parameter}
\scriptsize
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
 & Criteo & Avazu & Company \\ \hline
General & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=1000\\ opt=Adam\\ lr=1e-4\\ l2=1e-6\end{tabular} \\ \hline
LR & - & - & - \\ \hline
GBDT & \begin{tabular}[c]{@{}l@{}}depth=25\\ \#tree=1300\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=18\\ \#tree=1000\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=10\\ \#tree=1400\end{tabular} \\ \hline
FM & k=20 & k=40 & k=40 \\ \hline
FFM & k=4 & k=4 & k=12 \\ \hline
CCPM & \begin{tabular}[c]{@{}l@{}}k=20\\     conv= 7*1\\    kernel={[}256{]}\\     net={[}256*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv: 7*1\\     kernel = {[}128{]}\\     net= {[}128*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv= 2*1\\     kernel= {[}8,16,32,64{]}\\     net={[}512,256,128,1{]}\\     drop= 0.8\end{tabular} \\ \hline
DeepFM & \begin{tabular}[c]{@{}l@{}}k=20, LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\end{tabular} \\ \hline
XdeepFM & \begin{tabular}[c]{@{}l@{}}k=20\\     net={[}400*3,1{]}\\     CIN={[}100*4{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}700*5,1{]}\\     CIN:{[}100*2{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\\     CIN:{[}100{]}\end{tabular} \\ \hline
IPNN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     \end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\    \end{tabular} \\ \hline
PIN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\\     subnet={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     sub-net={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\     sub-net={[}40,10{]}\end{tabular} \\ \hline
FGCNN & \begin{tabular}[c]{@{}l@{}}k=20\\     conv=9*1\\  pool=2*1\\     kernel={[}38,40,42,44{]}\\     new={[}3,3,3,3{]}\\     BN=T\\     net={[}4096,2048,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=7*1\\ pool=2*1\\    kernel={[}6,8,10,14{]}\\     new={[}3,3,3,3{]}\\     BN=T\\     net={[}4096,2048,1024,\\ 512,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=13*1\\  pool=2*1 \\   kernel={[}6,8,10,12{]}\\     new={[}2,2,2,2{]}\\     BN=T\\     net={[}2048,1024,\\ 512,256,128,1{]}\\     drop=0.8\end{tabular} \\ \hline
\end{tabular}
}
Note: bs=Batch Size, opt=Optimizer, lr=Learning Rate, l2=L2 Regularization on Embedding Layer, k=Embedding Size, conv=Convolution Kernel shape, kernel=number of Convolution Kernels, pool=Max-Pooling Shape, net=MLP Structure, sub-net=Micro Network, drop=Keep Rate(drop=1.0 if not stated), LN=Layer Normalization, BN= Batch Normalization\{T=True\}, new=number of Kernels Generating New Features.
\end{table}

Table~\ref{table:parameter} summerizes the hyperparameters of each model.
For \textit{Criteo} and \textit{Avazu} Datasets, the hyperparameters of baseline models are set the same as in~\cite{pin}, in order to reproduce their results. In the FGCNN model, \textit{new} is the number of kernels when generating new features. The number of generated features can be calculated as $\sum_{i=1}^l \#fields/2^i*new_i$.

\begin{table*}[t]
\caption{Overall Performances\\
$\star: p < 10^{-4}$ (two-tailed t-test)}
\label{table:overall}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lllllll}
        & \multicolumn{2}{c}{Criteo}                                    & \multicolumn{2}{c}{Avazu}                                              & \multicolumn{2}{c}{Company}                        \\ \hline
Model   & AUC                 & \multicolumn{1}{l|}{Log Loss}           & AUC(\%)                  & \multicolumn{1}{l|}{Log Loss}               & AUC                      & Log Loss                \\ \hline
LR      & 78.00\%             & \multicolumn{1}{l|}{0.5631}             & 76.76\%                  & \multicolumn{1}{l|}{0.3868}                 & 90.12\%                  & 0.1371                  \\
GBDT    & 78.62\%             & \multicolumn{1}{l|}{0.5560}             & 77.53\%                  & \multicolumn{1}{l|}{0.3824}                 & 92.68\%                  & 0.1227                  \\
FM      & 79.09\%             & \multicolumn{1}{l|}{0.5500}             & 77.93\%                  & \multicolumn{1}{l|}{0.3805}                 & 93.26\%                  & 0.1191                  \\
FFM     & 79.80\%             & \multicolumn{1}{l|}{0.5438}             & 78.31\%                  & \multicolumn{1}{l|}{0.3781}                 & 93.58\%                  & 0.1170                  \\
CCPM    & 79.55\%             & \multicolumn{1}{l|}{0.5469}             & 78.12\%                  & \multicolumn{1}{l|}{0.3800}                 & 93.68\%                  & 0.1162                  \\
DeepFM  & 79.91\%             & \multicolumn{1}{l|}{0.5423}             & 78.30\%                  & \multicolumn{1}{l|}{0.3778}                 & 93.84\%                  & 0.1149                  \\
xDeepfm & 80.06\%             & \multicolumn{1}{l|}{0.5408}             & 78.55\%                  & \multicolumn{1}{l|}{0.3766}                 & 93.82\%                  & 0.1152                  \\
IPNN    & 80.13\%             & \multicolumn{1}{l|}{0.5399}             & 78.68\%                  & \multicolumn{1}{l|}{0.3757}                 & 93.87\%                  & 0.1148                  \\
PIN     & \underline{80.21\%} & \multicolumn{1}{l|}{\underline{0.5390}} & \underline{78.72\%}      & \multicolumn{1}{l|}{\underline{0.3755}}     & \underline{93.89\%}      & \underline{0.1146}      \\ \hline
FGCNN   & \textbf{80.22\%}    & \multicolumn{1}{l|}{\textbf{0.5388}}    & $\mathbf{78.83\%^\star}$ & \multicolumn{1}{l|}{$\mathbf{0.3746^\star}$} & $\mathbf{94.05\%^\star}$ & $\mathbf{0.1135^\star}$
\end{tabular}
}
\end{table*}

\subsubsection{Significance Test} To verify whether the improvement of FGCNN over baseline models is significant, we conduct Significance test as follows. We repeat the experiments for 10 times for FGCNN and the best baseline model and two-tailed pairwise t-test is performed to detect significant differences between FGCNN and the best baseline model. p-value of the t-test being less than $10^{-3}$ means the improvement is significant. 

\begin{table*}[t]
\caption{Performances of Different FGCNN Variants}
\label{table:remove}
\begin{tabular}{c|cc|cc|cc}
       & \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c}{Company} \\ \hline
Method & AUC          & Log Loss     & AUC         & Log Loss     & AUC          & Log Loss     \\ \hline
FGCNN  & \textbf{80.22\%}      & \textbf{0.5388}      & \textbf{78.83\%}     & \textbf{0.3746}       & \textbf{94.05\%}      & \textbf{0.1135}       \\
Removing Raw Features   & 80.21\%      & 0.5390       & 78.66\%     & 0.3757        & 93.98\%      &0.1141       \\
Removing New Features   & 80.13\%      & 0.5399       & 78.68\%     & 0.3757       & 93.87\%      & 0.1148       \\
Applying MLP for Feature Generation   & 80.12\%      & 0.5402       & 78.58\%     & 0.3761       & 94.04\%             &0.1135              \\
Removing Recombination Layer    & 80.11\%      & 0.5403       & 78.74\%     & 0.3753       & 94.04\%             & 0.1135             \\
%Removing Factorization Machine    & 80.09\%      & 0.5402       & 78.55\%     & 0.3764       &  94.00\%            &   0.1139           \\
%Using One Embedding Matrix   & 80.17\%      & 0.5394       & 78.68\%     & 0.3755       &     94.04\%        &  0.1136           
\end{tabular}
\end{table*}

\subsection{Overall Performance (Q1)}

In this subsection, we compare the performance of different models on the test set. Table~\ref{table:overall} summarizes the overall performances of all the compared models obtained on the three datasets, where underline numbers are the best results of the baseline models and bold numbers are the best results of all.
We have the following oberservations:

First, in majority of the cases, non-nueral network models perform worse than neural network models. As a powerful approach to learning feature representations, deep nueral network can learn sophisticated feature interactions much better than the models in which no feature interaction is modeled (i.e., LR), or the feature interactions are modeled by simple inner product operations (i.e., FM and FFM).

Second, we see that FGCNN achieves the best performance among all the models on the three evaluated datasets. It betters than PIN, which is the second best model, by 0.01\%, 0.14\% and 0.17\% in terms of AUC (0.03\%, 0.23\% and 0.96\% in terms of log loss) on Criteo, Avazu and Company datasets, which demonstrates the effectiveness of FGCNN. We conduct significant test to verify whether the improvement of FGCNN over PIN is significant. The p-value shows that FGCNN's improvement on Avazu and Company datasets is significant while is not the case on Criteo dataset. In fact, a small improvement in offline AUC is likely to lead to a significant increase in online CTR. As reported in~\cite{cheng2016wide}, compared with LR, Wide \& Deep improves AUC by 0.275\% (offline) and the improvement of online CTR is 3.9\%. The daily turnover of Company's App Store is millions of dollars, therefore even several percents lift in CTR brings extra millions of dollars each year. We also observe that FGCNN does not achieve significant improvement over PIN on Criteo dataset. The possible reason may be that modeling pairwise feature interactions play very important roles in Criteo dataset, and PIN's Micro-Network is able to learn such interactions better than inner product operations in FGCNN model.

Third, FGCNN outperforms IPNN by 0.11\%, 0.19\% and 0.19\% in terms of AUC (0.2\%, 0.29\% and 1.13\% in terms of log loss) on Criteo, Avazu and Company datasets, which verifies the effectiveness of \emph{feature generation} part of FGCNN model.

Fourth, CCPM, which applies CNN model directly, achieves the worst performancce among all the nueral network models; moreover, CCPM is worse than FFM on Criteo and Avazu datasets. It demonstrates that it is unsatisfying to directly using traditional CNN for CTR prediction task, as CNN is designed to generate neighbor patterns while the arrangement order of feature is usually no meaning in recommendation scenarios. 

\subsection{Effectiveness of FGCNN Variants (Q2)}

To study \textbf{Q2}, we conduct experiments to compare the performance among several variants of FGCNN model, where each variant is generated by removing or replacing some components in \emph{feature generation} part in FGCNN. The compared variants are described as follows:

\begin{itemize}
\item \textbf{Removing Raw Features}: In this variant, only new generated features (but not the original raw features) are fed to \emph{deep predictive learning} part in FGCNN.
 \item \textbf{Removing New Features}: This variant serves as the complementory of the first one, i.e., it removes the \emph{feature generation} part completely. This variant actually is IPNN.
 \item \textbf{Applying MLP for Feature Generation}: The \emph{feature generation} part of FGCNN is replacing by a MLP, with equal number of neurons in each layer. The numbers of neurons in different layers are designed to be consistent with the size of generated features in Recombination layers of original FGCNN.
 \item \textbf{Removing Recombination Layer}: This variant is to evaluate how recombination layer serves an a complementory of CNN to capture global pattern. In this variant, the recombination layer is removed from the \emph{feature generation} part of FGCNN so that it uses the output of pooling layer as new features.
% \item \textbf{Removing Factorization Machine}: removes the factorization machine Layer in the model.
% \item \textbf{Using One Embedding Matrix}: use the same embedding matrix for feature generation and DNN.
\end{itemize}

Table~\ref{table:remove} compared the performance of the listed FGCNN variants. As can be shown, removing any structure in FGCNN leads to performancce dropping. The detailed observations are discussed as follows.

First, FGCNN with original raw features or with new generated features alone performs worse than the FGCNN with both raw features and generated features. This result demonstrates that the generated features are good supplementary of the original features, which are both very crucial. 

Second, the performancce decrease of \textit{Appling MLP for Feature Generation}, compared to FGCNN, shows the ineffectiveness of MLP to identify important feature combinations from the large feature space. The combination of CNN and MLP simplifies the learning difficulties by using much less parameters than applying MLP entirely, with the idea of identifying local neighbor feature patterns via CNN and learning global feature interactions by MLP. 

Third, the recombination layer of \emph{feature generation} is important, of which the functionality is to capture global feature interactions to generate new features. As stated earlier, the arragement order of features has no meaning in CTR prediction task, removing recombination layer and leaving only CNN limit the \emph{feature generation} with only local neighbor feature patterns, which result in worse performance.
%Fourthly, \textit{Removing Factorization Machine} has the greatest impact on the performance, which shows the usefullness of Factorization Machine to capture explicit low-order feature interactions.
%Finally, if we only use the same embedding matrix for both feature generation part and Deep Predictive Learning part, the direction gradients from feature generation part and  DNN part may contradict which hinders the learning of FGCNN model. Therefore, using double embedding matrixs can be a good choice.

%Finally, the results of \textit{Replacing the convolution by Full Connection}
 %shows that although DNN can approximate any functions ideally, due to the large parameter space, it is usually hard to optimize. Therefore, the performance of \textit{Replacing the convolution by Full Connection} is relatively poor.  And it is even worse than \textit{Without New Features}, which shows new features generated by Full Connection are actually data noises.  We also have further experiments in the next section to show how the height of convolution kernel impacts(the bigger in height, the closer to Full Connection) the final performances, and it also demonstrates bigger heights often result in worse performances.
 
\subsection{Compatibility of FGCNN with Different Deep Predictive Models (Q3)}

As stated earlier in the paper, \emph{deep predictive learning} of FGCNN can be applied by any advanced deep neural networks. In this subsection, we study the follow research question: if we apply any state-of-the-art neural network as the \emph{deep predictive learning}, whether the \emph{feature generation} part will always boost the performance? If the answer is positive, the \emph{feature generation} can be viewed as an augmentation component to enhance any popular existing work, which demonstrates the good compatibility of FGCNN model

Table~\ref{table:integrete} presents the performancce comparison w/o \emph{feature generation}, when the \emph{deep predictive learning} is adopted with different models (i.e., FM, IPNN, DeepFM, DNN), in order to show FGCNN's compatibility. As can be observed, \emph{feature generation} part consistently improves the performance when every and each of the models are applied as the \emph{deep predictive learning}. Therefore, FGCNN can be viewed as a general framework to enhance the existing nerual networks by generating new features.

\begin{table*}[]
\caption{Compatibility Study of FGCNN}
\label{table:integrete}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c|}{Company} \\ \hline
& \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} \\ \hline
IPNN & 80.13\% & 0.5399 & 78.68\% & 0.3757 & 93.87\% & 0.1148 \\
FGCNN+IPNN & 80.22\% & 0.5388 & 78.83\% & 0.3746 & 94.05\% & 0.1135 \\ \hline
FM & 79.09\% & 0.5500 & 77.93\% & 0.3805 & 93.26\% & 0.1191 \\
FGCNN+FM & 79.67\% & 0.5455 & 78.13\% & 0.3794 & 93.66\% & 0.1165 \\ \hline
DeepFM & 79.91\% & 0.5423 & 78.36\% & 0.3777 & 93.84\% & 0.1149 \\
FGCNN+DeepFM & & & & & 93.93\% & 0.1145 \\ \hline
DNN & 79.87\% & 0.5428 & 78.30\% & 0.3778 & \% & \\
FGCNN+DNN & 80.09\% &0.5402 & 78.55\% & 0.3764 & 94.00\% & 0.1139 \\ \hline
\end{tabular}
}
\end{table*}

\subsection{Hyper-parameter Investigation (Q4)}
 
Our FGCNN model has several key hyper-parameters, i.e., height of convolution kernels, number of convolution kernels, number of convolution layers, and number of kernels for generating new features. In this subsection, to study the impact of these hyper-parameters, we investigate how FGCNN model works with the change of one hyper-parameter, while fixing the others.
 
\subsubsection{Height of Convolution Kernels}
 
The height of convolution kernels controls the percetion range of convolution layers. The larger the height is, local neighbor patterns of more features can be learned, but more weight parameters have to be optimized. We increase the height from 2 to the number of features in each dataset. As shown in Figure~\ref{fig:height}, AUC increases as the height increases at the beginning. However, after reaching a peak point, AUC decreases as the height continues increasing. The main reasons are two folds: \emph{first}, at the beginning when height increases, more features are treated as neighbors so as their features are learned, therefore the performance increases; \emph{second}, when height keeps increasing, the model training becomes more difficult as there are more weight parameters have to be optimized. Note that, when the height of convolution kernels is the number of features, a convolution layer is similar to a fully-connect layer. The performance decreasing when the height of convolution layer keeps increasing is consistent with the phenomenon that it is not performing well when applying MLP in \emph{feature generation} of FGCNN.
 
\subsubsection{Number of Convolution Layers}
 
As presented in Figure~\ref{fig:layers}, increasing the number of convolutional layers from 1 to 4 helps improving the performance of FGCNN. It may due to the fact that high-order feature interactions are very useful. \textcolor{red}{higher convolution layers}
 
\subsubsection{Number of Convolution Kernels}
 
Figure~\ref{fig:layers} shows how the performance of FGCNN changes when the number of convolution kernels increases. The x-axis of the figures represents the number of convolution kernels in each convolution layer. FGCNN achieves best performance when the numbers of convolution kernels are [38-40-42-44], [6-8-10-14] and [14-16-28-20] on Criteo, Avazu and Company datasets, respectively. The possible reason is that when a dataset involves more fields, more convolution kernels are needed to learn local neighbor feature interactions to generate useful new features. Recall that the numbers of fields in Criteo, Avazu and Company datasets are 39, 24 and 24, respectively.

\subsubsection{Number of Kernels for Generating New Features}
 
Lastly, we study how FGCNN works when changing the number of kernels for generating new features. As can be observed in Figure~\ref{fig:new}, increasing the number of kernels for generating new features leads to AUC improvement on Criteo and Avazu datasets. This phenomenon suggests that generating more new features will have more positive impact on final performance. \textcolor{red}{Huawei Dataset seems to be problematic.}
 
\subsection{Effect of Shuffling Order of Raw Features (Q5)}

As known, CNN is designed to capture local neighbor feature patterns so that it is sensitive to the arragement order of raw features. In this subsection, we study whether the arrangement order of raw features affect the performance of FGCNN. As stated earlier, the functionality of Recombination layer is to learn global non-neighbor feature interactions on the basis of CNN's exacted local feature patterns, aiming to alleviate the effect of changing the arrangement order of new features. To verify it, we compare the performance of two cases: w/o Recombination layers, when the arragement order of raw features is determined uniformly at random, repeating multiple times. The result of this set of experiments is summerized in Figure~\ref{fig:shuffle} and Table~\ref{table:shuffle}. 
 
The result shows that the case with Recombination layer achieves better (i.e., higher average AUC) and more stable (lower standard deviation) than that of without Recombination layer, which demonstrates the effect of Recombination layer to handle different arragement order of raw features. 
 
\begin{table}[]
\caption{average and standard deviation of AUC when shuffling arragement order of raw features multiple times}
\label{table:shuffle}
\begin{tabular}{|c|c|c|c|c|}
\hline
        & \multicolumn{2}{l|}{Without Recombination} & \multicolumn{2}{l|}{With Recombination} \\ \hline
        & average              & std                 & average             & std               \\ \hline
Criteo  & 80.08\%              & 0.01\%              & \textbf{80.20\% }            & \textbf{0.01\%  }          \\ \hline
Avazu   & 78.75\%              & 0.05\%              & \textbf{78.76\% }            &\textbf{0.03\% }           \\ \hline
Company & 94.01\%              & 0.01\%              & \textbf{94.02\%}             & \textbf{0.01\% }           \\ \hline
\end{tabular}
\end{table}
 \begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{height.jpg}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Height of Convolution Layers}\label{fig:height}
 \label{height}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{layers.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Number of Convolution Layers}\label{fig:layers}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{kernel.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Number of Convolution Kernels}\label{fig:kernels}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{new.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Number of Kernels for Generating New Features}\label{fig:new}
 \label{new}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{shuffle.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Shuffling Order of the Features}\label{fig:shuffle}
 \label{shuffle}
\end{figure*}




==> fgcnn www2019/experiments.tex <==
\section{Experiments}
In this section, we conduct extensive experiments to answer the following questions:
\begin{itemize}
       \item \textbf{(Q1)} Is it true that identifying important features first by CNN can boost the performance of DNN models?
       \item \textbf{(Q2)} How does each component in FGCNN affect the final performance?
       \item \textbf{(Q3)} How does the key parameters of  FGCNN impact its performance?
\end{itemize}
\subsection{Experiment Setup}
\subsubsection{Datasets} we conduct extensive experiments in the following three datasets:

\textit{Criteo}: Criteo\footnote{http://labs.criteo.com/downloads/download-terabyte-click-logs/} contains one month of click logs with billions of data samples. A small subset of Criteo was published in Criteo Display Advertising Challenge, 2013 and FFM was the winning solution~\cite{pin, ffm}. 'Day 6-12' is selected for training while 'day 13' is selected for evaluation. Due to the enormous data volume and serious imbalance(only 3\% samples is positive), negative sampling is applied to keep the imbalance ratio close to 1:1. We convert 13 numerical fields into one-hot features through bucketing. And the features in a certain field appearing less than 20 times are set as a dummy feature "other".

\textit{Avazu}: Avazu\footnote{http://www.kaggle.com/c/avazu-ctr-prediction} was published in the contest of Avazu Click-Through Rate Prediction, 2014. The publich dataset is randomly splitted into training and test sets at 4:1. Meanwhile, we remove the features appearing less than 20 times to reduce dimensionality.

\textit{Company}: In order to verify the performance of FGCNN in real  industrial CTR prediction, we conduct experiment on Company* Dataset. we collect  users' click logs record from the game center of Company* App Store while logs from 20180617 to 20180623 is used for training and logs in 20180624 is used for testing. The datasets contains app, user and context features. 

\begin{table}[]
\caption{Dataset statistics}
\label{dataset}
\begin{tabular}{l|llll}
Dataset & \#instances & \#features & \#fields & pos ratio \\ \hline
Criteo & 1$\times$10\textasciicircum{}8 & 1$\times$10\textasciicircum{}6 & 39 & 0.5 \\
Avazu & 4$\times$10\textasciicircum{}7 & 6$\times$10\textasciicircum{}5 & 24 & 0.17 \\
Company & 2.3$\times$10\textasciicircum{}8 & 1.6$\times$10\textasciicircum{}5 & 29 & 0.05
\end{tabular}
\end{table}

Table \ref{dataset} summarizes the statistics of 4 datasets.
\subsubsection{Baselines} 
Eight baseline models is selected for comparison, including LR~\cite{lr}, GBDT~\cite{gbdt}, FM~\cite{fm}, FFM~\cite{ffm}, CCPM~\cite{ccpm}, DeepFM~\cite{deepfm}, xDeepFM~\cite{xdeepfm}, IPNN~\cite{pin} and PIN~\cite{pin}. And since Wide\&Deep model needs feature engineering, it is not compared here. We use XGBoost~\cite{gbdt} and libFFM\footnote{https://github.com/guestwalk/libffm} as GBDT and libFFM in our experiments. Other models are implemented with Tensorflow.
\subsubsection{Evaluation Metrics} The evaluation metics are \textbf{AUC} and \textbf{log loss}.
\subsubsection{Parameter Settings}

\begin{table}[]
\caption{Parameter Settings Pooling not added}
\label{parameter}
\scriptsize
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
 & Criteo & Avazu & Company \\ \hline
General & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=1000\\ opt=Adam\\ lr=1e-4\\ l2=1e-6\end{tabular} \\ \hline
LR & - & - & - \\ \hline
GBDT & \begin{tabular}[c]{@{}l@{}}depth=25\\ \#tree=1300\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=18\\ \#tree=1000\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=10\\ \#tree=1400\end{tabular} \\ \hline
FM & k=20 & k=40 & k=40 \\ \hline
FFM & k=4 & k=4 & k=12 \\ \hline
CCPM & \begin{tabular}[c]{@{}l@{}}k=20\\     conv= 7*1\\    kernel={[}256{]}\\     net={[}256*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv: 7*1\\     kernel = {[}128{]}\\     net= {[}128*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv= 2*1\\     kernel= {[}8,16,32,64{]}\\     net={[}512,256,128,1{]}\\     drop= 0.8\end{tabular} \\ \hline
DeepFM & \begin{tabular}[c]{@{}l@{}}k=20, LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\end{tabular} \\ \hline
XdeepFM & \begin{tabular}[c]{@{}l@{}}k=20\\     net={[}400*3,1{]}\\     CIN={[}100*4{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}700*5,1{]}\\     CIN:{[}100*2{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\\     CIN:{[}100{]}\end{tabular} \\ \hline
IPNN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     \end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\    \end{tabular} \\ \hline
PIN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\\     subnet={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     sub-net={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\     sub-net={[}40,10{]}\end{tabular} \\ \hline
FGCNN & \begin{tabular}[c]{@{}l@{}}k=20\\     conv=9*1\\  pool=2*1\\     kernel={[}38,40,42,44{]}\\     new={[}3,3,3,3{]}\\     BN=True\\     net={[}4096,2048,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=7*1\\ pool=2*1\\    kernel={[}6,8,10,14{]}\\     new={[}3,3,3,3{]}\\     BN=T\\     net={[}4096,2048,1024,\\ 512,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=13*1\\  pool=2*1 \\   kernel={[}6-8-10-12{]}\\     new={[}2,2,2,2{]}\\     BN=T\\     net={[}2048,1024,\\ 512,256,128,1{]}\\     drop=0.8\end{tabular} \\ \hline
\end{tabular}
}
Notice: bs=Batch Size, opt=Optimizer, lr=Learning Rate, l2=L2 Regularization on Embedding Layer, k = Embedding size, conv= Convolution Kernel shape, kernel = Convolution kernels(Feature map),pool=max-pooling shape, net= DNN Structure, sub-net = Micro Network, drop = dropout rate, LN= Layer Normalization, BN= batch normalization, new = new feature map num for each feature generation.
\end{table}
Table~\ref{parameter} summerizes the hyperparameters for each model.
For \textit{Criteo} and \textit{Avazu} Datasets, the same hyperparameters as ~\cite{pin} is used to reproduce their results. In the FGCNN model, to simplify the parameter of the number of generated feature, we introduce parameter \textit{new} which works as the kernel in the convolution layer. The number of generated features can be calculated as $\sum_{i=1}^l \#fields/2^i*new_i$.

\begin{table*}[t]
\caption{Overall Performances\\
$\star: p<0.0001$}
\label{overall}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lllllll}
        & \multicolumn{2}{c}{Criteo}                                    & \multicolumn{2}{c}{Avazu}                                              & \multicolumn{2}{c}{Company}                        \\ \hline
Model   & AUC                 & \multicolumn{1}{l|}{Log Loss}           & AUC(\%)                  & \multicolumn{1}{l|}{Log Loss}               & AUC                      & Log Loss                \\ \hline
LR      & 78.00\%             & \multicolumn{1}{l|}{0.5631}             & 76.76\%                  & \multicolumn{1}{l|}{0.3868}                 & 90.12\%                  & 0.1371                  \\
GBDT    & 78.62\%             & \multicolumn{1}{l|}{0.5560}             & 77.53\%                  & \multicolumn{1}{l|}{0.3824}                 & 92.68\%                  & 0.1227                  \\
FM      & 79.09\%             & \multicolumn{1}{l|}{0.5500}             & 77.93\%                  & \multicolumn{1}{l|}{0.3805}                 & 93.26\%                  & 0.1191                  \\
FFM     & 79.80\%             & \multicolumn{1}{l|}{0.5438}             & 78.31\%                  & \multicolumn{1}{l|}{0.3781}                 & 93.58\%                  & 0.1170                  \\
CCPM    & 79.55\%             & \multicolumn{1}{l|}{0.5469}             & 78.12\%                  & \multicolumn{1}{l|}{0.3800}                 & 93.68\%                  & 0.1162                  \\
DeepFM  & 79.91\%             & \multicolumn{1}{l|}{0.5423}             & 78.30\%                  & \multicolumn{1}{l|}{0.3778}                 & 93.84\%                  & 0.1149                  \\
xDeepfm & 80.06\%             & \multicolumn{1}{l|}{0.5408}             & 78.55\%                  & \multicolumn{1}{l|}{0.3766}                 & 93.82\%                  & 0.1152                  \\
IPNN    & 80.13\%             & \multicolumn{1}{l|}{0.5399}             & 78.68\%                  & \multicolumn{1}{l|}{0.3757}                 & 93.87\%                  & 0.1148                  \\
PIN     & \underline{80.21\%} & \multicolumn{1}{l|}{\underline{0.5390}} & \underline{78.72\%}      & \multicolumn{1}{l|}{\underline{0.3755}}     & \underline{93.89\%}      & \underline{0.1146}      \\ \hline
FGCNN   & \textbf{80.22\%}    & \multicolumn{1}{l|}{\textbf{0.5388}}    & $\mathbf{78.83\%^\star}$ & \multicolumn{1}{l|}{$\mathbf{0.3746^\star}$} & $\mathbf{94.05\%^\star}$ & $\mathbf{0.1135^\star}$
\end{tabular}
}

\end{table*}
\subsubsection{Significance Test} To show whether the improvements is significant, we repeat the experiments for 5 times on FGCNN and the best baseline model. Then, two-tailed pairwise t-test is performed to detect significant differences between FGCNN and the best baseline model.
\begin{table*}[t]
\caption{Performances after removing the component in FGCNN}
\label{remove}
\begin{tabular}{l|ll|ll|ll}
       & \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c}{Company} \\ \hline
Method & AUC          & Log Loss     & Auc         & Log Loss     & Auc          & Log Loss     \\ \hline
FGCNN  & \textbf{80.22\%}      & \textbf{0.5388}      & \textbf{78.83\%}     & \textbf{0.3746}       & \textbf{94.05\%}      & \textbf{0.1135}       \\
Without Raw Features   & 80.21\%      & 0.5390       & 78.66\%     & 0.3757        & 93.98\%      &0.1141       \\
Without New Features   & 80.13\%      & 0.5399       & 78.68\%     & 0.3757       & 93.87\%      & 0.1148       \\
Replacing Convolution by MLP   & 80.12\%      & 0.5402       & 78.58\%     & 0.3761       & 94.04\%             &0.1135              \\
Removing Recombination Layer    & 80.11\%      & 0.5403       & 78.74\%     & 0.3753       & 94.04\%             & 0.1135             \\
Removing Factorization Machine    & 80.09\%      & 0.5402       & 78.55\%     & 0.3764       &  94.00\%            &   0.1139           \\
Using One Embedding Matrix   & 80.17\%      & 0.5394       & 78.68\%     & 0.3755       &     94.04\%        &  0.1136           
\end{tabular}
\end{table*}

\subsection{Overall Performance(Q1)}
Table ~\ref{overall} shows the overall performances, where underline numbers are the best results of baseline models and bold numbers are the best results of all. There are several oberservations:

Firstly, among all basline models, PIN is the best baseline model in three datasets. while xDeepFM(the third best model) tries to learn explicit and implicit low and high order feature interactions, PIN uses a micro network to learn pairwised feature interaction which demonstrates the effectiveness of order-2 cross features. In all baseline models, LR achives worst performance in the three datasets, which demonstrates that factorization-based models are essential for modeling sparse feature in the CTR prediction task. Moreover, CCPM is the worst deep learning model, which shows that it is unsatisfactory to directly using traditional Convolutional Neural Network to make predictions for click-through rate predictions. The main reason is that the arrangement of features in the CTR prediction does not have the different meaning like images and sentences, which makes traditional CNN model difficult to find useful neighboring information on a random feature arrangement. 

Secondly, FGCNN achieves the best performance on all datasets. In Company dataset, our prposed FGCNN model beats competitors by more than 0.16\% in AUC and 0.11\% in log loss. In fact, a small improvement in offline AUC evaluation is likely lead to a significant increase in online CTR.
As shown in ~\cite{cheng2016wide}, 0.275\% improvements in AUC lead to 3.8\% improvement in online CTR. The daily turnover of Company's APP store is millions of dollars, therefore even several percents increase in CTR can bring extra millions of dollars a year.
Recall that we only use inner product to learn explict feature interactions between generated features and old features, which is quite simple than PIN(using Micro Network for each feature pair). It can demonstrate that our FGCNN model do extract important cross features and the generated features do reduce the optimization difficulties of DNNs thus yielding better performances. Despite the significant improvements on \textit{Avazu} and \textit{Company} datasets, the FGCNN model can not achieve significant improvements than PIN on \textit{Criteo} Dataset. The possible reason is that pairwised feature interactions play an important role on the final performance and Micro-Network learns the interactions better than Inner Product. 

\subsection{Component Importances(Q2)}

To investigate how each component contributes to the actual performances, we conduct several experiments by removing some component on our FGCNN model:
\begin{itemize}
\item \textbf{Without Raw Features}: raw features are disregarded in the second part of FGCNN. Only generated features is fed to FM and Deep component.
 \item \textbf{Without New Features}: the feature generation process is removed in FGCNN. Only the raw features is fed to FM and Deep component.
 \item \textbf{Replacing Convolution by MLP}: Convolution layer is replaced by multi-layer  of full connections, hidden neurons in such layer is used as new features. The distribution of generated new features in MLP is exactly same as it in the Recombination Layer.
 \item \textbf{Removing Recombination Layer}: removes the recombination layer in FGCNN and uses the results of pooling layer as new features.
 \item \textbf{Removing Factorization Machine}: removes the factorization machine Layer in the model.
 \item \textbf{Using One Embedding Matrix}: use the same embedding matrix for feature generation and DNN.
\end{itemize}


%\textcolor{red}{adding the Replacing Convolution by Full Connection model picture}

Table ~\ref{remove} summerizes the performances after removing the components in FGCNN. As it shows, removing any components in FGCNN can lead to a drop in the performance.

Firstly, Only using raw features or new features rarely results in an optimal model, which demonstrate that the generated features are a good supplementary for the original feature space. Secondly, the decrease of performance after \textit{Replacing Convolution with MLP} shows it is difficult for Multi-Layer Perceptrons to identify important feature combinations in the large combinational space while CNN+Pooling+Recombination simplifies the its difficulties. 
Thirdly, if we remove the recombination layer, FGCNN is restricted by the feature interactions of neighbor features. Since the arragement order has no actual meaning in CTR prediction and it is usually quite randomized, it is necessary to recombine the neighboring information to generate global feature interactions.
Fourthly, \textit{Removing Factorization Machine} has the greatest impact on the performance, which shows the usefullness of Factorization Machine to capture explicit low-order feature interactions.
Finally, if we only use the same embedding matrix for both feature generation part and Deep Predictive Learning part, the direction gradients from feature generation part and  DNN part may contradict which hinders the learning of FGCNN model. Therefore, using double embedding matrixs can be a good choice.


%Finally, the results of \textit{Replacing the convolution by Full Connection}
 %shows that although DNN can approximate any functions ideally, due to the large parameter space, it is usually hard to optimize. Therefore, the performance of \textit{Replacing the convolution by Full Connection} is relatively poor.  And it is even worse than \textit{Without New Features}, which shows new features generated by Full Connection are actually data noises.  We also have further experiments in the next section to show how the height of convolution kernel impacts(the bigger in height, the closer to Full Connection) the final performances, and it also demonstrates bigger heights often result in worse performances.
\subsection{Compatibility with Other Models}
In the FGCNN model,  the generated features in the first layers can be viewed as an augmentation of original features. Therefore, many models can be used in our second component. FM, DeepFM, IPNN is compared in Table~\ref{integrete} to show FGCNN's Compatibilities. 
\begin{table*}[]
\caption{Integreting FGCNN with other models}
\label{tab:integrete}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
             & \multicolumn{2}{c|}{Criteo}                              & \multicolumn{2}{c|}{Avazu}                               & \multicolumn{2}{c|}{Company}                             \\ \hline
             & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} \\ \hline
IPNN         & 80.13\%                  & 0.5399                        & 78.68\%                  & 0.3757                        & 93.87\%                  & 0.1148                        \\
FGCNN+IPNN   & 80.22\%                  & 0.5388                        & 78.83\%                  & 0.3746                        & 94.05\%                  & 0.1135                        \\ \hline
FM           & 79.09\%                  & 0.5500                        & 77.93\%                  & 0.3805                        & 93.26\%                  & 0.1191                        \\
FGCNN+FM     &  79.67\%                        &  0.5455                             & 78.13\%                  & 0.3794                        & 93.66\%                         &  0.1165                             \\ \hline
DeepFM       & 79.91\%                  & 0.5423                        & 78.36\%                  & 0.3777                        & 93.84\%                  & 0.1149                        \\
FGCNN+DeepFM &                          &                               &                          &                               &   93.93\%                 &  0.1145                         \\ \hline
DNN       & 79.87\%                  & 0.5428                        & 78.30\%                  & 0.3778                        &  \%                  &                         \\
FGCNN+DNN &       80.09\%             &0.5402                               &   78.55\%                       &  0.3764                             &       94.00\%                   &        0.1139                      \\ \hline
\end{tabular}
}
\end{table*}
 \subsection{Parameter Analysis}
 We analyse some key parameters in FGCNN, to show how the parameters affect the performance of FGCNN.
 \subsubsection{Convolution Height}
 The first parameter is convolution height, which controls the percetion range of convolution layer. We try to increase the height from 2 to the number of features in each datasets. As shown in Figure ~\ref{height}, AUC often increases as the initial height increases.  After a critical point, AUC starts to decreases as the height continue increasing. The main reason is that the optimization difficuties is much higher when using bigger convolution heights, which is also the reason why full connections layers can not work well in identifying important patterns.
 \subsubsection{Convolution Layers}
 Experiments on different convolution layers show that as more convolution layers are used, performance is always better, which shows high-order feature interactions are very useful. \textcolor{red}{higher convolution layers}
 \subsubsection{Convolution Kernels}
 Convolution kernels is the second studied parameters. As Figure~\ref{layers} shows, AUC seems to increase with the increase of the number of used kernels in Criteo while AUC has a unstable correlations with the number of kernels. The possible reason is that the number of fields in criteo(39) is much more than it in Avazu(24). Therefore, the combination space in Criteo is much bigger than Avazu. So, more kernels are needed to generate important features. 
 \subsubsection{Number of Generated Features}
 We also studied how the number of new feature map after each pooling layer affect the performance. As Figure~\ref{new} shows, with the inrease of new feature map num, AUC in criteo is improved, and in Avazu the biggest new feature map num lead to the best AUC. it demonstrates that the generated new features have a great impact on final performance.
 
 \subsection{Will the arrangement order of raw features affect FGCNN?}
 Since CNN  will be affected by the arrangement of features, we wonder that if the order of features affects the performance of FGCNN. To study it, we shuffled the order of features before feeding it into \textit{feature generation} part. Recall that the major difference between \textit{feature generation} and traditional CNN structure is that \textit{feature generation} has a recombination layer which is designed to combine the neighboring interactions from CNN and generate global feature interactions. The recombination layer has the potential to break the limitation of CNN to learn effective combinations in any given inpute orders. To verify it, we compare models in two settings: without Recombination and with Recombination. The experiments are repeated in ten times and same model settings are applied here.  Figure ~\ref{shuffle} and Table~\ref{tab:shuffle} summerize such experiments. 
 
 As shown in Table ~\ref{tab:shuffle}, the setting with recombination achieve more stable(low standard deviation) and better performance(high average AUC) than it without recombination Layer. It demonstrates that FGCNN is more robust than traditional CNN. Due to that our best model in the original setting can be also viewed as a random arrangement of features, it is highly likely to achieve better performance based on better parameter settings in any randomized arragements.
 
 
 \begin{table}[]
\caption{AUCs after shuffling features' arrangement order}
\label{tab:shuffle}
\begin{tabular}{|l|l|l|l|l|}
\hline
        & \multicolumn{2}{l|}{Without Recombination} & \multicolumn{2}{l|}{With Recombination} \\ \hline
        & average              & std                 & average             & std               \\ \hline
Criteo  & 80.08\%              & 0.01\%              & \textbf{80.20\% }            & \textbf{0.01\%  }          \\ \hline
Avazu   & 78.75\%              & 0.05\%              & \textbf{78.76\% }            &\textbf{0.03\% }           \\ \hline
Company & 94.01\%              & 0.01\%              & \textbf{94.02\%}             & \textbf{0.01\% }           \\ \hline
\end{tabular}
\end{table}
 \begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{height.jpg}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Convolutional Height}
 \label{height}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{layers.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Convolutional Layers}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{kernel.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Convolutional Kernel}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{new.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{New feature map nums}
 \label{new}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{shuffle.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Shuffling the feature order}
 \label{shuffle}
\end{figure*}




==> fgcnn www2019/experiments_1025_ruiming.tex <==
\section{Experiments}

In this section, we conduct extensive experiments to answer the following questions. 
\begin{itemize}
       \item \textbf{(Q1)} How does FCGNN perform, compared to the state-of-the-art models for CTR prediction task?
       \item \textbf{(Q2)} How does each key structure in FGCNN boost the prediction performance?
       \item \textbf{(Q3)} How is the compatibility of FGCNN, i.e., applying different network structures as its \emph{deep predictive learning} part.
       \item \textbf{(Q4)} How do the key hyper-parameters of FGCNN (i.e., size and number of convolution kernels, number of generated features) impact its performance?
       \item \textbf{(Q5)} How does the \emph{feature generation} part perform when the order of raw features are random shuffled.
\end{itemize}

Note that when studying questions other than \textbf{Q3}, we adpot IPNN as the \emph{deep predictive learning} of FGCNN.

\subsection{Experimental Setup}

\subsubsection{Datasets} we conduct the experiment with the following three datasets:

\textit{Criteo}: Criteo\footnote{http://labs.criteo.com/downloads/download-terabyte-click-logs/} contains one month of click logs with billions of data samples. A small subset of Criteo was published in Criteo Display Advertising Challenge, 2013 and FFM was the winning solution~\cite{pin, ffm}. We select ``day 6-12'' as training set while select ``day 13'' for evaluation. Due to the enormous data volume and serious class imbalance (i.e., only 3\% samples are positive), negative sampling is applied to keep the positive and negative ratio close to 1:1. We convert 13 numerical fields into one-hot features through bucketing, where the features in a certain field appearing less than 20 times are set as a dummy feature ``other".

\textit{Avazu}: Avazu\footnote{http://www.kaggle.com/c/avazu-ctr-prediction} was published in the contest of Avazu Click-Through Rate Prediction, 2014. The publich dataset is randomly splitted into training and test sets at 4:1. Meanwhile, we remove the features appearing less than 20 times to reduce dimensionality.

\textit{Company}: In order to verify the performance of FGCNN in real industrial CTR prediction, we conduct experiment on Company Dataset. We collect users' click logs from Company App Store while logs from 20180617 to 20180623 is used for training and logs of 20180624 is used for test. Negative sampling is applied to reduce data amount and to balance the positive and negative ratio. The datasets contains app features (e.g., identification, category, etc), user features (e.g., user's behavior history, etc) and context features (e.g., operation time, etc). 

\begin{table}[]
\caption{Dataset statistics}
\label{table:dataset}
\begin{tabular}{l|llll}
Dataset & \#instances & \#features & \#fields & pos ratio \\ \hline
Criteo & $1\times 10^{8}$ & $1\times 10^{6}$ & 39 & 0.5 \\
Avazu & $4\times 10^{7}$ & $6\times 10^{5}$ & 24 & 0.17 \\
Company & $2.3\times 10^{8}$ & $1.6\times 10^{5}$ & 29 & 0.05
\end{tabular}
\end{table}

Table~\ref{table:dataset} summarizes the statistics of the three datasets.

\subsubsection{Baselines} 

We compare eight baseline models in our experiment, including LR~\cite{lr}, GBDT~\cite{gbdt}, FM~\cite{fm}, FFM~\cite{ffm}, CCPM~\cite{ccpm}, DeepFM~\cite{deepfm}, xDeepFM~\cite{xdeepfm}, IPNN and PIN~\cite{pin}. We use XGBoost~\cite{gbdt} and libFFM\footnote{https://github.com/guestwalk/libffm} as the implementation of GBDT and libFFM in our experiments, and the other baseline models are implemented with Tensorflow\footnote{https://www.tensorflow.org/}.

\subsubsection{Evaluation Metrics} The evaluation metics are \textbf{AUC} (Area Under ROC) and \textbf{log loss} (cross entropy).

\subsubsection{Parameter Settings}

\begin{table}[]
\caption{Parameter Settings}
\label{table:parameter}
\scriptsize
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
 & Criteo & Avazu & Company \\ \hline
General & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular} & \begin{tabular}[c]{@{}l@{}}bs=1000\\ opt=Adam\\ lr=1e-4\\ l2=1e-6\end{tabular} \\ \hline
LR & - & - & - \\ \hline
GBDT & \begin{tabular}[c]{@{}l@{}}depth=25\\ \#tree=1300\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=18\\ \#tree=1000\end{tabular} & \begin{tabular}[c]{@{}l@{}}depth=10\\ \#tree=1400\end{tabular} \\ \hline
FM & k=20 & k=40 & k=40 \\ \hline
FFM & k=4 & k=4 & k=12 \\ \hline
CCPM & \begin{tabular}[c]{@{}l@{}}k=20\\     conv= 7*1\\    kernel={[}256{]}\\     net={[}256*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv: 7*1\\     kernel = {[}128{]}\\     net= {[}128*3,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv= 2*1\\     kernel= {[}8,16,32,64{]}\\     net={[}512,256,128,1{]}\\     drop= 0.8\end{tabular} \\ \hline
DeepFM & \begin{tabular}[c]{@{}l@{}}k=20, LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\end{tabular} \\ \hline
XdeepFM & \begin{tabular}[c]{@{}l@{}}k=20\\     net={[}400*3,1{]}\\     CIN={[}100*4{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}700*5,1{]}\\     CIN:{[}100*2{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     net={[}400*3,1{]}\\     drop=0.9\\     CIN:{[}100{]}\end{tabular} \\ \hline
IPNN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     \end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\    \end{tabular} \\ \hline
PIN & \begin{tabular}[c]{@{}l@{}}k=20\\     LN=T\\     net={[}700*5,1{]}\\     subnet={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     LN=T\\     net={[}500*5,1{]}\\     sub-net={[}40,5{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=30\\     net={[}1000*3,1{]}\\     drop=0.7\\     sub-net={[}40,10{]}\end{tabular} \\ \hline
FGCNN & \begin{tabular}[c]{@{}l@{}}k=20\\     conv=9*1\\  pool=2*1\\     kernel={[}38,40,42,44{]}\\     new={[}3,3,3,3{]}\\     BN=T\\     net={[}4096,2048,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=7*1\\ pool=2*1\\    kernel={[}6,8,10,14{]}\\     new={[}3,3,3,3{]}\\     BN=T\\     net={[}4096,2048,1024,\\ 512,1{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\     conv=13*1\\  pool=2*1 \\   kernel={[}6,8,10,12{]}\\     new={[}2,2,2,2{]}\\     BN=T\\     net={[}2048,1024,\\ 512,256,128,1{]}\\     drop=0.8\end{tabular} \\ \hline
\end{tabular}
}
Note: bs=Batch Size, opt=Optimizer, lr=Learning Rate, l2=L2 Regularization on Embedding Layer, k=Embedding Size, conv=Convolution Kernel shape, kernel=number of Convolution Kernels, pool=Max-Pooling Shape, net=MLP Structure, sub-net=Micro Network, drop=Keep Rate(drop=1.0 if not stated), LN=Layer Normalization, BN= Batch Normalization\{T=True\}, new=number of Kernels Generating New Features.
\end{table}

Table~\ref{table:parameter} summerizes the hyperparameters of each model.
For \textit{Criteo} and \textit{Avazu} Datasets, the hyperparameters of baseline models are set the same as in~\cite{pin}, in order to reproduce their results. In the FGCNN model, \textit{new} is the number of kernels when generating new features. The number of generated features can be calculated as $\sum_{i=1}^l \#fields/2^i*new_i$.

\begin{table*}[t]
\caption{Overall Performances\\
$\star: p < 10^{-4}$ (two-tailed t-test)}
\label{table:overall}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lllllll}
        & \multicolumn{2}{c}{Criteo}                                    & \multicolumn{2}{c}{Avazu}                                              & \multicolumn{2}{c}{Company}                        \\ \hline
Model   & AUC                 & \multicolumn{1}{l|}{Log Loss}           & AUC(\%)                  & \multicolumn{1}{l|}{Log Loss}               & AUC                      & Log Loss                \\ \hline
LR      & 78.00\%             & \multicolumn{1}{l|}{0.5631}             & 76.76\%                  & \multicolumn{1}{l|}{0.3868}                 & 90.12\%                  & 0.1371                  \\
GBDT    & 78.62\%             & \multicolumn{1}{l|}{0.5560}             & 77.53\%                  & \multicolumn{1}{l|}{0.3824}                 & 92.68\%                  & 0.1227                  \\
FM      & 79.09\%             & \multicolumn{1}{l|}{0.5500}             & 77.93\%                  & \multicolumn{1}{l|}{0.3805}                 & 93.26\%                  & 0.1191                  \\
FFM     & 79.80\%             & \multicolumn{1}{l|}{0.5438}             & 78.31\%                  & \multicolumn{1}{l|}{0.3781}                 & 93.58\%                  & 0.1170                  \\
CCPM    & 79.55\%             & \multicolumn{1}{l|}{0.5469}             & 78.12\%                  & \multicolumn{1}{l|}{0.3800}                 & 93.68\%                  & 0.1162                  \\
DeepFM  & 79.91\%             & \multicolumn{1}{l|}{0.5423}             & 78.30\%                  & \multicolumn{1}{l|}{0.3778}                 & 93.84\%                  & 0.1149                  \\
xDeepfm & 80.06\%             & \multicolumn{1}{l|}{0.5408}             & 78.55\%                  & \multicolumn{1}{l|}{0.3766}                 & 93.82\%                  & 0.1152                  \\
IPNN    & 80.13\%             & \multicolumn{1}{l|}{0.5399}             & 78.68\%                  & \multicolumn{1}{l|}{0.3757}                 & 93.87\%                  & 0.1148                  \\
PIN     & \underline{80.21\%} & \multicolumn{1}{l|}{\underline{0.5390}} & \underline{78.72\%}      & \multicolumn{1}{l|}{\underline{0.3755}}     & \underline{93.89\%}      & \underline{0.1146}      \\ \hline
FGCNN   & \textbf{80.22\%}    & \multicolumn{1}{l|}{\textbf{0.5388}}    & $\mathbf{78.83\%^\star}$ & \multicolumn{1}{l|}{$\mathbf{0.3746^\star}$} & $\mathbf{94.05\%^\star}$ & $\mathbf{0.1135^\star}$
\end{tabular}
}
\end{table*}

\subsubsection{Significance Test} To verify whether the improvement of FGCNN over baseline models is significant, we conduct Significance test as follows. We repeat the experiments for 10 times for FGCNN and the best baseline model and two-tailed pairwise t-test is performed to detect significant differences between FGCNN and the best baseline model. p-value of the t-test being less than $10^{-3}$ means the improvement is significant. 

\begin{table*}[t]
\caption{Performances of Different FGCNN Variants}
\label{table:remove}
\begin{tabular}{c|cc|cc|cc}
       & \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c}{Company} \\ \hline
Method & AUC          & Log Loss     & AUC         & Log Loss     & AUC          & Log Loss     \\ \hline
FGCNN  & \textbf{80.22\%}      & \textbf{0.5388}      & \textbf{78.83\%}     & \textbf{0.3746}       & \textbf{94.05\%}      & \textbf{0.1135}       \\
Removing Raw Features   & 80.21\%      & 0.5390       & 78.66\%     & 0.3757        & 93.98\%      &0.1141       \\
Removing New Features   & 80.13\%      & 0.5399       & 78.68\%     & 0.3757       & 93.87\%      & 0.1148       \\
Applying MLP for Feature Generation   & 80.12\%      & 0.5402       & 78.58\%     & 0.3761       & 94.04\%             &0.1135              \\
Removing Recombination Layer    & 80.11\%      & 0.5403       & 78.74\%     & 0.3753       & 94.04\%             & 0.1135             \\
%Removing Factorization Machine    & 80.09\%      & 0.5402       & 78.55\%     & 0.3764       &  94.00\%            &   0.1139           \\
%Using One Embedding Matrix   & 80.17\%      & 0.5394       & 78.68\%     & 0.3755       &     94.04\%        &  0.1136           
\end{tabular}
\end{table*}

\subsection{Overall Performance (Q1)}

In this subsection, we compare the performance of different models on the test set. Table~\ref{table:overall} summarizes the overall performances of all the compared models obtained on the three datasets, where underline numbers are the best results of the baseline models and bold numbers are the best results of all.
We have the following oberservations:

First, in majority of the cases, non-nueral network models perform worse than neural network models. As a powerful approach to learning feature representations, deep nueral network can learn sophisticated feature interactions much better than the models in which no feature interaction is modeled (i.e., LR), or the feature interactions are modeled by simple inner product operations (i.e., FM and FFM).

Second, we see that FGCNN achieves the best performance among all the models on the three evaluated datasets. It betters than PIN, which is the second best model, by 0.01\%, 0.14\% and 0.17\% in terms of AUC (0.03\%, 0.23\% and 0.96\% in terms of log loss) on Criteo, Avazu and Company datasets, which demonstrates the effectiveness of FGCNN. We conduct significant test to verify whether the improvement of FGCNN over PIN is significant. The p-value shows that FGCNN's improvement on Avazu and Company datasets is significant while is not the case on Criteo dataset. In fact, a small improvement in offline AUC is likely to lead to a significant increase in online CTR. As reported in~\cite{cheng2016wide}, compared with LR, Wide \& Deep improves AUC by 0.275\% (offline) and the improvement of online CTR is 3.9\%. The daily turnover of Company's App Store is millions of dollars, therefore even several percents lift in CTR brings extra millions of dollars each year. We also observe that FGCNN does not achieve significant improvement over PIN on Criteo dataset. The possible reason may be that modeling pairwise feature interactions play very important roles in Criteo dataset, and PIN's Micro-Network is able to learn such interactions better than inner product operations in FGCNN model.

Third, FGCNN outperforms IPNN by 0.11\%, 0.19\% and 0.19\% in terms of AUC (0.2\%, 0.29\% and 1.13\% in terms of log loss) on Criteo, Avazu and Company datasets, which verifies the effectiveness of \emph{feature generation} part of FGCNN model.

Fourth, CCPM, which applies CNN model directly, achieves the worst performancce among all the nueral network models; moreover, CCPM is worse than FFM on Criteo and Avazu datasets. It demonstrates that it is unsatisfying to directly using traditional CNN for CTR prediction task, as CNN is designed to generate neighbor patterns while the arrangement order of feature is usually no meaning in recommendation scenarios. 

\subsection{Effectiveness of FGCNN Variants (Q2)}

To study \textbf{Q2}, we conduct experiments to compare the performance among several variants of FGCNN model, where each variant is generated by removing or replacing some components in \emph{feature generation} part in FGCNN. The compared variants are described as follows:

\begin{itemize}
\item \textbf{Removing Raw Features}: In this variant, only new generated features (but not the original raw features) are fed to \emph{deep predictive learning} part in FGCNN.
 \item \textbf{Removing New Features}: This variant serves as the complementory of the first one, i.e., it removes the \emph{feature generation} part completely. This variant actually is IPNN.
 \item \textbf{Applying MLP for Feature Generation}: The \emph{feature generation} part of FGCNN is replacing by a MLP, with equal number of neurons in each layer. The numbers of neurons in different layers are designed to be consistent with the size of generated features in Recombination layers of original FGCNN.
 \item \textbf{Removing Recombination Layer}: This variant is to evaluate how recombination layer serves an a complementory of CNN to capture global pattern. In this variant, the recombination layer is removed from the \emph{feature generation} part of FGCNN so that it uses the output of pooling layer as new features.
% \item \textbf{Removing Factorization Machine}: removes the factorization machine Layer in the model.
% \item \textbf{Using One Embedding Matrix}: use the same embedding matrix for feature generation and DNN.
\end{itemize}

Table~\ref{table:remove} compared the performance of the listed FGCNN variants. As can be shown, removing any structure in FGCNN leads to performancce dropping. The detailed observations are discussed as follows.

First, FGCNN with original raw features or with new generated features alone performs worse than the FGCNN with both raw features and generated features. This result demonstrates that the generated features are good supplementary of the original features, which are both very crucial. 

Second, the performancce decrease of \textit{Appling MLP for Feature Generation}, compared to FGCNN, shows the ineffectiveness of MLP to identify important feature combinations from the large feature space. The combination of CNN and MLP simplifies the learning difficulties by using much less parameters than applying MLP entirely, with the idea of identifying local neighbor feature patterns via CNN and learning global feature interactions by MLP. 

Third, the recombination layer of \emph{feature generation} is important, of which the functionality is to capture global feature interactions to generate new features. As stated earlier, the arragement order of features has no meaning in CTR prediction task, removing recombination layer and leaving only CNN limit the \emph{feature generation} with only local neighbor feature patterns, which result in worse performance.
%Fourthly, \textit{Removing Factorization Machine} has the greatest impact on the performance, which shows the usefullness of Factorization Machine to capture explicit low-order feature interactions.
%Finally, if we only use the same embedding matrix for both feature generation part and Deep Predictive Learning part, the direction gradients from feature generation part and  DNN part may contradict which hinders the learning of FGCNN model. Therefore, using double embedding matrixs can be a good choice.

%Finally, the results of \textit{Replacing the convolution by Full Connection}
 %shows that although DNN can approximate any functions ideally, due to the large parameter space, it is usually hard to optimize. Therefore, the performance of \textit{Replacing the convolution by Full Connection} is relatively poor.  And it is even worse than \textit{Without New Features}, which shows new features generated by Full Connection are actually data noises.  We also have further experiments in the next section to show how the height of convolution kernel impacts(the bigger in height, the closer to Full Connection) the final performances, and it also demonstrates bigger heights often result in worse performances.
 
\subsection{Compatibility of FGCNN with Different Deep Predictive Models (Q3)}

As stated earlier in the paper, \emph{deep predictive learning} of FGCNN can be applied by any advanced deep neural networks. In this subsection, we study the follow research question: if we apply any state-of-the-art neural network as the \emph{deep predictive learning}, whether the \emph{feature generation} part will always boost the performance? If the answer is positive, the \emph{feature generation} can be viewed as an augmentation component to enhance any popular existing work, which demonstrates the good compatibility of FGCNN model

Table~\ref{table:integrete} presents the performancce comparison w/o \emph{feature generation}, when the \emph{deep predictive learning} is adopted with different models (i.e., FM, IPNN, DeepFM, DNN), in order to show FGCNN's compatibility. As can be observed, \emph{feature generation} part consistently improves the performance when every and each of the models are applied as the \emph{deep predictive learning}. Therefore, FGCNN can be viewed as a general framework to enhance the existing nerual networks by generating new features.

\begin{table*}[]
\caption{Compatibility Study of FGCNN}
\label{table:integrete}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c|}{Company} \\ \hline
& \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Log Loss} \\ \hline
IPNN & 80.13\% & 0.5399 & 78.68\% & 0.3757 & 93.87\% & 0.1148 \\
FGCNN+IPNN & 80.22\% & 0.5388 & 78.83\% & 0.3746 & 94.05\% & 0.1135 \\ \hline
FM & 79.09\% & 0.5500 & 77.93\% & 0.3805 & 93.26\% & 0.1191 \\
FGCNN+FM & 79.67\% & 0.5455 & 78.13\% & 0.3794 & 93.66\% & 0.1165 \\ \hline
DeepFM & 79.91\% & 0.5423 & 78.36\% & 0.3777 & 93.84\% & 0.1149 \\
FGCNN+DeepFM & & & & & 93.93\% & 0.1145 \\ \hline
DNN & 79.87\% & 0.5428 & 78.30\% & 0.3778 & \% & \\
FGCNN+DNN & 80.09\% &0.5402 & 78.55\% & 0.3764 & 94.00\% & 0.1139 \\ \hline
\end{tabular}
}
\end{table*}

\subsection{Hyper-parameter Investigation (Q4)}
 
Our FGCNN model has several key hyper-parameters, i.e., height of convolution kernels, number of convolution kernels, number of convolution layers, and number of kernels for generating new features. In this subsection, to study the impact of these hyper-parameters, we investigate how FGCNN model works with the change of one hyper-parameter, while fixing the others.
 
\subsubsection{Height of Convolution Kernels}
 
The height of convolution kernels controls the percetion range of convolution layers. The larger the height is, local neighbor patterns of more features can be learned, but more weight parameters have to be optimized. We increase the height from 2 to the number of features in each dataset. As shown in Figure~\ref{fig:height}, AUC increases as the height increases at the beginning. However, after reaching a peak point, AUC decreases as the height continues increasing. The main reasons are two folds: \emph{first}, at the beginning when height increases, more features are treated as neighbors so as their features are learned, therefore the performance increases; \emph{second}, when height keeps increasing, the model training becomes more difficult as there are more weight parameters have to be optimized. Note that, when the height of convolution kernels is the number of features, a convolution layer is similar to a fully-connect layer. The performance decreasing when the height of convolution layer keeps increasing is consistent with the phenomenon that it is not performing well when applying MLP in \emph{feature generation} of FGCNN.
 
\subsubsection{Number of Convolution Layers}
 
As presented in Figure~\ref{fig:layers}, increasing the number of convolutional layers from 1 to 4 helps improving the performance of FGCNN. It may due to the fact that high-order feature interactions are very useful. \textcolor{red}{higher convolution layers}
 
\subsubsection{Number of Convolution Kernels}
 
Figure~\ref{fig:layers} shows how the performance of FGCNN changes when the number of convolution kernels increases. The x-axis of the figures represents the number of convolution kernels in each convolution layer. FGCNN achieves best performance when the numbers of convolution kernels are [38-40-42-44], [6-8-10-14] and [14-16-28-20] on Criteo, Avazu and Company datasets, respectively. The possible reason is that when a dataset involves more fields, more convolution kernels are needed to learn local neighbor feature interactions to generate useful new features. Recall that the numbers of fields in Criteo, Avazu and Company datasets are 39, 24 and 24, respectively.

\subsubsection{Number of Kernels for Generating New Features}
 
Lastly, we study how FGCNN works when changing the number of kernels for generating new features. As can be observed in Figure~\ref{fig:new}, increasing the number of kernels for generating new features leads to AUC improvement on Criteo and Avazu datasets. This phenomenon suggests that generating more new features will have more positive impact on final performance. \textcolor{red}{Huawei Dataset seems to be problematic.}
 
\subsection{Effect of Shuffling Order of Raw Features (Q5)}

As known, CNN is designed to capture local neighbor feature patterns so that it is sensitive to the arragement order of raw features. In this subsection, we study whether the arrangement order of raw features affect the performance of FGCNN. As stated earlier, the functionality of Recombination layer is to learn global non-neighbor feature interactions on the basis of CNN's exacted local feature patterns, aiming to alleviate the effect of changing the arrangement order of new features. To verify it, we compare the performance of two cases: w/o Recombination layers, when the arragement order of raw features is determined uniformly at random, repeating multiple times. The result of this set of experiments is summerized in Figure~\ref{fig:shuffle} and Table~\ref{table:shuffle}. 
 
The result shows that the case with Recombination layer achieves better (i.e., higher average AUC) and more stable (lower standard deviation) than that of without Recombination layer, which demonstrates the effect of Recombination layer to handle different arragement order of raw features. 
 
\begin{table}[]
\caption{average and standard deviation of AUC when shuffling arragement order of raw features multiple times}
\label{table:shuffle}
\begin{tabular}{|c|c|c|c|c|}
\hline
        & \multicolumn{2}{l|}{Without Recombination} & \multicolumn{2}{l|}{With Recombination} \\ \hline
        & average              & std                 & average             & std               \\ \hline
Criteo  & 80.08\%              & 0.01\%              & \textbf{80.20\% }            & \textbf{0.01\%  }          \\ \hline
Avazu   & 78.75\%              & 0.05\%              & \textbf{78.76\% }            &\textbf{0.03\% }           \\ \hline
Company & 94.01\%              & 0.01\%              & \textbf{94.02\%}             & \textbf{0.01\% }           \\ \hline
\end{tabular}
\end{table}
 \begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{height.jpg}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Height of Convolution Layers}\label{fig:height}
 \label{height}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{layers.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Number of Convolution Layers}\label{fig:layers}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{kernel.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Number of Convolution Kernels}\label{fig:kernels}
 \label{layers}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{new.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Number of Kernels for Generating New Features}\label{fig:new}
 \label{new}
\end{figure*}
\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{shuffle.png}
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \caption{Shuffling Order of the Features}\label{fig:shuffle}
 \label{shuffle}
\end{figure*}




==> fgcnn www2019/experiments_1026_huifeng.tex <==
\section{Experiments}

In this section, we conduct extensive experiments to answer the following questions.
\begin{itemize}
       \item \textbf{(Q1)} How does FGCNN perform, compared to the state-of-the-art models for CTR prediction task?
       \item \textbf{(Q2)} Can FGCNN improve the performance of other state-of-the-art models by using their structures in  \emph{Deep Classifier}?
       \item \textbf{(Q3)} How does each key structure in FGCNN boost the performance of FGCNN?
       \item \textbf{(Q4)} How do the key hyper-parameters of FGCNN
(i.e., size of convolutional kernels,number of convolutional layers, number
of generated features) impact its performance?
       \item \textbf{(Q5)} How does  \emph{Feature Generation}  perform when the order of raw features are randomly shuffled?
\end{itemize}

Note that when studying questions other than \textbf{Q2}, we adpot IPNN as the \emph{Deep Classifier} in FGCNN.

\subsection{Experimental Setup}
\begin{table}[t]
\caption{Dataset Statistics}
\vspace{-3ex}
\label{table:dataset}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|llll}
\hline
Dataset & \#instances & \#features & \#fields & pos ratio \\ \hline
Criteo & $1\times 10^{8}$ & $1\times 10^{6}$ & 39 & 0.5 \\
Avazu & $4\times 10^{7}$ & $6\times 10^{5}$ & 24 & 0.17 \\
Huawei App Store & $2.3\times 10^{8}$ & $1.6\times 10^{5}$ & 29 & 0.05 \\\hline
\end{tabular}
}
\vspace{-1ex}
\end{table}
\begin{table}[h]
\vspace{-3ex}
\caption{Parameter Settings}
\vspace{-3ex}
\label{table:parameter}
\scriptsize
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
Param   & Criteo                                                                                                                       & Avazu                                                                                                                               & Huawei App Store                                                                                                                                            \\ \hline
General & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular}                                                         & \begin{tabular}[c]{@{}l@{}}bs=2000\\ opt=Adam\\ lr=1e-3\end{tabular}                                                                & \begin{tabular}[c]{@{}l@{}}bs=1000\\ opt=Adam\\ lr=1e-4\\ l2=1e-6\end{tabular}                                                                     \\ \hline
LR      & --                                                                                                                           & --                                                                                                                                  & --                                                                                                                                                 \\ \hline
GBDT    & \begin{tabular}[c]{@{}l@{}}depth=25\\ \#tree=1300\end{tabular}                                                               & \begin{tabular}[c]{@{}l@{}}depth=18\\ \#tree=1000\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}}depth=10\\ \#tree=1400\end{tabular}                                                                                     \\ \hline
FM      & k=20                                                                                                                         & k=40                                                                                                                                & k=40                                                                                                                                               \\ \hline
FFM     & k=4                                                                                                                          & k=4                                                                                                                                 & k=12                                                                                                                                               \\ \hline
CCPM    & \begin{tabular}[c]{@{}l@{}}k=20\\ conv= 7*1\\ kernel=[256]\\ net=[256*3,1]\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}k=40\\ conv: 7*1\\ kernel = [128]\\ net= [128*3,1]\end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}k=40\\ conv= 13*1\\ kernel= [8,16,32,64]\\ net=[512,256,128,1]\\ drop= 0.8\end{tabular}                                  \\ \hline
DeepFM  & \begin{tabular}[c]{@{}l@{}}k=20\\ LN=T\\ net=[700*5,1]\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}k=40\\ LN=T\\ net=[500*5,1]\end{tabular}                                                                 & \begin{tabular}[c]{@{}l@{}}k=40\\ net=[2048,1024,512,1]\\ drop=0.9\end{tabular}                                                                    \\ \hline
XdeepFM & \begin{tabular}[c]{@{}l@{}}k=20\\ net=[400*3,1]\\ CIN=[100*4]\end{tabular}                                                   & \begin{tabular}[c]{@{}l@{}}k=40\\ net=[700*5,1]\\ CIN:[100*2]\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}k=40\\ net=[2048,1024,512,1]\\ drop=0.9\\ CIN:[100*4]\end{tabular}                                                                \\ \hline
IPNN    & \begin{tabular}[c]{@{}l@{}}k=20\\ LN=T\\ net=[700*5,1]\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}k=40\\ LN=T\\ net=[500*5,1]\end{tabular}                                                                 & \begin{tabular}[c]{@{}l@{}}k=40\\ net=[2048,1024,\\ 512,256,128,1]\\ drop=0.7\end{tabular}                                                         \\ \hline
PIN     & \begin{tabular}[c]{@{}l@{}}k=20\\ LN=T\\ net=[700*5,1]\\ subnet=[40,5]\end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}k=40\\ LN=T\\ net=[500*5,1]\\ sub-net=[40,5]\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}k=40\\ net=[2048,1024,512,1]\\ drop=0.9\\ sub-net=[80,10]\end{tabular}                                                  \\ \hline
FGCNN   & \begin{tabular}[c]{@{}l@{}}k=20\\ conv=9*1\\ kernel=[38,40,42,44]\\ new=[3,3,3,3]\\ BN=T\\ ruenet=[4096,2048,1]\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\ conv=7*1\\ kernel=[14,16,18,20]\\ new=[3,3,3,3]\\ BN=T\\ net=[4096,2048,\\ 1024,512,1]\end{tabular} & \begin{tabular}[c]{@{}l@{}}k=40\\ conv=13*1\\ kernel=[6, 8, 10, 12]\\ new=[2,2,2,2]\\ BN=T\\ net=[2048,1024,\\ 512,256,128,1]\\ drop=0.8\end{tabular} \\ \hline
\end{tabular}
}
Note: bs=batch size, opt=optimizer, lr=learning rate, l2=l2 regularization on Embedding Layer, k=embedding size, conv=shape of convolutional kernels, kernel=number of convolutional kernels, pool=max-pooling shape, net=MLP structure, sub-net=micro metwork, drop=dropout rate, LN=layer normalization, BN= batch normalization\{T=True\}, new=number of kernels for new features.
\vspace{-5ex}
\end{table}
\begin{table*}[t]
\centering
\vspace{-4ex}
%\scriptsize
\caption{Overall Performance\\
$\star: p < 10^{-2}\ \star\star: p<10^{-4} $ (two tailed t-test)}
\vspace{-3ex}
\label{table:overall}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lll|ll|ll}
 \hline\hline
        & \multicolumn{2}{|c|}{Criteo}                                    & \multicolumn{2}{|c|}{Avazu}                                              & \multicolumn{2}{|c}{Huawei App Store}                        \\ \hline
\multicolumn{1}{l|}{Model}   & AUC                 & \multicolumn{1}{l|}{Log Loss}           & AUC(\%)                  & \multicolumn{1}{l|}{Log Loss}               & AUC                      & Log Loss                \\ \hline
\multicolumn{1}{l|}{LR}      & 78.00\%             & \multicolumn{1}{l|}{0.5631}             & 76.76\%                  & \multicolumn{1}{l|}{0.3868}                 & 90.12\%                  & 0.1371                  \\
\multicolumn{1}{l|}{GBDT}    & 78.62\%             & \multicolumn{1}{l|}{0.5560}             & 77.53\%                  & \multicolumn{1}{l|}{0.3824}                 & 92.68\%                  & 0.1227                  \\
\multicolumn{1}{l|}{FM}      & 79.09\%             & \multicolumn{1}{l|}{0.5500}             & 77.93\%                  & \multicolumn{1}{l|}{0.3805}                 & 93.26\%                  & 0.1191                  \\
\multicolumn{1}{l|}{FFM}     & 79.80\%             & \multicolumn{1}{l|}{0.5438}             & 78.31\%                  & \multicolumn{1}{l|}{0.3781}                 & 93.58\%                  & 0.1170                  \\
\multicolumn{1}{l|}{CCPM}    & 79.55\%             & \multicolumn{1}{l|}{0.5469}             & 78.12\%                  & \multicolumn{1}{l|}{0.3800}                 & 93.71\%                  & 0.1159                 \\
\multicolumn{1}{l|}{DeepFM}  & 79.91\%             & \multicolumn{1}{l|}{0.5423}             & 78.36\%                  & \multicolumn{1}{l|}{0.3777}                 & 93.91\%                  & 0.1145                  \\
\multicolumn{1}{l|}{xDeepFM} & 80.06\%             & \multicolumn{1}{l|}{0.5408}             & 78.55\%                  & \multicolumn{1}{l|}{0.3766}                 & 93.91\%                  & 0.1146                 \\
\multicolumn{1}{l|}{IPNN}    & 80.13\%             & \multicolumn{1}{l|}{0.5399}             & 78.68\%                  & \multicolumn{1}{l|}{0.3757}                 & \underline{93.95}\%                  & \underline{0.1143}                  \\
\multicolumn{1}{l|}{PIN}     & \underline{80.18\%}\footnotemark[11] & \multicolumn{1}{l|}{\underline{0.5393}} & \underline{78.72\%}      & \multicolumn{1}{l|}{\underline{0.3755}}     & 93.91\%      & 0.1146      \\ \hline
\multicolumn{1}{l|}{FGCNN}   & $\mathbf{80.22\%}^\star$     & \multicolumn{1}{l|}{$\mathbf{0.5388}^\star$}    & $\mathbf{78.83\%^{\star\star}}$ & \multicolumn{1}{l|}{$\mathbf{0.3746^{\star\star}}$} & $\mathbf{94.07\%^{\star\star}}$ & $\mathbf{0.1134^{\star\star}}$\\ \hline\hline
\end{tabular}
}
\vspace{-3ex}
\end{table*}


\subsubsection{Datasets} Experiments are conducted in the following three datasets:

\textit{Criteo}: Criteo\footnote{http://labs.criteo.com/downloads/download-terabyte-click-logs/} contains one month of click logs with billions of data samples. A small subset of Criteo was published in Criteo Display Advertising Challenge 2013 and FFM was the winning solution~\cite{pin, ffm}. We select ``day 6-12'' as training set while select ``day 13'' for evaluation. Due to the enormous data volume and serious class imbalance (i.e., only 3\% samples are positive), negative sampling is applied to keep the positive and negative ratio close to 1:1. We convert 13 numerical fields into one-hot features through bucketing, where the features in a certain field appearing less than 20 times are set as a dummy feature ``other``.

\textit{Avazu}: Avazu\footnote{http://www.kaggle.com/c/avazu-ctr-prediction} was published in the contest of Avazu Click-Through Rate Prediction, 2014. The public dataset is randomly splitted into training and test sets at 4:1. Meanwhile, we remove the features appearing less than 20 times to reduce dimensionality.

\textit{Huawei App Store}: In order to evaluate the performance in industrial CTR prediction problems, we conduct experiments on Huawei App Store Dataset. We collect users' click logs from Huawei App Store while logs from 20180617 to 20180623 are used for training and logs of 20180624 are used for test. Negative sampling is applied to reduce data amount and to adjust the ratio of positive class and negative class. The dataset contains app features (e.g., identification, category), user features (e.g., user's behavior history) and context features (e.g., operation time).




In addition, the statistics of the three datasets are summarized in Table~\ref{table:dataset}.

\subsubsection{Baselines}

We compare nine baseline models in our experiments, including LR~\cite{lr}, GBDT~\cite{gbdt}, FM~\cite{fm}, FFM~\cite{ffm}, CCPM~\cite{ccpm}, DeepFM~\cite{deepfm}, xDeepFM~\cite{xdeepfm}, IPNN and PIN~\cite{pin}. Wide \& Deep is not compared here because some state-of-the-art models (such as xDeepFM, DeepFM, PIN) have shown better performance in their publications. We use XGBoost~\cite{gbdt} and libFFM\footnote{https://github.com/guestwalk/libffm} as the implementation of GBDT and libFFM, respectively.  In our experiments, the other baseline models are implemented with Tensorflow\footnote{https://www.tensorflow.org/}.

\subsubsection{Evaluation Metrics} The evaluation metrics are \textbf{AUC} (Area Under ROC) and \textbf{log loss} (cross entropy).

\subsubsection{Parameter Settings}




Table~\ref{table:parameter} summerizes the hyper-parameters of each model.
For \textit{Criteo} and \textit{Avazu} Datasets, the hyper-parameters of baseline models are set to be the same as in~\cite{pin}. Notice that when conducting experiments on Criteo and Avazu, we observed that FGCNN uses more parameters in \emph{Deep Classifier} than other models. To make fair comparisons, we also conduct experiments to increase the parameters in MLPs of other deep models. However, all these models cannot achieve better performance than the original settings\footnote{Due to the limited pages, we do not show the experimental result in the paper.}. The reason could be the overfitting problem where such models simply use embedding of raw features for training but use a complex structure. On the other hand, since our model augments the feature space and enriches the input, more parameters in \emph{Deep Classifier} can boost the performance of our model.

In FGCNN model, \textit{new} is the number of kernels when generating new features. The number of generated features can be calculated as $\sum_{i=1}^{n_c} \#fields/2^i*new_i$.



\subsubsection{Significance Test} We repeat the experiments 10 times by changing the random seed for FGCNN and the best baseline model. The two-tailed pairwise t-test is performed to detect significant differences between FGCNN and the best baseline model. %p-value of the t-test being less than $10^{-3}$ means the improvement is significant.
\begin{table*}[]
\caption{Compatibility Study of FGCNN}
\vspace{-3ex}
\label{table:integrete}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{c|ll|ll|ll}
\hline\hline
& \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c}{Huawei App Store} \\ \hline
& \multicolumn{1}{l}{AUC} & \multicolumn{1}{l|}{Log Loss} & \multicolumn{1}{l}{AUC} & \multicolumn{1}{l|}{Log Loss} & \multicolumn{1}{l}{AUC} & \multicolumn{1}{l}{Log Loss} \\ \hline
FM & 79.09\% & 0.5500 & 77.93\% & 0.3805 & 93.26\% & 0.1191 \\
FGCNN+FM & \textbf{79.67\%} & \textbf{0.5455} & \textbf{78.13\%} & \textbf{0.3794}  & \textbf{93.66}\% & \textbf{0.1165} \\ \hline
DNN & 79.87\% & 0.5428 & 78.30\% & 0.3778 & 93.85\% &0.1149 \\
FGCNN+DNN & \textbf{80.09\%} &\textbf{0.5402} & \textbf{78.55\%} & \textbf{0.3764} & \textbf{94.00\%} & \textbf{0.1139} \\ \hline
DeepFM & 79.91\% & 0.5423 & 78.36\% & 0.3777 & 93.91\% & 0.1145 \\
FGCNN+DeepFM & \textbf{79.94\%} & \textbf{0.5421}&\textbf{78.44\%} & \textbf{0.3771}& \textbf{93.93\%} & \textbf{0.1145} \\ \hline
IPNN & 80.13\% & 0.5399 & 78.68\% & 0.3757 & 93.95\% & 0.1143 \\
FGCNN+IPNN & \textbf{80.22\%} & \textbf{0.5388} & \textbf{78.83\%} & \textbf{0.3746} & \textbf{94.07\%} & \textbf{0.1134} \\ \hline
\hline

\end{tabular}
}
\vspace{-2ex}
\end{table*}



\subsection{Overall Performance (Q1)}
\footnotetext[11]{According to the experimental recordings, the results of PIN in ~\cite{pin} uses the trick of adaptive embedding size. Here, we use fixed embedding size for all the deep models.}

In this subsection, we compare the performance of different models on the test set. Table~\ref{table:overall} summarizes the overall performance of all the compared models on the three datasets, where the underlined numbers are the best results of the baseline models and bold numbers are the best results of all models.
We have the following observations:

Firstly, in majority of the cases, non-neural network models perform worse than neural network models. The reason is that deep neural network can learn complex feature interactions much better than the models where no feature interaction is modeled (i.e., LR), or feature interactions are modeled by simple inner product operations (i.e., FM and FFM).

Secondly,  FGCNN achieves the best performance among all the models on the three evaluated datasets. It is significantly better than the best baseline models with 0.05\%, 0.14\% and 0.13\% improvements in AUC (0.09\%, 0.24\% and 0.79\% in log loss) on Criteo, Avazu and Huawei App Store datasets, which demonstrates the effectiveness of FGCNN.  In fact, a small improvement in offline AUC is likely to lead to a significant increase in online CTR. As reported in~\cite{cheng2016wide}, compared with LR, Wide \& Deep improves offline AUC by 0.275\% and the improvement of online CTR is 3.9\%. The daily turnover of Huawei App Store is millions of dollars. Therefore, even a few lifts in CTR brings extra millions of dollars each year. %We also observe that FGCNN does not achieve significant improvement over PIN on Criteo dataset. The possible reason may be that modeling pairwise feature interactions plays very important role in Criteo dataset, and PIN's Micro-Network is able to learn such interactions better than inner product operations in FGCNN model.

Thirdly, with the help of the generated new features, FGCNN outperforms IPNN by 0.11\%, 0.19\% and 0.13\% in terms of AUC (0.2\%, 0.29\% and 0.79\% in terms of log loss) on Criteo, Avazu and Huawei App Store datasets. It demonstrates that the generated features are very useful and  they can effectively reduce the optimization difficulties of traditional DNNs thus leading to better performance.

Fourthly, CCPM, which applies CNN directly, achieves the worst performance among neural network models.  Moreover, CCPM performs worse than FFM on Criteo and Avazu datasets. It shows that directly using traditional CNN for CTR prediction task is inadvisable, as CNN is designed to generate neighbor patterns while the arrangement order of feature is usually no meaning in recommendation scenarios. However, in FGCNN, we leverage the strength of CNN to extract local patterns while complementing it with Recombination Layer to extract global feature interactions and generate new features. Therefore, better performance is achieved.
\subsection{Compatibility of FGCNN with Different Models (Q2)}

As stated in Section ~\ref{sec:clf}, \emph{Feature Generation}  can augment the original feature space and \emph{Deep Classifier} of FGCNN can adopt any advanced deep neural networks. Therefore, we select several models  as \emph{Deep Classifeir} to verify the utility of \emph{Feature Generation}, including non-deep models (FM), deep learning models (DNN, DeepFM, IPNN).

Table~\ref{table:integrete} summarizes the performance. We have the following observations: Firstly, with the help of the generated new features, the performance of all models are improved, which demonstrates the effectiveness of the generated features and shows the compatibility of FGCNN. Secondly, we observe that when only using raw features, DeepFM always outperforms DNN. But when using the augmented features, FGCNN+DNN outperforms FGCNN+DeepFM. The possible reason is that DeepFM sums up the inner product of input features to the last MLP layer which may cause contradictory gradient updates (compared with MLP) on embeddings.% and increase the learning difficulties of the model. 
This could be one of the reasons why IPNN (feeding the product into MLP) outperforms DeepFM in all datasets.

In a word, the results show that our FGCNN model can be viewed as a general framework to enhance the existing neural networks by generating new features automatically.

\subsection{Effectiveness of FGCNN Variants(Q3)}
\begin{table*}[t]
\vspace{-2ex}
\caption{Performance of Different FGCNN Variants}
\vspace{-3ex}
\label{table:remove}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll}
\hline\hline
       & \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu} & \multicolumn{2}{c}{Huawei App Store} \\ \hline
Method & AUC          & Log Loss     & AUC         & Log Loss     & AUC          & Log Loss     \\ \hline
FGCNN  & \textbf{80.22\%}      & \textbf{0.5388}      & \textbf{78.83\%}     & \textbf{0.3746}       & \textbf{94.07\%}      & \textbf{0.1134}       \\
Removing Raw Features   & 80.21\%      & 0.5390       & 78.66\%     & 0.3757        & 94.01\%      &0.1138       \\
Removing New Features   & 80.13\%      & 0.5399       & 78.68\%     & 0.3757       &  93.95\%      &  0.1143      \\
Applying MLP for Feature Generation   & 80.12\%      & 0.5402       & 78.58\%     & 0.3761       & 94.04\%             &0.1135              \\
Removing Recombination Layer    & 80.11\%      & 0.5403       & 78.74\%     & 0.3753       & 94.04\%             & 0.1135             \\
\hline\hline
%Removing Factorization Machine    & 80.09\%      & 0.5402       & 78.55\%     & 0.3764       &  94.00\%            &   0.1139           \\
%Using One Embedding Matrix   & 80.17\%      & 0.5394       & 78.68\%     & 0.3755       &     94.04\%        &  0.1136
\end{tabular}
}
\vspace{-2ex}
\end{table*}


 We conduct experiments to study how each component in FGCNN contributes to the final performance. Each variant is generated by removing or replacing some components in FGCNN, which is described as follows:

\begin{itemize}
\item \textbf{Removing Raw Features}: In this variant, raw features are not input into \textit{Deep Classifier} and only the  generated new  features are fed to \emph{Deep Classifier}.
 \item \textbf{Removing New Features}: This variant removes \emph{Feature Generation}. Actually, it is equivalent to IPNN.
 \item \textbf{Applying MLP for \textit{Feature Generation}}: \emph{Feature Generation} is replaced by MLP which takes the neurons in each layer as new features. This variant uses the same hidden layers and generates the same number of features in each layer as FGCNN.
 \item \textbf{Removing Recombination Layer}: This variant is to evaluate how \emph{Recombination Layer} complements CNN to capture global feature interactions.  The \emph{Recombination Layer} is removed from \emph{Feature Generation}   so that the output of pooling layer serves as new features directly. The number of generated new features in each layer keeps the same as FGCNN.
% \item \textbf{Removing Factorization Machine}: removes the factorization machine Layer in the model.
% \item \textbf{Using One Embedding Matrix}: use the same embedding matrix for feature generation and DNN.
\end{itemize}

As shown in  Table~\ref{table:remove}, removing any component in FGCNN leads to a drop in performance. We have the following observations:

Firstly, FGCNN with raw features alone or with new generated features alone performs worse than the FGCNN with both of them. This result demonstrates that the generated features are good supplementaries to the original features, which are both crucial.

Secondly, the performance decrease of \textit{Appling MLP for Feature Generation}, compared to FGCNN, shows the ineffectiveness of MLP to identify the sparse but important feature combinations from a large number of parameters. CNN simplifies the learning difficulties by using the shared convolutional kernels, which has much fewer parameters to get the desired combinations. Moreover,  MLP recombines the neighbor feature interactions, which is extracted by CNN, to generate global feature interactions.

Thirdly, removing the Recombination Layer will limit the generated features as neighbor feature interactions. Since the arrangement order of raw features has no actual meanings in the CTR prediction task,  the restriction can lead to losing important non-neighbor feature interactions thus resulting in worse performance.
%Fourthly, \textit{Removing Factorization Machine} has the greatest impact on the performance, which shows the usefullness of Factorization Machine to capture explicit low-order feature interactions.
%Finally, if we only use the same embedding matrix for both feature generation part and Deep Predictive Learning part, the direction gradients from feature generation part and  DNN part may contradict which hinders the learning of FGCNN model. Therefore, using double embedding matrixs can be a good choice.

%Finally, the results of \textit{Replacing the convolution by Full Connection}
 %shows that although DNN can approximate any functions ideally, due to the large parameter space, it is usually hard to optimize. Therefore, the performance of \textit{Replacing the convolution by Full Connection} is relatively poor.  And it is even worse than \textit{Without New Features}, which shows new features generated by Full Connection are actually data noises.  We also have further experiments in the next section to show how the height of convolution kernel impacts (the bigger in height, the closer to Full Connection) the final performances, and it also demonstrates bigger heights often result in worse performances.




\subsection{Hyper-parameter Investigation (Q4)}

Our FGCNN model has several key hyper-parameters, i.e., the height of convolutional kernels, number of convolutional kernels, number of convolutional layers, and the number of kernels for generating new features. In this subsection, to study the impact of these hyper-parameters, we investigate how FGCNN model works by changing one hyper-parameter while fixing the others on Criteo and Huawei App Store datasets.

\subsubsection{Height of Convolutional Kernels}
 
The height of convolutional kernels controls the perception range of convolutional layers. The larger the height is, the more features are involved in the neighbor patterns, but more parameters need to be optimized. To investigate its impact, we increase the height from 2 to the number of fields of a dataset. As shown in the top of Figure~\ref{fig:param_all},
the performance generally ascends first and then descends as the height of convolutional kernels increases\footnote{Due to that \textit{Feature Generation} and \textit{Deep Classifier} interrelate with each other, the curve has some fluctuations.}.
\begin{figure}[t]
 \centering
 \includegraphics[width=0.45\textwidth,height=9cm]{parameter_all_odd.pdf}
 \vspace{-4ex}
 \caption{Parameter study of height of convolutional kernel, number of convolutional layers and number of  kernels for new features (from top to bottom)}
 \vspace{-3ex}
 \label{fig:param_all}
\end{figure}

% \begin{figure}[h]
%  \centering
%  \includegraphics[width=0.47\textwidth,height=3cm]{height_avazu_criteo.pdf}
%  \vspace{-3ex}
%  \caption{Height of Convolution Kernels}\label{fig:height}
%  \vspace{-3ex}
%  \label{height}
% \end{figure}
% \begin{figure}[h]
%  \centering
%  \includegraphics[width=0.47\textwidth,height=3cm]{layers_avazu_criteo.pdf}
%  % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
%  \vspace{-3ex}
%  \caption{Number of Convolution Layers}\label{fig:layers}
% \vspace{-3ex}
%  \label{layers}
% \end{figure}
% \begin{figure}[h]
%  \centering
%  \includegraphics[width=0.47\textwidth,height=3cm]{news_avazu_criteo.pdf}
%  % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
%  \vspace{-3ex}
%  \caption{Number of Kernels for New Features}\label{fig:new}
%  \vspace{-3ex}
%  \label{new}
% \end{figure}
The results show that as more features are involved in the convolutional kernels, higher-order feature interactions can be learned so that the performance increases. However, due to that useful feature interactions are usually sparse, larger heights can cause more difficulties to learn them effectively, leading to a decrease in performance. This observation is consistent with the finding in Section 3.4, i.e., the performance decreases in Appling MLP for Feature Generation.

\subsubsection{Number of Convolutional Layers}
As shown in  the middle of  Figure~\ref{fig:param_all}, as the number of convolutional layers increases, the performance of FGCNN is improved. Notice that more layers usually lead to higher-order feature interactions. Therefore, the result also shows the effectiveness of high-order feature interactions. 

\subsubsection{Number of Kernels for Generating New Features}
We study how the number of generated features affects the performance of FGCNN. We use the same number of kernels for new features in different \emph{Recombination Layers}.  As can be observed in the bottom of Figure~\ref{fig:param_all}, the performance is gradually improved with more features generated. The results verify our research idea that it is useful to identify the sparse but important feature interactions first, which can effectively reduce the learning difficulties of DNNs. However, the useful feature interactions can be sparse and limited. If too many  features are generated, the extra new features are noisy which will increase the learning difficulties of MLP,  leading to the decrease in the performance.

\subsection{Effect of Shuffling Order of Raw Features (Q5)}
\begin{figure}[h]
 \centering
\vspace{-2ex}
 \includegraphics[width=0.45\textwidth]{shuffle_criteo_company.pdf}%[width=0.49\textwidth,height=3cm]
 % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
 \vspace{-3ex}
 \caption{Shuffling the order of raw features}\label{fig:shuffle}
 \vspace{-3ex}
 \label{shuffle}
\end{figure}

As mentioned before, CNN is designed to capture local neighbor feature patterns so that it is sensitive to the arrangement order of raw features. In our FGCNN model, the design of Recombination Layer is to learn global feature interactions based on CNN's extracted local patterns. Intuitively, our model should have more stable performance than traditional CNN's structure if the order of raw features is shuffled. Therefore,  to verify it, we compare the performance of two cases: with/without Recombination Layer. The arrangement order of raw features is shuffled many times at random where the two compared cases are performed for the same shuffled arrangement order. 


As shown in  Figure~\ref{fig:shuffle}, the case with Recombination Layer achieves better and more stable performance than that of without Recombination Layer. It demonstrates that with the help of Recombination Layer, FGCNN can greatly reduce the side effects of changing the arrangement order of raw features, which also demonstrates the robustness of our model.
% \begin{figure}[h]
%  \centering
%  \includegraphics[width=0.47\textwidth]{kernels_avazu_criteo.pdf}
%  % height.jpg: 0x0 px, 0dpi, nanxnan cm, bb=
%  \caption{Number of Convolution Kernels}\label{fig:kernels}
%  \label{layers}
% \end{figure}






==> fgcnn www2019/introduction.tex <==
\section{Introduction}
\label{Introduction}

With the rapid development of the Internet and mobile devices, our daily activities connect closely to online services, such as online shopping, online news and videos, online social networks, and many more. Recommender systems are a powful information filter for guiding users to find the items of interest in a gigantic and rapidly expanding pool of candidates. As elaborated in~\cite{alphaNDCG}, if an IR system's response to each query is a ranking of documents in decreasing order of probability of relevance, the overall effectiveness of the system to its user will be maximized. With this principle, the prediction of Click-Through Rate (CTR) is crucial for recommender systems, where the task is to estimate the probability a user will click on a recommended item. In online advertising applications, which is a billion-dollar scenario, the ranking strategy of candidate advertisement is by CTR$\times$bid with ``bid'' being the benifit the system receives once the online advertisement is clicked. In such an application, the performance of CTR prediction models~\cite{pin,deepfm,din} is one of the key facors to boost the revenue of the system.

The key challenge for CTR prediction tasks is effectively modeling feature interactions. Despite their simplicity, generalized linear models, such as FTRL~\cite{ftrl}, have shown decent performance in practice. However, such models lack the ability to learn feature interactions, and a common practice is to manually include pairwise feature interactions in designing its feature space. To overcome this limitation, Factorization Machines (FM)~\cite{fm} are proposed to model pairwise feature interactions as inner product of latent vectors between features and show promising results.

As a powerful approach to learning feature representations, deep neural networks have achieved remarkable progress in computer vision~\cite{din,Huang2016Densely,Kaiming2015Deep,Szegedy2016Inception,Xie2017Aggregated} and natural language processing~\cite{Bahdanau2014Neural,Bordes2016Learning,Radford2017Learning,Vaswani2017Attention}. Being able to learn sophisticated feature interactions automatically, some deep learning models have been proposed for CTR predictions~\cite{pin,deepfm,xdeepfm,ccpm,afm,crossnet,din}, of which all feed raw features to deep neural network to learn feature interactions explicitly or implicitly. Theoretically, deep neural networks are able to learn arbitrary feature interactions (of the raw features) to fit the traning target, by approximating any mathmatical function given the raw features, however, it is quite difficult to learn such feature interactions effectively in practice~\cite{pin,Shalevshwartz2017Failures}. 

Observing such obstacle, Wide \& Deep Learning~\cite{cheng2016wide} leverages the expertise feature engineering by the \emph{wide} component to help learning sophisticated feature interactions automatically by the \emph{deep} component, as shown on the left hand side of Figure~\ref{fig:wide-deep}. Empirically, with the help of generating new features\footnote{Here, new features are the feature interactions of the original raw features. In the rest of this paper, we may use the term ``new features'' for the ease of presentation.} by the wide component, the Wide \& Deep Learning model improves the performance of deep neural network (i.e., the deep component of Wide \& Deep learning alone) significantly, more specifically, 0.6\% AUC improvement in offline test and 1\% CTR improvement in online test.

However, feature engineering (to generate new features) in the wide component of Wide \& Deep Learning is expensive and requires domain knowledge. It would be more effective and more efficient to generate such new features automatically by machine learning models, more generally, deep neural networks. Applying the automatically learning new features, our proposed general framework is presented on the right hand side of Figure~\ref{fig:wide-deep}\footnote{Ignore the text ``CNN'' in the red box in Figure~\ref{fig:wide-deep} for now.}. The orginal raw features are input into a machine learning model (represented by the red box in Figure~\ref{fig:wide-deep}), which generates new features, and then the original raw features and new generated features are combined and fed into the hidden layers of deep neural networks. Generating new features could expand the original feature space and identify useful feature interactions betweeen the original raw features, which reduces the learning difficulies of the hidden layers later and leads to better performance.

\begin{figure}[t]
 \includegraphics[width=0.5\textwidth]{FGCNN_wide_deep.pdf}
 \caption{Comparision Between our Model and Wide\&Deep Model}\label{fig:wide-deep}
\end{figure}

A straightforward method to generate new features is by Multi-Layer Perceptron (MLP). Useful feature interactions are usually sparse in the space of raw features~\cite{pin}, therefore it is difficult to identify such useful feature interactions via learning distinguishable weights among all the feature interactions, by applying MLP alone without any advanced network structure. For example, we have four user features: \textit{user.Name}, \textit{user.Age}, \textit{user.Height}, \textit{user.Gender} to predict whether a user will download a specific online game. Assume that the groundtruth is that the feature interaction between \textit{user.Age} and \textit{user.Gender} is the only signal that matters, so that an optimal model should identify this and only this feature interaction. When performing MLP with only one hidden layer, the optimal weights associated to the embeddings of \textit{user.Name} and \textit{user.ID} should be all 0's, which is fairly difficult to achieve. 

As an advanced network structure of deep nueral networks, Convolutional Neural Network (CNN), which consists of one or multiple kernels with shared weights to capture useful local patterns, has achived great improvement in the area of computer vision~\cite{Huang2016Densely} and natural language processing~\cite{Bahdanau2014Neural}. The case of shared weights alleviates optimization difficulty of the overall model, since there are less weights to optimize. Therefore CNN provides a potentially good solution to realize our idea, i.e., to learn use feature combinations with less weights. However, applying CNN directly results in unsatisfying performance as CNN is designed to generate neighbor patterns but there is usually no meaning of features' arrangement order in CTR prediction.
This is also the reason why there are very few research works to study CNN in CTR prediction task. For example, whether the arrangement order of features being \emph{(Name, Age, Height, Gender)} or \emph{(Age, Name, Height, Gender)} does not make any difference to discribe the semantics of a sample, which is completely different from the case of images and sentences (where the order of pixels and words are very important). In this work, to overcome this limitation when applying CNN to learn feature interactions, we perform CNN and MLP as complementory of each other: learning local neighbor feature interactions via CNN and learning global non-neighbor feature interactions by MLP, which will significantly reduce the number of weights and capture local-global feature interactions at the same time.

In this paper, we propose a new model for CTR prediction task, namely FGCNN (Feature Generation by Convolutional Neural Network). FGCNN can be decomposited to two parts: \emph{feature generation} and \emph{deep predictive learning}. The \emph{feature generation} aims to identify and generate new important features from the original raw features. To avoid learning too many weight parameters by applying MLP directly, we propose to use CNN and MLP as complementory of each other, to identify important feature interactions as the new generated features. More specifically, CNN is performed to learn local neighbor feature interactions, while MLP is applied to recombine CNN's learning pattern, so as to extract global non-neighbor patterns. With both orignal raw features and new generated features, the \emph{deep predictive learning} learns further interactions between all the features, in order to make accurate prediction. Any advanced network structure (such as xDeepFM~\cite{xdeepfm}, DeepFM~\cite{deepfm}, PIN~\cite{pin}) can be adopted as the second part of FGCNN (namely, deep predictive learning), therefore our model has good compatibility with the existing deep learning research works in recommender system. For the ease of illustration, in the main part of this paper, we will adopt IPNN model~\cite{pin} as deep predictive learning part of FGCNN, due to its good trade-off between model complexity and accuracy. To verify the compatibility of our model, the cases of adopting some other existing models as deep predictive learning of or model are also studied empirically.

To summarize, the main contributions of this paper can be highlighted as follows:

\begin{itemize}
\item In CTR prediction task, we identify an important direction, i.e., generating new features automatically before feeding into the predictive models, which could expand the original feature space and identify useful feature interactions between raw features to reduce the learning difficulies of the predictive models.
\item We propose FGCNN model, which consists of \emph{feature generation} and \emph{deep predictive learning}. Feature generation part generates global and local feature interactions as new features, by using CNN and MLP as complementory of each other. More specifically, CNN extracts local patterns with limited parameters to learn, while MLP extends CNN's learning results by extracting global feature interactions. Deep predictive learning part are utilized to learn further interactions between the original raw features and the new generated features (by feature generation part). We adopt IPNN model as deep predictive learning of FGCNN in the main part of this work, however, any advanced predictive model can be adopted, which shows the compatibility of our FGCNN model.
\item We conduct empirical experiment to show the superiority of FGCNN over eight state-of-the-art CTR predictive models on three large-scale datasets (including two public datasets and a private one). Besides, functionality of different components, effect of hyper parameters, and compatibility of our model are also studied in detail. 
\end{itemize}
\textcolor{red}{TBD: the organization of the paper ....}


==> fgcnn www2019/introduction_1023_huifeng.tex <==
\section{Introduction}
\label{Introduction}


Click-Through Rate (CTR) is a crucial task for recommender systems, which estimates the probability of a user to click on  a given item~\cite{pin,deepfm}. In an online advertising application, which is a billion-dollar scenario, the ranking strategy of candidate advertisements is by CTR$\times$bid where ``bid'' is the profit that the system receives once the advertisement is clicked on. In such applications, the performance of CTR prediction models~\cite{pin,deepfm,din} is one of the core factors determining system's revenue.
\begin{figure}[!t]
%\vspace{-1ex}
 \includegraphics[width=0.48\textwidth]{FGCNN_wide_deep.pdf}
 \vspace{-6ex}
 \caption{Comparision Between our Model and Wide \& Deep Model}\label{fig:wide-deep}
 \vspace{-3ex}
\end{figure}

The key challenge for CTR prediction tasks is to effectively model feature interactions. Generalized linear models, such as FTRL~\cite{ftrl}, perform well in practice, but these models lack the ability to learn feature interactions.
To overcome the limitation, Factorization Machine~\cite{fm} and its variants~\cite{ffm} are proposed to model pairwise feature interactions as the inner product of latent vectors and show promising results.
Recently, deep neural networks (DNN) have achieved remarkable progress in computer vision~
\cite{Kaiming2015Deep,Szegedy2016Inception} 
and natural language processing
~\cite{Bahdanau2014Neural,Vaswani2017Attention}. And some deep learning models have been proposed for CTR predictions, such as PIN~\cite{pin}, xDeepFM~\cite{xdeepfm} and etc.
%\cite{pin,deepfm,xdeepfm,ccpm,afm,crossnet,din}, 
Such models feed raw features to a deep neural network to learn feature interactions explicitly or implicitly. Theoretically, DNN is able to learn arbitrary feature interactions from the raw features. However, due to that useful interactions are ususally sparse compared with the combination space of raw features, it is of great difficulties to learn them effectively from a large number of parameters~\cite{pin,Shalevshwartz2017Failures}. 


Observing such difficulties, Wide \& Deep Learning~\cite{cheng2016wide} leverages feature engineering in the \emph{wide} component to help the learning of \emph{deep} component.  With the help of artificial features, the performance of deep component is improved significantly (0.6\% improvement on offline AUC and 1\% improvement on online CTR).
However, feature engineering can be expensive and requires domain knowledge. If we can generate sophisticated feature interactions automatically by machine learning models, it will be more practical and robust.

Therefore, as shown in Figure~\ref{fig:wide-deep}, we propose a general framework for automatical feature generation. 
Raw features are input into a machine learning model (represented by the red box in Figure~\ref{fig:wide-deep}) to identify and generate new features \footnote{Here, new features are the feature interactions of the raw features. In the rest of this paper, we may use the term ``new features'' for the ease of presentation.}. After that, the  raw features and the generated new features are combined and fed into a deep neural network.  The generated features are able to reduce the learning difficulties of deep models by capturing the sparse but important feature interactions in advance.

The most straightforward way for automatical feature generation is to perform Multi-Layer Perceptron (MLP\footnote{MLP is a neural network with several fully connected layers.}) and use the hidden neurons as the generated features. However, as mentioned above, due to that useful feature interactions are usually sparse~\cite{pin}, it is rather difficult for MLP to learn such interactions from a huge parameter space. For example, suppose we have four user features: \textit{Name}, \textit{Age}, \textit{Height}, \textit{Gender} to predict whether a user will download an online game. Assume that  the feature interaction between \textit{Age} and \textit{Gender} is the only signal that matters, so that an optimal model should identify this and only this feature interaction. When performing MLP with only one hidden layer, the optimal weights associated to the embeddings of \textit{Name} and \textit{Height} should be all 0's, which is fairly difficult to achieve. 

As an advanced neural network structure, Convolutional Neural Network (CNN) %, which consists of many kernels with shared weights to capture useful local patterns,
has achieved great success in the area of computer vision~\cite{Huang2016Densely} and natural language processing~\cite{Bahdanau2014Neural}. In CNN, the design of shared weights and pooling mechanism greatly reduces the number of parameters needed to find important local patterns and it will alleviate the optimization difficulties of  later MLP structures. Therefore, CNN provides a potentially good solution to realize our idea (identify the sparse but important feature interactions). However, applying CNN  directly could result in unsatisfactory performance. In CTR prediction, different arrange orders of original features do not have different meanings. For example, whether the arrangement order of features being \emph{(Name, Age, Height, Gender)} or \emph{(Age, Name, Height, Gender)} does not make any difference to describe the semantics of a sample, which is completely different from the case of images and sentences. If we only use the neighbor patterns extracted by CNN, many useful global feature interactions will be lost.
This is also why CNN models do not perform well for CTR prediction task. 
To overcome this limitation, we perform CNN and MLP, which complement each other, to learn global-local feature interactions for feature generation.%, which not only leverages the strength of CNN (fewer parameters to optimize) and MLP (global interactions) but also avoid the weakness of them (CNN: only learn local interactions, MLP: too many paramters).

In this paper, we propose a new model for CTR prediction task, namely Feature Generation by Convolutional Neural Network (FGCNN), which consists of two components: \emph{Feature Generation} and \emph{Deep Classifier}. 
In \emph{Feature Generation}, a CNN+MLP structure is designed to identify and generate new important features from raw features. More specifically, CNN is performed to learn neighbor feature interactions, while MLP is applied to recombine them  to extract global feature interactions. After \emph{Feature Generation}, the feature space can be augmented by combining raw features and new features.
In \emph{Deep Classifier}, almost all state-of-the-art network structures (such as PIN~\cite{pin}, xDeepFM~\cite{xdeepfm}, DeepFM~\cite{deepfm}) can be adopted. Therefore, our model has good compatibility with the state-of-the-art models in recommender systems. 
For the ease of illustration, we will adopt IPNN model~\cite{pin,pnn} as \emph{Deep Classifier} in FGCNN, due to its good trade-off between model complexity and accuracy.  Experimental results in three large-scale datasets show that FGCNN significantly outperforms nine state-of-the-art models, demonstrating the effectiveness of FGCNN. While adopting other models in \emph{Deep Classifier}, better performance is always achieved, which shows the usefulness of the generated features. Step-by-step analyses show that each component in FGCNN contributes to the final performance. Compared with traditional CNN structure, our CNN+MLP structure performs better and more stable when the order of raw features changes, which demonstrates the robustness of FGCNN.

To summarize, the main contributions of this paper can be highlighted as follows:
\begin{itemize}
\vspace{-1ex}
\item   An important direction is identified for CTR prediction: it is both necessary and useful to reduce the optimization difficulties of deep learning models by automatically generating important features in advance.

\item We propose a new model-FGCNN for automatical feature generation and classification, which consists of two components: \emph{Feature Generation} and \emph{Deep Classifier}. \emph{Feature Generation} leverages CNN and MLP, which complement each other, to  identify the important but sparse features. Moreover, almost all other CTR models can be applied in \emph{Deep Classifier} to learn and predict based on the generated and raw features.

\item Experiments on three large-scale datasets demonstrate the overall effectiveness of FGCNN model. When the generated features are used in other models, better performance is always achieved, which shows the great compatibility and robustness of our FGCNN model.
\end{itemize}
The rest of this paper is organized as follows: Section 2 presents the proposed FGCNN model in detail. Experimental results will be shown and discussed in Section 3. Related works will be introduced in Section 4. Section 5 concludes the paper. 
%\textcolor{red}{TBD: the organization of the paper ....}


==> fgcnn www2019/model.tex <==
\section{Feature Generation by Convolution Neural Network Model}
\newpage
\subsection{overview}
In this section, we will introduce the proposed Feature Generation by Convolution Neural Network Model. As shown in Figure ~\ref{fig:model_overview}, the model consists of two components:
\textcolor{red}{\textit{Feature Generation}  better name Convolutional Feature Generation ?} and \textit{FM and Deep Component}.
The first component focus on identifying usefull local and global patterns to generate new features while the second part works on using Factorization Machine and Deep Neural Network to learn implicit and explict feature interactions. Each componet will be detailed in the following parts.

\subsection{Feature Generation}
As mentioned in Section~\ref{Introduction},  although MLP can approximate learn any specific feature interactions theoratically, it is quite difficult to learn in practice~\cite{Shalevshwartz2017Failures}. One possible reason is that usefull cross features are usually sparse in the combination space of raw features and it is challenging for MLP to identify important feature combinations while disregarding useless combinations. Many data scientists tries to extract useful features from raw data first based on their domain knowledge and feed the extracted features and  raw features to DNNs such as Wide\&Deep Learning. And such methods do improve the performance of DNNs, which demonstrates the effectiveness of identifying important features before using DNNs. However, feature engineering is expensive and requires domain knowledge. Therefore, we wonder whether we can use Neural Network to automatically identify some cross features as feature engineering does and then use DNN to learn further feature interactions. 

 Simply using fully connected neural network can not works well for feature combination idenfication, since the optimal combinations is sparse and it is hard to learn the weights of unrelated features(usually the weights of their embedding) as zero during optimization. For example, we want to use the embedding of four features -\textbf{(User.Name, User.ID, User.Age, User.Gender)} to predict whether a user will download a game Application. In practice, only the combination of \textbf{Age} and \textbf{Gender(Age$<$30 and gender$=$Male) }could contribute to the prediction. And it could be quite challenging in multi-layer perceptron to learn the optimal weights as the number of unrelated features and the size of feature's embedding increase.  
 
 Convolutional Neural Network(CNN) recently has achieved great progress in the area of computer vision and natural language processing . The main advanteges of CNN is that the convolution kernel with shared weights in the convolution kernel can capture important local patterns and pooling is used to reduce the input demension. Shared weight means less parameters which usually lead to simplified optimization difficulties for find optimal combination weights. The nature of CNN matches our initial intention of discovering important feature interactions from a large combination space.  However, unlike sentences or images, different arrangement of features does not change meaning of a sample in the area of Click-Through Rate Prediction. For example, whether \textbf{(User.Name, User.ID, User.Age, User.Gender)} or \textbf{(User.Gender, User.ID, User.Age, User.Name)} is actually the same to portray a given user. Due to this, CNN is criticised of only learning the feature interactions between neighbor features, which also limited the use of CNN in this area.
 
 \begin{figure}[t]
  \includegraphics[width=0.48\textwidth]{CNN+Pooling+MLP.pdf}
  \caption{How CNN+Pooling+MLP captures non-neighbor interactions to generate new features}
  \label{fig:CNN+Pooling+MLP}
 \end{figure}

 In this paper, CNN+Pooling+Recombination is proposed to overcome the weakness of CNN, which is able to capture neighbor and non-neighbor feature interactions. Figure~\ref{fig:CNN+Pooling+MLP} shows an example of how CNN+Poooling+Recombination works. As it shows, the structure not only leverages the benifits of Convolution layer and Pooling Layer to learn feature interactions in a neighboring region, but also has the ability to capture the interactions of non-neighbor features. Moreover, with the height in the convolution kernel increases, it is possible to learn high-order feature interactions.

 In the following parts, we will detail the structure seperately:
 
 
 \subsubsection{Embedding Layer}
 In most CTR Prediction tasks, data are collected in a multi-field categorical form. And each data instance is transformed into a high-dimensional sparse(binary) vector via one-hot encoding~\cite{He2014Practical}.For example,
\textbf{(Gender=Male, ID=123, Age=18, Name=Mary)} can be representated as:
 \begin{equation}
  \underbrace{(0,1)}_{\text{Gender=Male}}\underbrace{ (0,...1,0,0)}_{\text{ID=123}}\underbrace{(0,1,...0,0)}_{\text{Age=18}}\underbrace{(1,0,0,..,0)}_{\text{Name=Mary}}
 \end{equation}

 Next, each one entry $i (1 \le i \le n)$ will be representated by a low dimensional vector $e_i \in R^{1*k}$, where $n$ is the number of fields and $k$ is embedding size. 
 Then, all embedding vector $e_i( 1 \le i \le n)$ will be concatenated as a embedding matrix $E \in R^{n*k}$.   
 In this paper, since the embedding matrix $E$ will be used in both feature genenration and DNNs, to reduce the inconsistency in the direction of gradients, we introduce another embedding  matrix $E' \in R^{n*k}$ for accepting gradient updates from DNN while  $E$ accepts gradient updates from feature genenration.\label{embedding}
 
 
 
 \subsubsection{Convolution Layer}
 After the embedding layer, we can get the embedding matrix $E = (e_1^T, e_2^T,...e_n^T)^T \in R^{n*k}$ of raw features, where $n$ is the number of fields and $k$ is embedding size. The convolution layer is obtained by convolving a matrix $\mathcal{W} \in R^{H*1*f}$ with non-linear activation functions($H$ is the height of convolution matrix and $f$ is the number of feature maps). Suppose the output of Convolution Layer is $F \in R^{n*k*f}$:
\begin{align}
 F_{i,j,m} &= tanh(\sum_{h=1}^H  E_{i-h+1,j}*\mathcal{W}_{h,0,m})\\
 tanh(x) &= \frac{exp(x)-exp(-x)}{exp(x)+exp(-x)}
\end{align}
Note: the above equation excludes padding while actual model uses it. 
 \subsubsection{Pooling Layer}
 After getting the result $F \in R^{n*k*f}$ of Convolution Layer, max pooling is applied to reduce the  number of  paramenters. In our model, $p*1$ is the preferred kernel. Suppose the output in this layer is $\mathbb{F} \in R^{(n/p)*k*f}$:
 \begin{equation}
  \mathbb{F}_{i,j,m} = max(F_{i*p,j,m},F_{i*p+1,j,m},..., F_{i*p+p-1,j,m})
 \end{equation}
 \subsubsection{Recombination Layer}
 After Convolution Layer and Pooling Layer, $\mathbb{F}$ already contains information in the neighboring fields. Due to that important feature interactions is usually sparse and the arrangement of raw features is quite random, some feature interactions can be losed if using $\mathbb{F}$ as the feature interaction results and generating features. Therefore, we introduce a fully connected layer to recombine the interactions from different positions.  Suppose the weights is $\mathbb{W}\in R^{(n/p*k*f) * (N *k)}$ and the bias is ${b} \in R^{(N*k)}$ where $n$ is the field num, $p$ is the pooling kernel size, $k$ is the embed size, $f$ is the number of feature maps and $N$ is the number of new features.  The new features can be represented as $\mathbb{N} \in R^{N*k}$:
 \begin{align}
  &\mathbb{N} = tanh(\mathbb{F}*\mathbb{W} + {b}) 
 \end{align}

 So far, new features are generated among patterns from different Convolution+Pooling results. Furthermore, the Convolution+Pooling+Recombination operations can be repeated many times to yield
 different orders of feature interactions.
 Recall the whole process of Convolution+Pooling+Recombination, Convolution Layer enumurates some possible feature interactions and Pooling Layer filters useless iteractions while Recombination Layer recombines the information in each corner to generate new features. 
 
Old feature and new features can be concatenated as：
\begin{align}
\mathbb{E}&=(E'^T,\mathbb{N}^T)^T 
\end{align}
where $E'$ is the embedding matrix for DNN(see Section ~\ref{embedding}). The augmented feature set can be further leveraged by different Deep Models.

Unlike traditional models only use Deep Neural Network to learn implicit and explicit feature interaction and make final predictions, our method try to identify some important patterns to generate new feature first to reduce the learning difficulties in DNN. This is also the major difference from traditional models.
\subsection{FM and Deep Component}
After the feature generation process by CNN, raw features and new features are concatenated as $\mathbb{E}=(e_1^T,e_2^T,...,e_{N+n}^T)^T \in R^{(N+n)*k}$ where $N$ is the number of new features, $n$ is the number of raw features and $k$ is embedding size. The second part adopts the structure of IPNN model~\cite{pin}, which involves a Factorization Machine~\cite{Rendle2011Factorization} and a Multi-Layer Perceptron(MLP) to make a final predictions. The main reason for choosing IPNN rather than other models(such as xDeepFM, deepFM, and PIN) is that IPNN outperforms other models except PIN in many datasets~\cite{pin} and IPNN is more suitable than PIN when the number of input features is big since IPNN use inner-product to model pairwise interactions and PIN use Micro-Network to model them.
\subsubsection{Factorization Machine Component}
Factorization Machine is proposed in ~\cite{Rendle2011Factorization} to learn feature interactions for recommendation. FM models pairwise(order-2) feature interactions as inner product of feature's embeddings~\cite{deepfm}. In our model, we use the inner product of different features to get explicit feature interactions. The output of FM component $R_{fm}$ can be reformulated as:
\begin{equation}
    R_{fm} = (<\mathbb{E}_{1},\mathbb{E}_2>,<\mathbb{E}_i, \mathbb{E}_j>,...<\mathbb{E}_{N+n-1},\mathbb{E}_{N+n}>)
\end{equation}
The total interactions in FM component is $\frac{(N+n)*(N+n-1)}{2}$. 
\subsubsection{Deep Component}
As we get the FM results and embedding matrix of raw features and generated features, the two results is fed into Multi-Layer-Perceptron to learn implicit feature Interactions. Suppose input for the i-th hidden layer is $I_i$ and the output for the i-th hidden layer is $O_i$:
\begin{align}
 &I_0 = (R_{fm}, \mathbb{E})\\
 &O_i = relu(I_{i}*W_i+b_i) \\
 &I_{i+1} = O_{i}
\end{align}
where $W_i$ is the weight matrix for layer-$i$ and $b$ is the bias. For the last layer, we will make final predictions:
\begin{equation}
 y = sigmoid(I_i*W_i+b_i)
\end{equation}

\subsubsection{Batch Normalization}
Batch Normalization(BN) is proposed in~\cite{BN} to solve covariate shift and accelerate DNN training and it works quite well in our FGCNN model.

BN normalizes activations $w^Tx$ using statistics within a mini-batch
\begin{equation}
 BN(w^Tx) = \frac{w^Tx-avg_i(w^Tx)}{std_i(w^Tx)} *g +b
\end{equation} where $g$ and $b$ scale and shift the normalized values. 

In the FGCNN model, Batch Normalization is applied before each activation function to accelerate model training.
\subsubsection{Objective Function}
The objective function in the   FGCNN model is to minimize cross entropy, which is defined as:
\begin{equation}
 \mathcal{L}(y,\sigma(\hat{y})) = -y log(\sigma{\hat(y)})-(1-y)log(1-\sigma(\hat{y}))
\end{equation}
where $y \in \{0,1\}$ is the label and $\sigma(\hat{y}) \in (0,1)$ is the predicted probability of $y=1$.


\subsection{Complexity Analysis}
We analyse our proposed FGCNN model to study the model complexity. The notations that will be used are summerized in Table~\ref{notations}. \textcolor{red}{summarize the complixities}
\begin{table}[h]
\caption{Notations}
\label{notations}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|l|l|}
\hline
Parameter & Meaning \\ \hline
$k$ & embed size \\ \hline
$n$ & field num \\ \hline
$l$ & num of convolution layers \\ \hline
$m$ & number of hidden layers \\ \hline
$h_i$ & height of conv kernel in the i-th conv layer \\ \hline
$p$ & pooling height(width=1) \\ \hline
$f_i$ & feature map num in the i-th conv layer \\ \hline
$N_i$ & new feature num in the i-th recombination layer \\ \hline
$H_i$ & hidden neurons in the i-th Hidden layer \\ \hline

\end{tabular}}
\end{table}
\subsubsection{Space Complexities}
In the i-th convolution layer, there are total $h_if_{i-1}f_i$ parameters for conv matrix. And in the i-th pooling layer, the number of neurons in pooling output is $n/p^ikf_i$. Therefore, for the i-th recombination Layer to generate $N_i$ new features, the parameter for the weight matrix is $n/p^ikf_i N_ik$(since the number of bias is relatively small, we do not discuss it here). In the convolution+pooling+recombination Layer, the number of total parameters $p_1$is :
\begin{equation}
p_1 = \sum_{i=1}^{l} h_if_{i-1}f_i+ n/p^ik^2f_iN_i
\end{equation}
After the feature generating process, we can get $T = n+\sum_{i=0}^{l} N_i$ in total.
Notice that $l$ is usually less than 5 and $k^2$ is often bigger than $f_{i-1}$ meanwhile $f_i/p^i$ is usually a small number, the total parameters in the feature generating process is $p_1 = O(\sum_{i=0}^{l-1} n/p^ik^2f_i N_i) = O(\sum_{i=0}^{l-1}nk^2N_i) = O(nk^2T)$.

 For the first hidden layer, the number of parameters in the weight matrix is $(T(T-1)/2+Tk)H_i$. In the i-th layer, the number of parameters is $H_(i-1)H_i$. Total parameters in the FM and Deep Component is 
\begin{equation}
 p_2 = \frac{T(T-1)+2Tk}{2}H_0 + \sum_{i=1}^{m} H_iH_{i-1}
\end{equation}
$p_2$ can be simplified as  $O(T^2H_0+\sum_{i=1}^mH_iH_{i-1})$. Therefore, the space complexities of FGCNN is $O(T^2H_0+nk^2T+\sum_{i=1}^mH_iH_{i-1})$, which is dominated by the number of generated features, the number of hidden neurons and the size of embedding.
\subsubsection{Time Complexities}
In the i-th convolution layer, the output demension is $n/p^ikf_i$ and each point is calculated from $h_if_{i-1}$ data points. Therefore, the time complexity in the i-th convolution layer is $n/p^ikf_ih_if_{i-1} = O(nkf_ih_i)$ . In the pooling layer, we just need to scan the output of convolution layer. So the time complexity in the i-th pooling layer is $n/p^ikf_i$. In the i-th recombination layer,  the time complexity is $n/p^ikf_iN_ik = O(nkN_ik)$. The total time complexity during the feature generating process is
\begin{equation}
 t_1 = \sum_{i=1}^l O(nkf_ih_i) + O(nkN_i*k) = O(nTk^2)+ \sum_{i=1}^l O(nkf_ih_i)
\end{equation} where $T = n+\sum_{i=0}^{l} N_i$

In the FM layer, the time complexity to calculate pairwise inner product is $\frac{T(T-1)k}{2}$. In the first hidden layer, the number of input neurons is $T(T-1)/2+Tk$ while the number of output units is $H_0$. Therefore, the time complexity of the first hidden layer is $O(T^2H_0)$. For the other hidden layers, the time complexity is $O(H_iH_{i-1})$. So, the total complexity in the FM and Deep Component is
\begin{equation}
 t_2 = O(T^2H_0)+\sum_{i=1} O(H_iH_{i-1}) = O(T^2H_0+\sum_{i=1} H_iH_{i-1})
\end{equation}
The total time complexity for FGCNN model is $t_1+t_2 = O(T^2H_0+nTk^2+\sum_{i=1}^lnkf_ih_i+\sum_{i=1}H_iH_{i-1})$ which is dominated by the number of generated feature, the number of neurons in first hidden layer, embed size and  convolutional parameters. 


==> fgcnn www2019/model_1025_huifeng.tex <==
\section{Feature Generation by Convolution Neural Network Model}

\subsection{overview}

In this section, we will introduce the proposed Feature Generation by Convolutional Neural Network (FGCNN in short) model.
The notations that will be used are summerized in Table~\ref{notations}.
\begin{table}[!t]
\caption{Notations}
\label{notations}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|c|l|}
\hline
Parameter & Meaning \\ \hline
$k$ & embedding size \\ \hline
$n$ & the number of fields\\ \hline
$l$ & the number of convolution layers \\ \hline
$m$ & the number of hidden layers \\ \hline
$h^i$ & the height of convolutional kernel in the i-th convolutional layer \\ \hline
$p^i$ & pooling height(width=1) of i-th convolution layer \\ \hline
$E^i$ & the input of the i-th convolutional layer \\ \hline
$f^i$ & the number of feature maps in the i-th convolutional layer \\ \hline
$FC^i$ & the output of the i-th convolutional layer \\ \hline
$N^i$ & the number of new features in the i-th recombination layer \\ \hline
$FP^i$ & the output of the i-th pooling layer \\ \hline
$H_i$ & the neurons in the i-th hidden layer \\ \hline

\end{tabular}}
\end{table}
As shown in Figure ~\ref{fig:model_overview}, the model consists of three components: \textcolor{red}{Feature Embedding}, \textcolor{red}{\textit{Feature Generation}} and \textcolor{red}{\textit{Deep  Predictive Learning}}. Specifically, the second component focuses on identifying useful local and global patterns to generate new features as a complementary for raw features, while the third part works on capturing feature interactions based on the augmented feature space implicitly and explicitly through a deep predictive learning model. The details of these components are introduced in the following.

\subsection{Feature Embedding}\label{embedding}
In computer vision and natural language processing, the input data are usually images and sentences, which are known to be dense, so DNNs can be applied directly on the raw features. However, in most CTR Prediction tasks, the input are sparse and collected in a multi-field categorical form, which is widely used in related works~\cite{xdeepfm,pin,deepfm}. Each data instance is transformed into a high-dimensional sparse(binary) vector via one-hot encoding~\cite{He2014Practical}. For example,
\textbf{(Gender=Male, ID=123, Age=18, Name=Mary)} can be representated as:
 \begin{equation}
  \underbrace{(0,1)}_{\text{Gender=Male}}\underbrace{ (0,...1,0,0)}_{\text{ID=123}}\underbrace{(0,1,...0,0)}_{\text{Age=18}}\underbrace{(1,0,0,..,0)}_{\text{Name=Mary}}
 \end{equation}

An embedding layer is applied to compress the raw features to the dense real-value vectors. The feature embedding is used as the field embedding if the field is univalent. Take the above instance as an example, the embedding of feature ``Male'' is taken as the embedding of field ``Gender''. Similar with \cite{xdeepfm}, if the field is multivalent, the sum of feature embedding is used as the field embedding.

Specifically, each entry $i (1 \le i \le n)$ will be represented as a low dimensional vector $e_i \in R^{1*k}$, where $n$ is the number of fields and $k$ is embedding size.
Then, all embedding vector $e_i( 1 \le i \le n)$ will be concatenated as a embedding matrix $E=(e_1^T, e_2^T, ..., e_n^T)^T$, where $E \in R^{n*k}$.
In this paper, the embedding matrix $E$ will be used in both feature generation and deep predictive learning. To reduce the inconsistency in the direction of gradients when updating parameters, another embedding  matrix $E' \in R^{n*k}$  is introduced and fed into deep predictive learning model. In other words, $E'$ for deep predictive learning model while $E$ for feature generation component.
\subsection{Feature Generation}
In practice, the ability of learning sophisticated feature interactions is critical for CTR models. Although MLP is able to approximate any specific feature interaction theoretically, it is difficult to learn in practice because the combination space of raw features is too sparse. It is challenging for MLP to identify important feature interactions while disregarding useless combinations. For the purpose of capturing more meaningful feature interaction, Wide \& Deep model utilizes the manually designed features as a complementary of raw features. As a result, both offline AUC and online CTR are improved. However, it is impractical because designing manually features is expensive and requires domain knowledge. Therefore, we wonder whether we can design a feature generation model to automatically identify some cross features as feature engineering does.

Due to the ability of feature representation, deep learning promotes the progress in many fields related to machine learning. However, simply using fully connected neural network can not works well for feature combination identification. Since the optimal combinations is sparse and it is hard to learn the weights of unrelated features (usually the weights of their embedding) as zero during optimization. For example, we want to use the embedding of four features -\textbf{(User.Name, User.ID, User.Age, User.Gender)} to predict whether a user will download a game Application. In practice, only the combination of \textbf{Age} and \textbf{Gender(Age$<$30 and gender$=$Male) }could contribute to the prediction.


Recently, Convolutional Neural Network (CNN) has achieved great progress in the area of computer vision and natural language processing. CNN has many advantages, two of which are more important: (1) the convolutional kernel with shared weights can capture important local patterns; (2) the pooling technique is used to reduce the input dimension and select meaningful features. In addition, shared weight means less parameters which usually lead to easier learning process and lower optimization difficulty. So CNN is suitable for discovering important feature interactions from a large combination space, which is matching our initial intention. Unfortunately, unlike sentences and images, different arrangement of features does not change the meaning of a sample in the area of CTR prediction. For example, whether \textbf{(User.Name, User.ID, User.Age, User.Gender)} or \textbf{(User.Gender, User.ID, User.Age, User.Name)} is actually the same to portray a given user. Therefore, CNN is criticised of only learning the feature interactions between neighbor features, which also limited the use of CNN in this area.


 \begin{figure}[t]
  \includegraphics[width=0.48\textwidth]{CNN+Pooling+MLP.pdf}
  \caption{How CNN+Pooling+MLP captures non-neighbor interactions to generate new features}
  \label{fig:CNN+Pooling+MLP}
 \end{figure}

In order to overcome this limitation to take the advantage of CNN to capture neighbor and non-neighbor feature interactions, a CNN+Pooling+Recombination structure is proposed in this paper. Figure~\ref{fig:CNN+Pooling+MLP} shows an example of how CNN+Poooling+Recombination works. As it shows, the structure not only leverages the benefits of convolution layer and pooling layer to learn feature interactions in a neighboring region, but also has the ability to capture the interactions of non-neighbor features. Moreover, with the height in the convolution kernel increases, it is possible to learn high-order feature interactions.

 In the following parts, we will detail the structure separately:





 \subsubsection{Convolution Layer}
 After the embedding layer, we can get the embedding matrix $E = (e_1^T, e_2^T,...e_n^T)^T \in R^{n*k}$ of raw features, where $n$ is the number of fields and $k$ is embedding size. For convenience, rename the embedding matrix as $E^{1}$.
 To capture the local neighbor feature interactions, the convolution layer is obtained by convolving a matrix $\mathcal{W} \in R^{H*1*f^{1}}$ with non-linear activation functions($H$ is the height of convolution matrix and $f^1$ is the number of feature maps in the first convolution layer). Suppose the output of the first Convolution Layer is denoted as $FC^{1} \in R^{n*k*f^1}$, we can get:
\begin{align}
 FC^{1}_{i,j,f^{1}_{o_1}} &= tanh(\sum_{h=1}^H  E^{1}_{i-h+1,j}*\mathcal{W}_{h,0,f^{1}_{o_1}})\\
 tanh(x) &= \frac{exp(x)-exp(-x)}{exp(x)+exp(-x)}
\end{align}
where $f^{1}_{o_1}$ denotes the $o_1-{th}$ kernel in the first convolution layer. Note: the above equation excludes padding while actual model uses it.
 \subsubsection{Pooling Layer}
 After getting the result $FC^1$ of the first Convolution Layer, max pooling is applied to seize the most important feature interactions and reduce the number of  parameters. In our model, $p^1*1$ is the preferred kernel of the first pooling layer. Suppose the output in this layer is $\mathbb{FP}^1 \in R^{(n/p^1)*k*f}$:
 \begin{equation}
  \mathbb{FP}^1_{i,j,f^1_{o_1}} = max(FC^1_{i*p^1,j,f^1_{o_1}},..., FC^1_{i*p^1+p^1-1,j,f^1_{o_1}})
 \end{equation}
 \subsubsection{Recombination Layer}
 After Convolution Layer and Pooling Layer, $\mathbb{FP}^1$ already contains information in the neighboring fields. Due to that important feature interactions is usually sparse and the arrangement of raw features is quite random, some feature interactions might be ignored if using $\mathbb{FP}^1$ as the feature interaction results and generating features. Therefore, we introduce a fully connected layer to recombine the interactions from different positions. Specifically, set the weight matrix as $\mathbb{W}^1\in R^{(n/p^1*k*f^1) * (N^1 *k)}$ and the bias as ${b^1} \in R^{(N^1*k)}$, where $n$ is the field num and $p^1$ is the size of pooling kernel in the first pooling layer, $k$ is the embedding size, $f^1$ is the number of feature maps in first convolution layer and $N^1$ is the number of new features after one time convolution and pooling.  The new features can be represented as $\mathbb{N}^1 \in R^{N^1*k}$:
 \begin{align}
  &\mathbb{N}^1 = tanh(\mathbb{FP}^1*\mathbb{W}^1 + {b^1})
 \end{align}
\subsubsection{Concatenation}
 So far, new features are generated among patterns from different Convolution+Pooling results. Furthermore, the Convolution+Pooling+Recombination operations can be repeated many times to yield different orders of feature interactions. Recall the whole process of Convolution+Pooling+Recombination, Convolution Layer enumerates some possible feature interactions and Pooling Layer filters useless interactions while Recombination Layer recombines the information in each corner to generate new features. If we set the number of convolution layers as $l$, new features $\mathbb{N} \in R^{N*k}$, where $N=\sum_{i=1}^{l}{N^i}$, are generated by Feature Generation component:
 \textcolor{red}{pls. modify the mistake in the following equation}
 \begin{align}
\mathbb{N}&= (\mathbb{N}^1, \mathbb{N}^2, ..., \mathbb{N}^l)
 \end{align}
Particularly,
\begin{align}
 \mathbb{N}^l &= tanh(\mathbb{FP}^l*\mathbb{W}^l + {b^l})
 \end{align}
 \begin{align}
  \mathbb{FP}^l_{i,j,f^l_{o_l}} &= max(FC^{l}_{i*p^l,j,f^l_{o_l}},..., FC^l_{i*p^l+p^l-1,j,f^l_{o_l}})
  \end{align}
  \begin{align}
 FC^{l}_{i,j,f^l_{o_l}} &= tanh(\sum_{o_{l-1}=1}^{f^{l-1}}\sum_{h=1}^H  E^{l}_{i-h+1,j,f^{l-1}_{o_{l-1}}}*\mathcal{W}_{h,0,f^{l}_{o_l}})
\end{align}
where $\mathbb{W}_l$ is the weight matrix and ${b_l}$ is bias in the $l_{th}$ recombination layer, $\mathbb{FP}^l$ is the output of $l_{th}$ pooling layer, $FC^{l}$ is the output of $l_{th}$ convolution layer, $f^l_{o_l}$ is the $o_l$-th kernel in $l$-th convolution layer, and $E^{l}$ is $\mathbb{FP}^{l-1}$.
Then, old feature and new features can be concatenated as£º
\begin{align}
\mathbb{E}&=(E'^T,\mathbb{N}^T)^T
\end{align}
where $E'$ is the embedding matrix for DNN(see Section ~\ref{embedding}). The augmented feature set can be further leveraged by different Deep Models.

Unlike traditional models only use Deep Neural Network to learn implicit and explicit feature interaction and make final predictions, our method try to identify some important patterns to generate new feature first to reduce the learning difficulties in DNN. This is also the major difference from traditional models.
\subsection{Deep Predictive Learning}
After the feature generation process by CNN, raw features and new features are concatenated as the augmented embedding matrix $\mathbb{E} \in R^{(N+n)*k}$ where $N$ is the number of new features, $n$ is the number of raw features and $k$ is embedding size. In order to learn the feature interactions implicitly and explicitly, deep predictive learning model adopts the structure of IPNN model~\cite{pin}, which involves a Factorization Machine~\cite{Rendle2011Factorization} and a Multi-Layer Perceptron(MLP) to make a final predictions.
In fact, IPNN outperforms other models except PIN in many datasets~\cite{pin}. The motivation behind our selection is that IPNN is more efficient than PIN since IPNN use inner-product to model pairwise interactions and PIN use Micro-Network to model them.
\subsubsection{Factorization Machine Component}
Factorization Machine is proposed in ~\cite{Rendle2011Factorization} to learn feature interactions for recommendation. FM models pairwise (order-2) feature interactions as inner product of feature's embeddings~\cite{deepfm}. In our model, we use the inner product of different features to get explicit feature interactions. The output of FM component $R_{fm}$ can be reformulated as:
\begin{equation}
    R_{fm} = (<\mathbb{E}_{1},\mathbb{E}_2>,<\mathbb{E}_i, \mathbb{E}_j>,...<\mathbb{E}_{N+n-1},\mathbb{E}_{N+n}>)
\end{equation}
where $\mathbb{E}_{i}$ is the embedding of the $i$-th vector, $<a,b>$ means the inner product of vector a and b and the number of interactions in FM component is $\frac{(N+n)*(N+n-1)}{2}$.
\subsubsection{Deep Component}
As we get the FM results and the augmented embedding matrix $\mathbb{E}$, the two results are fed into Multi-Layer-Perceptron to learn implicit feature Interactions. Suppose input for the i-th hidden layer is $I_i$ and the output for the i-th hidden layer is $O_i$:
\begin{align}
 &I_0 = (R_{fm}, flatten(\mathbb{E}))\\
 &O_i = relu(I_{i}*W_i+b_i) \\
 &I_{i+1} = O_{i}
\end{align}
where $W_i$ is the weight matrix for layer-$i$ and $b$ is the bias. For the last layer, we will make final predictions:
\begin{equation}
 y = sigmoid(I_i*W_i+b_i)
\end{equation}

\subsubsection{Batch Normalization}
Batch Normalization(BN) is proposed in~\cite{BN} to solve covariant shift and accelerate DNN training and it works quite well in our FGCNN model.

BN normalizes activations $w^Tx$ using statistics within a mini-batch
\begin{equation}
 BN(w^Tx) = \frac{w^Tx-avg_i(w^Tx)}{std_i(w^Tx)} *g +b
\end{equation} where $g$ and $b$ scale and shift the normalized values.

In the FGCNN model, Batch Normalization is applied before each activation function to accelerate model training.
\subsubsection{Objective Function}
The objective function in the   FGCNN model is to minimize cross entropy, which is defined as:
\begin{equation}
 \mathcal{L}(y,\sigma(\hat{y})) = -y log(\sigma{\hat(y)})-(1-y)log(1-\sigma(\hat{y}))
\end{equation}
where $y \in \{0,1\}$ is the label and $\sigma(\hat{y}) \in (0,1)$ is the predicted probability of $y=1$.


\subsection{Complexity Analysis}
In this section, we analyse the space and time complexities of the proposed FGCNN model.  \textcolor{red}{summarize the complexities}
\subsubsection{Space Complexities}
The space complexities include three aspects, namely feature embedding, feature generation and deep predictive learning. In the feature embedding component, there are $2nk$ parameters.

In the feature generation component, there are $h^if^{i-1}f^i$ parameters for convolution matrix in $i$-th convolution layer and $n/p^ikf_i$ neurons in the output of $i$-th pooling layer. In addition, the number of parameters in $i$-th recombination layer is $n/p^ikf^iN^ik$ (since the number of bias is relatively small, we do not discuss it here). Therefore, the total parameters of feature generation component is:
$\sum_{i=1}^{l} h^if^{i-1}f^i+ n/p^ik^2f^iN^i$.

After the feature generating process, we can get $T = n+N$ feature embeddings in total.
Generally, $l$ is less than 5 and $k^2$ is bigger than $f^{i-1}$ meanwhile $f^i/p^i$ is a small number, the space complexity $s_1$ of the feature generating process can be represented as the following formulation:
\begin{equation}
s_1=O(\sum_{i=0}^{l-1} n/p^ik^2f_i N_i) = O(\sum_{i=0}^{l-1}nk^2N_i) = O(nk^2T).
\end{equation}

 For the first hidden layer, the number of parameters in the weight matrix is $(T(T-1)/2+Tk)H_i$. In the $i$-th hidden layer, the number of parameters is $H_(i-1)H_i$. So the space complexity of the deep predictive learning component is:
\begin{equation}\label{eq:p-dpl}
s_2=O(\frac{T(T-1)+2Tk}{2}H_0 + \sum_{i=1}^{m} H_iH_{i-1}),
\end{equation}
where Eq.~(\ref{eq:p-dpl}) can be simplified as  $O(T^2H_0+\sum_{i=1}^mH_iH_{i-1})$. Therefore, the space complexities of FGCNN is $O(T^2H_0+nk^2T+\sum_{i=1}^mH_iH_{i-1})$, which is dominated by the number of generated features, the number of hidden neurons and the size of embedding.
\subsubsection{Time Complexities}
In the $i$-th convolution layer, the output dimension is $n/p^ikf_i$ and each point is calculated from $h_if_{i-1}$ data points. Therefore, the time complexity of the i-th convolution layer is $n/p^ikf_ih_if_{i-1} = O(nkf_ih_i)$ . In the pooling layer, we only need scan the output of convolution layer. So the time complexity of the i-th pooling layer is $n/p^ikf_i$. In the i-th recombination layer,  the time complexity is $n/p^ikf_iN_ik = O(nkN_ik)$. The total time complexity during the feature generating process is
\begin{align}
\begin{split}
 t_1 &= \sum_{i=1}^l O(nkf_ih_i) + O(nkN_i*k) \\ 
 &= O(nTk^2)+ \sum_{i=1}^l O(nkf_ih_i)
 \end{split}
\end{align}

In the FM layer, the time complexity to calculate pairwise inner product is $\frac{T(T-1)k}{2}$. In the first hidden layer, the number of input neurons is $T(T-1)/2+Tk$ while the number of output units is $H_0$. Therefore, the time complexity of the first hidden layer is $O(T^2H_0)$. For the other hidden layers, the time complexity is $O(H_iH_{i-1})$. So, the total complexity in the FM and Deep Component is
\begin{equation}
\begin{split}
 t_2 &= O(T^2H_0)+\sum_{i=1} O(H_iH_{i-1}) \\
 &= O(T^2H_0+\sum_{i=1} H_iH_{i-1})
 \end{split}
\end{equation}
The total time complexity for FGCNN model is $t_1+t_2 = O(T^2H_0+nTk^2+\sum_{i=1}^lnkf_ih_i+\sum_{i=1}H_iH_{i-1})$ which is dominated by the number of generated features, the number of neurons in the first hidden layer, embedding size and convolutional parameters.


==> fgcnn www2019/model_1026_ruiming.tex <==
\section{Feature Generation by Convolutional Neural Network Model}

\subsection{Overview}

In this section, we will describe the proposed Feature Generation by Convolutional Neural Network (FGCNN) model in detail. The used notations are summarized in Table~\ref{table:notations}. 




As shown in Figure~\ref{fig:model_overview}, FGCNN model consists of two components: \textit{Feature Generation} and \textit{Deep Classifier}. More specifically, \textit{Feature Generation} focuses on identifying useful local and global patterns to generate new features as a complement to  raw features, while \textit{Deep Classifier} learns and predicts based on the augmented feature space  through a deep learning model. Besides the two components, we will also formalize \textit{Feature Embedding} of our model. The details of these components are presented in the following subsections. 

\subsection{Feature Embedding}\label{embedding}

%In the area of computer vision, the input images, represented by pixel values in images, are dense and relatively low-dimensional, therefore neural networks are able to handle such input with a reasonable number of parameters. However,
In most CTR prediction tasks, data is collected in a multi-field categorical form\footnote{Features in numerical form are usually transformed into categorical form by bucketing.}~\cite{Shan2016Deep,Zhang2016Deep}, so that each data instance is normally transformed into a high-dimensional sparse (binary) vector via one-hot encoding~\cite{He2014Practical}. For example,
(Gender=Male, Height=175, Age=18, Name=Bob) can be represented as:
 \begin{equation}
  \underbrace{(0,1)}_{\text{Gender=Male}}\underbrace{ (0,...,1,0,0)}_{\text{Height=175}}\underbrace{(0,1,...,0,0)}_{\text{Age=18}}\underbrace{(1,0,0,..,0)}_{\text{Name=Bob}}
 \end{equation}
 
 %Due to the high dimensionality, raw features If raw features in one-hot encoding were fed into neural networks directly, the number of parameters would be unacceptable. Therefore, 
An embedding layer is applied upon the raw features' input to compress them to low-dimensional vectors. In our model, if a field is univalent (e.g., ``Gender=Male''), its embedding is the feature embedding of the field; if a field is multivalent (e.g., ``Interest=Football, Basketball''), the embedding of the field takes the sum of features' embeddings~\cite{dnnyoutube}.

More formally, in an instance, each field $i\ (1 \le i \le n_f)$ is represented as a low-dimensional vector $e_i \in R^{1\times k}$, where $n_f$ is the number of fields and $k$ is embedding size.
Therefore, each instance can be represented as an embedding matrix $E = (e_1^T, e_2^T, ..., e_{n_f}^T)^T$, where $E \in R^{n_f\times k}$. %, by concatenating the field embedding vectors of this instance.
In FGCNN model, the embedding matrix $E$ can be utilized in both \textit{Feature Generation} and \textit{Deep Classifier}.  To avoid the inconsistency of gradient direction when updating parameters, we will introduce another embedding matrix $E' \in R^{n_f\times k}$ for \emph{Deep Classifier} while $E$ is used in \emph{Feature Generation}.
\begin{table}[t]
\vspace{-1ex}
\caption{Notations}
\vspace{-3ex}
\label{table:notations}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|c|l|}
\hline
Parameter & Meaning \\ \hline
$k$ & embedding size \\ \hline
$t_f$ & the total number of one-hot features \\ \hline
$n_f$ & the number of fields\\ \hline
$n_c$ & the number of convolutional layers \\ \hline
$n_h$ & the number of hidden layers \\ \hline
$h^i$ & the height of convolutional kernel in the $i$-th convolutional layer \\ \hline
$h_p$ & pooling height (width=1) of pooling layers \\ \hline
$e_i$ &  the embedding vector for $i$-th field \\ \hline
$E^i$ & the input of the $i$-th convolutional layer \\ \hline
$m_c^i$ & the number of feature maps in the $i$-th convolutional layer \\ \hline
$m_r^i$ & the number of new features' map in the $i$-th recombination layer \\ \hline
$N_i$ & the number of generated features in the $i$-th recombination layer (=$n_f/h_p^im_r^i$) \\ \hline
$C_{:,:,j}^{i}$ & the $j$-th output  feature map of the $i$-{th} convolutional layer \\ \hline
$\mathbb{WC}_{:,:,j}^{i}$ & weights for the $j$-th output feature map of $i$-th convolutional layer\\ \hline
$S_{:,:,j}^{i}$ & the $j$-th output feature map of the $i$-th pooling layer \\ \hline
$\mathbb{WR}^{i}$ & weights for the $i$-th recombination layer \\ \hline
$\mathbb{BR}^{i}$ & bias for the $i$-th recombination layer \\ \hline
$R_{:,:,j}^{i}$ & the $j$-th output map of new features in the $i$-th recombination layer \\ \hline
$W^{i}$ & weights for the $i$-th hidden layer\\ \hline
$B^{i}$ & biases for the $i$-th hidden layer \\ \hline
$H_i$ & number of hidden neorons in the $i$-th hidden layer \\ \hline
\end{tabular}}
\vspace{-3ex}
\end{table}
\subsection{Feature Generation}

As stated in Section~\ref{Introduction}, generating new features from raw features helps improve the performance of deep learning models (as demonstrated by Wide \& Deep Learning~\cite{cheng2016wide}). To achieve this goal, \emph{Feature Generation} designs a proper neural network structure to identify useful feature interactions then generate new features automatically. As argued in Section~\ref{Introduction}, using MLP or CNN alone is not able to generate effective feature interactions from raw features, due to the following reasons: \emph{Firstly}, %MLP consists of only fully connected layers with a large number of parameters. 
 useful feature interactions are always sparse in the combination space of raw features. Therefore, it is difficult for MLP to learn them from a large amount of parameters. \emph{Secondly}, although CNN can alleviates optimization difficulties of MLP by reducing the number of paramters, it only generates neighbor feature interactions which can lose many useful global feature interactions.

 \begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{CNN+Pooling+MLP.pdf}
  \vspace{-3ex}
  \caption{CNN+Recombination structure is able to capture global non-neighbor feature interactions to generate new features. CNN consists of convolutional layer and pooling layer, while Recombination consists of a fully connected layer.}
  \vspace{-5ex}
  \label{fig:CNN+Pooling+MLP}
 \end{figure}

In order to overcome the weakness of applying MLP or CNN alone, as shown in the upper part of Figure~\ref{fig:model_overview}, we perform CNN and MLP~\footnote{According to its function, we will call MLP with one hidden layer as recombination layer later.} as a complement to each other for feature generation. Figure~\ref{fig:CNN+Pooling+MLP} shows an example of CNN+Recombination structure to capture global feature interactions. As can be observed, CNN learns useful neighbor feature patterns with a limited number of parameters, while recombination layer (which is a fully connected layer) generates global feature interactions based on the neighbor patterns provided by CNN. Therefore, important features can be generated  effectively via this neural network structure, which has fewer parameters than directly applying MLP for feature generation. 

In the following parts, we detail the CNN+Recombination structure of \textit{Feature Generation}, namely, \textit{Convolutional Layer}, \textit{Pooling layer}  and \textit{Recombination layer}.

\subsubsection{Convolutional Layer}
 
Each instance is represented as an embedding matrix $E\in R^{n_f\times k}$ via feature embedding, where $n_f$ is the number of fields and $k$ is embedding size. For convenience, reshape the embedding matrix as $E^{1} \in R^{n_f\times k\times 1}$ as the input matrix of the first convolutional layer.
To capture the neighbor feature interactions, a convolutional layer is obtained by convolving a matrix $\mathbb{WC}^1 \in R^{h^1\times 1\times 1\times m_c^{1}}$ with non-linear activation functions (where $h^1$ is the height of the first convolutional weight matrix and $m_c^1$ is the number of feature maps in the first convolutional layer). Suppose the output of the first convolutional layer is denoted as $C^{1} \in R^{n_f\times k\times m_c^1}$, we can formulate the convolutional layer as follows:
\begin{shrinkeq}{0ex}
\begin{equation}
 C_{p,q,i}^1 = tanh(\sum_{m=1}^1\sum_{j=1}^{h^1} E_{p+j-1,q,m}^1 {\mathbb{WC}}_{j,1,1,i}^1)
\end{equation}
\begin{equation}
 tanh(x) = \frac{exp(x)-exp(-x)}{exp(x)+exp(-x)}
\end{equation}


% \begin{align}
%  &C_{p,q,i}^1 = tanh(\sum_{m=1}^1\sum_{j=1}^{h^1} E_{p+j-1,q,m}^1 {\mathbb{WC}}_{j,1,1,i}^1)\\
%  &tanh(x) = \frac{exp(x)-exp(-x)}{exp(x)+exp(-x)}
% \end{align}
\end{shrinkeq}

where $C_{:,:,i}^1$ denotes the $i$-th feature map in the first convolutional layer and $p, q$ are the row and column index of the $i$-th feature map. Notice that the above equation excludes padding which is performed in practice.

\subsubsection{Pooling Layer}

After the first convolutional layer, a max-pooling layer is applied to seize the most important feature interactions and reduce the number of parameters. We refer $h_p$ as the height of pooling layers (width=1). %The output of the first convolutional layer (i.e., the input of the first pooling layer) is represented as $C^1 \in R^{n_f\times k\times m_c^1}$, while 
The output in the first pooling layer is $S^1 \in R^{(n_f/h_p)\times k\times m_c^1}$: %where $m_c^1$ is the number of feature maps in the first  convolutional layer, $n_f$ is the number of fields and $k$ is embedding size:
\begin{equation}
  S^1_{p,q,i} = max(C^1_{p\cdot h_p,q,i},\ ...\ , C^1_{p\cdot h_p+h_p-1,q,i})
\end{equation}
The pooling result of the $i$-th pooling layer will be the input for the $(i+1)$-th convolutional layer:
$ E^{i+1} = S^i$.



\subsubsection{Recombination Layer}

After the first convolutional layer and pooling layer, $S^1 \in R^{(n_f/h_p)\times k\times m_c^1}$ contains the patterns of  neighbor features. Due to the nature of CNN, global non-neighbor feature interactions will be ignored if $S^1$ is regarded as the generated new features. Therefore, we introduce a fully connected layer to recombine the local neighbor feature patterns and generate important new features. We denote the weight matrix as $\mathbb{WR}^1\in R^{(n_f/h_pkm_c^1) \times  (n_f/h_pkm_r^1)}$ and the bias as ${\mathbb{BR}^1} \in R^{(n_f/h_pkm_r^1)}$, where $m_c^1$ is the number of feature maps in  the first convolutional layer and $m_r^1$  is the number of new features' map in the first recombination Layer. Therefore, in the $i$-th recombination layer, $n_f/h_p^im_r^i$ features are generated:
\begin{shrinkeq}{-1ex}
\begin{align}
  &R^1 = tanh(S^1\cdot \mathbb{WR}^1 + {\mathbb{BR}^1})
\end{align}
\end{shrinkeq}
 
\subsubsection{Concatenation}
\vspace{-0.5ex}
New features can be generated by performing CNN+Recombination multiple times. Assume there are $n_c$ convolutional layers, pooling layers and recombination layers and $N_i =n_f/h_p^im_r^i$ fields of  features are generated by $i$-th round denoted as $R^i$. The overall new features $\mathcal{R} \in R^{N\times k}$ (where $N=\sum_{i=1}^{n_c}{N_i}$) generated by \textit{Feature Generation} are formalized as:
\vspace{-0.5ex}
\begin{shrinkeq}{-1ex}
 \begin{align}
\mathcal{R}&= (R^1, R^2, ..., R^{n_c})
 \end{align}
 \end{shrinkeq}


% Particularly,
% \begin{align}
%  R^i &= tanh(S^i\cdot \mathbb{WR}^i + {\mathbb{BR}^i})\\
%   S^i_{p,q,j} &= max(C^i_{p*h_p,q,j},..., C^i_{p*h_p+h_p-1,q,j})\\
%   C_{p,q,j}^i &= tanh(\sum_m \sum_{h=1}^H  E_{p-h^1+1,q,m}^i* {\mathbb{WC}}_{h^1,1,m,j}^i)
%  \end{align}
% where ${WR}^i$ is the weight matrix and ${BR}^i$ is bias in the $i$-th recombination layer, $\mathbb{S}^i$ is the output of $i$-th pooling layer, $C^{i}$ is the output of $i$-th convolutional layer, $E^i$ is the input of $i$-th convolutional layer. 
Then, raw features and new features are concatenated as
\begin{shrinkeq}{-1ex}
\begin{align}
\mathbb{E}& = (E'^T,\mathcal{R}^T)^T
\end{align}
\end{shrinkeq}

where $E'$ is the embedding matrix of raw features  for \textit{Deep Classifier} (see Section~\ref{embedding}). Both the raw features and new features are utilized for CTR prediction in \textit{Deep Classifier}, which will be elaborated in the next subsection.

\subsection{Deep Classifier}\label{sec:clf}

As mentioned above,  raw features and new features are concatenated as an augmented embedding matrix $\mathbb{E} \in R^{(N+n_f)\times k}$, where $N$ and $n_f$ are the number of fields of new features and raw features respectively. $\mathbb{E}$ is input into \emph{Deep Classifier}, which aims to learn further interactions between the raw features and new generated features. In this subsection, for the ease of presentation, we adopt IPNN model~\cite{pin} as the network structure in \textit{Deep Classifier}, due to its good trade-off between model complexity and accuracy. In fact, any advanced network structure can be adopted, which shows the compatibility of FGCNN with the existing works. The compatibility of FGCNN model will be verified empirically in  Section 3. 

\subsubsection{Network Structure}

IPNN model~\citep{pin} combines the learning ability of FM~\cite{Rendle2011Factorization} and MLP. It utilizes an FM layer to extract  pairwise feature interactions from embedding vectors by inner product operations. After that,   the embeddings of input features and the results of FM layer are concatenated and fed to MLP for learning. As evaluated in~\cite{pin}, the performance of IPNN is slightly worse than PIN (the best model in~\cite{pin}), but IPNN is much more efficient.  We will illustrate the network structure of IPNN model.
\begin{figure}[t]
 \centering
 %\vspace{-2ex}
 \includegraphics[width=0.48\textwidth]{IPNN.pdf}
 % IPNN.pdf: 0x0 px, 0dpi, nanxnan cm, bb=
 \vspace{-5ex}
 \caption{Structure of IPNN Model}
 \vspace{-4ex}
  \label{fig:ipnn}
\end{figure}

As shown in Figure~\ref{fig:ipnn}, the pariwise feature interactions of augmented embedding matrix $\mathbb{E}\in R^{(N+n_f)\times k}$ are modeled by an FM layer, as follows:
\vspace{-0.5ex}
\begin{equation}
    R_{fm} = (<\mathbb{E}_{1},\mathbb{E}_2>,...,<\mathbb{E}_{N+n_f-1},\mathbb{E}_{N+n_f}>)
\end{equation}
where $\mathbb{E}_{i}$ is the embedding of the $i$-th field, $<a,b>$ means the inner product of $a$ and $b$. The number of pairwise feature interactions in the FM layer is $\frac{(N+n_f)(N+n_f-1)}{2}$.

After the FM layer, $R_{fm}$ is concatenated with the augmented embedding matrix $\mathbb{E}$, which are fed into MLP with $n_h$ hidden layers to learn implicit feature interactions. We refer the input for the $i$-th hidden layer as $I_i$ and the output for the $i$-th hidden layer as $O_i$. The MLP is formulated as:
\begin{shrinkeq}{-0.1ex}
\begin{align}
 &I_1 = (R_{fm}, flatten(\mathbb{E}))\\
 &O_i = relu(I_{i}W^i+B^i) \\
 &I_{i+1} = O_{i}
\end{align}
\end{shrinkeq}
where $W^i$ and $B^i$ are the weight matrix and bias of the $i$-th hidden layer in MLP. For the last hidden layer (the $n_h$-th layer), we will make final predictions:
\begin{equation}
 \hat{y} = sigmoid(O_{n_h}W^{n_h+1}+b^{n_h+1})
\end{equation}
\vspace{-5ex}
\subsubsection{Batch Normalization}

Batch Normalization (BN) is proposed in~\cite{BN} to solve covariant shift and accelerate DNN training. It normalizes activations $w^Tx$ using statistics within a mini-batch, as follows:
\begin{equation}
 BN(w^Tx) = \frac{w^Tx-avg_i(w^Tx)}{std_i(w^Tx)} g +b
\end{equation} 
where $g$ and $b$ scale and shift the normalized values.

In the FGCNN model, Batch Normalization is applied before each activation function to accelerate model training.

\subsubsection{Objective Function}

The objective function in the FGCNN model is to minimize cross entropy of predicted values and the labels, which is defined as:
\begin{equation}
 \mathcal{L}(y,\hat{y}) = -y log\hat{y}-(1-y)log(1-\hat{y})
\end{equation}
where $y \in \{0,1\}$ is the label and $\hat{y} \in (0,1)$ is the predicted probability of $y=1$.

\subsection{Complexity Analysis}
\label{complexity}
In this section, we analyse the space and time complexity of FGCNN model. Notations in Table ~\ref{table:notations} will be reused.  %\textcolor{red}{summarize the complexities}

\subsubsection{Space Complexity}

The space complexity of FGCNN model consists of  three parts, namely \textit{Feature Embedding}, \textit{Feature Generation} and \textit{Deep Classifier}. In feature embedding, since there are two matrices (one for \textit{Feature Generation} and one for \textit{Deep Classifier} (as discussed in  Section~\ref{embedding})), there are $s_0 = 2t_fk$ parameters, where $t_f$ is the total number of one-hot raw features.

In \textit{Feature Generation}, there are $h^im_c^{i-1}m_c^i$ parameters for convolutional matrix in $i$-th convolutional layer and $n_f/h_p^ik m_c^i$ neurons in the output of $i$-th pooling layer. In addition, the number of parameters in $i$-th recombination layer is $n_f^2/h_p^{2i}k^2m_c^im_r^i$, which will generate $N_i = n_f/h_p^im_r^i$ fields of new features ($n_f/h_p^i = N_i/m_r^i$). Therefore, the total parameters of \textit{Feature Generation} is:
\begin{shrinkeq}{-1ex}
\begin{align}
&\sum_{i=1}^{n_c} h^im_c^{i-1}m_c^i+ n_f^2/h_p^{2i}k^2m_c^im_r^i = \\
&\sum_{i=1}^{n_c} h^im_c^{i-1}m_c^i + N_i^2k^2m_c^i/m_r^i
\end{align}
\end{shrinkeq}
After the \textit{Feature Generation} process, we can get $T = n_f+\sum_{i=1}^{n_c} N_i$ feature embeddings in total.
Normally, $m_r^i$ is usually set as $1,2,3,4$ and  $m_r^i=m_r^{i-1}$. Meanwhile, $h_p$ is usually set to 2 so that $N_{i} = N_1/2^{i-1}$. Furthermore, $N_i^2 k^2 >> h_i m_c^{i-1}$ and $\sum_{i=1}^{n_c} m_c^i/m_r^i 2^{2(i-1)}$ is usually a small number. The space complexity $s_1$ of the feature generating process can be simplified as:
\begin{shrinkeq}{-0.5ex}
\begin{align}
s_1&=O(\sum_{i=1}^{n_c} N_1^2/2^{2(i-1)}k^2m_c^i/m_r^i) = O(N_1^2 k^2)
\end{align}
\end{shrinkeq}


For the first hidden layer of \textit{Deep Classifier}, the number of parameters in the weight matrix is $(T(T-1)/2+Tk)H_1$ (recall that the input is the raw and new features' embedding and their pairwised product). In the $i$-th hidden layer, the number of parameters is $H_{i-1}H_i$. Therefore, the space complexity of \textit{Deep Classifier} is:
\begin{shrinkeq}{-0.5ex}
\begin{equation}\label{eq:p-dpl}
s_2=O(\frac{T(T-1)+2Tk}{2}H_1 + \sum_{i=2}^{n_h} H_iH_{i-1})
\end{equation}
\end{shrinkeq}
where Eq.~(\ref{eq:p-dpl}) can be simplified as  $O(T^2H_1+\sum_{i=2}^{n_h}H_iH_{i-1})$  since $Tk < T(T-1)$ usually. 

In summary, the overall space complexity of FGCNN is $s_0+s_1+s_2=O(t_fk+N_1^2k^2+T^2H_1+\sum_{i=1}^qH_iH_{i-1})$, which is dominated by the number of one-hot features, the number of generated features, the number of hidden neurons and the embedding size.

\subsubsection{Time Complexity}

We first analyze the time complexity in \textit{Feature Generation}. In the $i$-th convolutional layer, the output dimension is $n_f/h_p^{i-1}km_c^i = N_ih_p/m_r^ikm_c^i$ (recall that $N_i = n_f/h_p^im_r^i$) and each point is calculated from $h^im_c^{i-1}$ data points where $h^i$ is the  height of convolutional kernels in the $i$-th convolutional layer. Therefore, the time complexity of the $i$-th convolutional layer is $N_i h_p km_c^i  h^i m_c^{i-1}/m_r^i$ . In the pooling layer, the time complexity of the $i$-th pooling layer is $n_f/h_p^{i-1}km_c^i=N_ih_pkm_c^i/m_r^i $. In the $i$-th recombination layer, the time complexity is $n/h_p^ikm_c^i \cdot  N_ik = N_i^2k^2m_c^i/m_r^i$ (recall $h_p =2$ and $N_i = N_1 / 2^{i-1}$). Therefore, total time complexity of the \textit{Feature Generation} is
\begin{shrinkeq}{-1ex}
\begin{align*}
 t_1 &= \sum_{i=1}^{n_c} N_i h_p km_c^i  h^i m_c^{i-1}/m_r^i+ N_ih_pkm_c^i/m_r^i + N_i^2k^2m_c^i/m_r^i\\ 
 &= \sum_{i=1}^{n_c} N_1km_c^{i}/(m_r^i2^{i-1})(2 h^i m_c^{i-1}+2 + N_1/2^{i-1}k)\\
 &= O(N_1k\sum_{i=1}^{n_c}m_c^{i-1}h^i+N_1^2k^2)\ 
\end{align*}
\end{shrinkeq}
(Notice: $m_c^{i}/(m_r^i2^{i})$ is usually a small number ranging from 2 to 10)

Then, we analyze the time complexity of \textit{Deep Classifier} (taking IPNN as an example). In the FM layer, the time complexity to calculate pairwise inner product is $\frac{T(T-1)k}{2}$. The number of neurons, that are input to the first hidden layer is $T(T-1)/2+Tk$. Therefore, the time complexity of the first hidden layer is $O((T(T-1)/2+Tk)H_1)=O(T^2H_1)$. For the other hidden layers, the time complexity is $O(H_iH_{i-1})$. Therefore, the total time complexity in \textit{Deep Classifier} is
\begin{shrinkeq}{-1ex}
\begin{equation}
 t_2 = O(T^2H_1)+\sum_{i=2}^{n_h} O(H_iH_{i-1})
\end{equation}
\end{shrinkeq}

In summary, the overall time complexity for FGCNN model is $t_1+t_2 = O(N_1k\sum_{i=1}^{n_c}m_c^{i-1}h^i+N_1^2k^2+T^2H_1+\sum_{i=2}^qH_iH_{i-1})$ which is dominated by the number of generated features, the number of neurons in the hidden layers, embedding size and convolutional parameters.



==> fgcnn www2019/related_work.tex <==
\vspace{-1ex}
\section{Related Work}
Click-Through Rate Prediction is normally formulated as a binary classification problem~\cite{Richardson2007Predicting,Chen2016Deep}. In this section, we will introduce two important categories of models in Click-Through Rate predictions, namely \textbf{shallow models} and \textbf{deep learning models}. 

\subsection{Shallow Models for CTR Prediction}
Due to the robustness and efficiency,  Logistic Regression (LR) models~\cite{Ren2016User,Lee2012Estimating}, such as FTRL~\cite{ftrl} are widely used in CTR prediction. To learn feature interactions, a common practice is to manually design pairwise feature interactions in its feature space~\cite{deepfm2,Sun2017Practical}. Poly-2~\cite{poly2} models all pairwise feature interactions to avoid feature engineering. Factorization Machine (FM)~\cite{fm} introduces  low-dimensional vectors for each feature and models feature interactions through inner product of feature vectors. FM improves the ability of modelling feature interactions when data is sparse.  FFM~\cite{ffm} enables each feature to have multiple latent vectors to perform interactions with features  from different fields. LR, Poly-2 and FM variants are widely used in CTR prediction in industry. 

\subsection{Deep Learning for CTR Prediction}
Deep learning has achieved great success in different areas, such as computer vision~\cite{Kaiming2015Deep,Szegedy2016Inception,Huang2016Densely,Xie2017Aggregated}, natural language processing~\cite{Bahdanau2014Neural,Bordes2016Learning,Radford2017Learning,Vaswani2017Attention} etc. In order to leverage deep Learning for CTR prediction, several models are proposed~\cite{crossnet,deepsurvey}. FNN~\cite{fnn} is proposed in ~\cite{fnn}, which uses FM to pre-train the embedding of raw features and then feeds the embeddings to several fully connected layers. Some models adopt DNN to improve FM, such as Attentional FM~\cite{afm}, Neural FM~\cite{nfm}. 

Wide \& Deep Learning~\cite{cheng2016wide} jointly trains a wide model and a deep model where the wide model leverages the effectiveness of feature engineering and the deep model learns implicit feature interactions. Despite the usefulness of wide component, feature engineering is expensive and requires expertise. 
To avoid feature engineering, DeepFM~\cite{deepfm} introduces FM layer (order-2 feature interaction) as a wide component and uses a deep component to learn implicit feature interactions. Different from DeepFM, IPNN~\cite{pin} (also known as PNN in ~\cite{pnn}) feeds both the result of FM layer and embeddings of raw features into MLP   and results in comparable performance. Rather than using inner product to model pairwise feature interactions as DeepFM and IPNN, PIN~\cite{pin} uses a Micro-Network  to learn complex feature interaction for each feature pair. xDeepFM~\cite{xdeepfm} proposes a novel Compressed Interaction Network (CIN) to explicitly generate feature interactions at the vector-wise level.

There are several models which use CNN for CTR Prediction. 
CCPM~\cite{ccpm} applies multiple convolutional layers to explore neighbor feature dependencies. CCPM performs convolutions on the neighbor fields in a certain alignment. Due to that the order of features has no actual meaning in CTR predictions, CCPM can only learn limited feature interactions between neighbor features. In ~\cite{cnntencent}, it is shown that features' arrangement order has a great impact on the final performance of CNN based models. Therefore, the authors propose to generate a set of suitable feature sequences to provide different local information for convolutional layers. However, the key weakness of CNN is not solved. 

In this paper, we propose FGCNN model, which splits the CTR prediction task into two stages: \textit{Feature Generation} and \textit{Deep Classifier}.  \textit{Feature Generation} augments the original feature space by generating new features while most state-of-the-art models can be adopted in \textit{Deep Classifier} to learn and prediction based on the augmented feature space. Different from traditional CNN models for CTR Prediction~\cite{ccpm,cnntencent}, FGCNN can leverage the strength of CNN to extract local information and it greatly alleviates the weakness of CNN by introducing the \textit{Recombination Layer} to recombine information from different local patterns learned by CNN to generating new features.







==> introduction.tex <==
\section{Introduction}
\label{Introduction}

With the rapid development of the Internet and mobile devices, our daily activities connect closely to online services, such as online shopping, online news and videos, online social networks, and many more. Recommender systems are a powful information filter for guiding users to find the items of interest in a gigantic and rapidly expanding pool of candidates. As elaborated in~\cite{alphaNDCG}, if an IR system's response to each query is a ranking of documents in decreasing order of probability of relevance, the overall effectiveness of the system to its user will be maximized. With this principle, the prediction of Click-Through Rate (CTR) is crucial for recommender systems, where the task is to estimate the probability a user will click on a recommended item. In online advertising applications, which is a billion-dollar scenario, the ranking strategy of candidate advertisement is by CTR$\times$bid with ``bid'' being the benifit the system receives once the online advertisement is clicked. In such an application, the performance of CTR prediction models~\cite{pin,deepfm,din} is one of the key facors to boost the revenue of the system.

The key challenge for CTR prediction tasks is effectively modeling feature interactions. Despite their simplicity, generalized linear models, such as FTRL~\cite{ftrl}, have shown decent performance in practice. However, such models lack the ability to learn feature interactions, and a common practice is to manually include pairwise feature interactions in designing its feature space. To overcome this limitation, Factorization Machines (FM)~\cite{fm} are proposed to model pairwise feature interactions as inner product of latent vectors between features and show promising results.

As a powerful approach to learning feature representations, deep neural networks have achieved remarkable progress in computer vision~\cite{din,Huang2016Densely,Kaiming2015Deep,Szegedy2016Inception,Xie2017Aggregated} and natural language processing~\cite{Bahdanau2014Neural,Bordes2016Learning,Radford2017Learning,Vaswani2017Attention}. Being able to learn sophisticated feature interactions automatically, some deep learning models have been proposed for CTR predictions~\cite{pin,deepfm,xdeepfm,ccpm,afm,crossnet,din}, of which all feed raw features to deep neural network to learn feature interactions explicitly or implicitly. Theoretically, deep neural networks are able to learn arbitrary feature interactions (of the raw features) to fit the traning target, by approximating any mathmatical function given the raw features, however, it is quite difficult to learn such feature interactions effectively in practice~\cite{pin,Shalevshwartz2017Failures}. 

Observing such obstacle, Wide \& Deep Learning~\cite{cheng2016wide} leverages the expertise feature engineering by the \emph{wide} component to help learning sophisticated feature interactions automatically by the \emph{deep} component, as shown on the left hand side of Figure~\ref{fig:wide-deep}. Empirically, with the help of generating new features\footnote{Here, new features are the feature interactions of the original raw features. In the rest of this paper, we may use the term ``new features'' for the ease of presentation.} by the wide component, the Wide \& Deep Learning model improves the performance of deep neural network (i.e., the deep component of Wide \& Deep learning alone) significantly, more specifically, 0.6\% AUC improvement in offline test and 1\% CTR improvement in online test.

However, feature engineering (to generate new features) in the wide component of Wide \& Deep Learning is expensive and requires domain knowledge. It would be more effective and more efficient to generate such new features automatically by machine learning models, more generally, deep neural networks. Applying the automatically learning new features, our proposed general framework is presented on the right hand side of Figure~\ref{fig:wide-deep}\footnote{Ignore the text ``CNN'' in the red box in Figure~\ref{fig:wide-deep} for now.}. The orginal raw features are input into a machine learning model (represented by the red box in Figure~\ref{fig:wide-deep}), which generates new features, and then the original raw features and new generated features are combined and fed into the hidden layers of deep neural networks. Generating new features could expand the original feature space and identify useful feature interactions betweeen the original raw features, which reduces the learning difficulies of the hidden layers later and leads to better performance.

\begin{figure}[t]
 \includegraphics[width=0.5\textwidth]{FGCNN_wide_deep.pdf}
 \caption{Comparision Between our Model and Wide\&Deep Model}\label{fig:wide-deep}
\end{figure}

A straightforward method to generate new features is by Multi-Layer Perceptron (MLP). Useful feature interactions are usually sparse in the space of raw features~\cite{pin}, therefore it is difficult to identify such useful feature interactions via learning distinguishable weights among all the feature interactions, by applying MLP alone without any advanced network structure. For example, we have four user features: \textit{user.Name}, \textit{user.Age}, \textit{user.Height}, \textit{user.Gender} to predict whether a user will download a specific online game. Assume that the groundtruth is that the feature interaction between \textit{user.Age} and \textit{user.Gender} is the only signal that matters, so that an optimal model should identify this and only this feature interaction. When performing MLP with only one hidden layer, the optimal weights associated to the embeddings of \textit{user.Name} and \textit{user.ID} should be all 0's, which is fairly difficult to achieve. 

As an advanced network structure of deep nueral networks, Convolutional Neural Network (CNN), which consists of one or multiple kernels with shared weights to capture useful local patterns, has achived great improvement in the area of computer vision~\cite{Huang2016Densely} and natural language processing~\cite{Bahdanau2014Neural}. The case of shared weights alleviates optimization difficulty of the overall model, since there are less weights to optimize. Therefore CNN provides a potentially good solution to realize our idea, i.e., to learn use feature combinations with less weights. However, applying CNN directly results in unsatisfying performance as CNN is designed to generate neighbor patterns but there is usually no meaning of features' arrangement order in CTR prediction.
This is also the reason why there are very few research works to study CNN in CTR prediction task. For example, whether the arrangement order of features being \emph{(Name, Age, Height, Gender)} or \emph{(Age, Name, Height, Gender)} does not make any difference to discribe the semantics of a sample, which is completely different from the case of images and sentences (where the order of pixels and words are very important). In this work, to overcome this limitation when applying CNN to learn feature interactions, we perform CNN and MLP as complementory of each other: learning local neighbor feature interactions via CNN and learning global non-neighbor feature interactions by MLP, which will significantly reduce the number of weights and capture local-global feature interactions at the same time.

In this paper, we propose a new model for CTR prediction task, namely FGCNN (Feature Generation by Convolutional Neural Network). FGCNN can be decomposited to two parts: \emph{feature generation} and \emph{deep predictive learning}. The \emph{feature generation} aims to identify and generate new important features from the original raw features. To avoid learning too many weight parameters by applying MLP directly, we propose to use CNN and MLP as complementory of each other, to identify important feature interactions as the new generated features. More specifically, CNN is performed to learn local neighbor feature interactions, while MLP is applied to recombine CNN's learning pattern, so as to extract global non-neighbor patterns. With both orignal raw features and new generated features, the \emph{deep predictive learning} learns further interactions between all the features, in order to make accurate prediction. Any advanced network structure (such as xDeepFM~\cite{xdeepfm}, DeepFM~\cite{deepfm}, PIN~\cite{pin}) can be adopted as the second part of FGCNN (namely, deep predictive learning), therefore our model has good compatibility with the existing deep learning research works in recommender system. For the ease of illustration, in the main part of this paper, we will adopt IPNN model~\cite{pin} as deep predictive learning part of FGCNN, due to its good trade-off between model complexity and accuracy. To verify the compatibility of our model, the cases of adopting some other existing models as deep predictive learning of or model are also studied empirically.

To summarize, the main contributions of this paper can be highlighted as follows:

\begin{itemize}
\item In CTR prediction task, we identify an important direction, i.e., generating new features automatically before feeding into the predictive models, which could expand the original feature space and identify useful feature interactions between raw features to reduce the learning difficulies of the predictive models.
\item We propose FGCNN model, which consists of \emph{feature generation} and \emph{deep predictive learning}. Feature generation part generates global and local feature interactions as new features, by using CNN and MLP as complementory of each other. More specifically, CNN extracts local patterns with limited parameters to learn, while MLP extends CNN's learning results by extracting global feature interactions. Deep predictive learning part are utilized to learn further interactions between the original raw features and the new generated features (by feature generation part). We adopt IPNN model as deep predictive learning of FGCNN in the main part of this work, however, any advanced predictive model can be adopted, which shows the compatibility of our FGCNN model.
\item We conduct empirical experiment to show the superiority of FGCNN over eight state-of-the-art CTR predictive models on three large-scale datasets (including two public datasets and a private one). Besides, functionality of different components, effect of hyper parameters, and compatibility of our model are also studied in detail. 
\end{itemize}
\textcolor{red}{TBD: the organization of the paper ....}


==> model.tex <==
\section{Feature Generation by Convolution Neural Network Model}
\newpage
\subsection{overview}
In this section, we will introduce the proposed Feature Generation by Convolution Neural Network Model. As shown in Figure ~\ref{fig:model_overview}, the model consists of two components:
\textcolor{red}{\textit{Feature Generation}  better name Convolutional Feature Generation ?} and \textit{FM and Deep Component}.
The first component focus on identifying usefull local and global patterns to generate new features while the second part works on using Factorization Machine and Deep Neural Network to learn implicit and explict feature interactions. Each componet will be detailed in the following parts.

\subsection{Feature Generation}
As mentioned in Section~\ref{Introduction},  although MLP can approximate learn any specific feature interactions theoratically, it is quite difficult to learn in practice~\cite{Shalevshwartz2017Failures}. One possible reason is that usefull cross features are usually sparse in the combination space of raw features and it is challenging for MLP to identify important feature combinations while disregarding useless combinations. Many data scientists tries to extract useful features from raw data first based on their domain knowledge and feed the extracted features and  raw features to DNNs such as Wide\&Deep Learning. And such methods do improve the performance of DNNs, which demonstrates the effectiveness of identifying important features before using DNNs. However, feature engineering is expensive and requires domain knowledge. Therefore, we wonder whether we can use Neural Network to automatically identify some cross features as feature engineering does and then use DNN to learn further feature interactions. 

 Simply using fully connected neural network can not works well for feature combination idenfication, since the optimal combinations is sparse and it is hard to learn the weights of unrelated features(usually the weights of their embedding) as zero during optimization. For example, we want to use the embedding of four features -\textbf{(User.Name, User.ID, User.Age, User.Gender)} to predict whether a user will download a game Application. In practice, only the combination of \textbf{Age} and \textbf{Gender(Age$<$30 and gender$=$Male) }could contribute to the prediction. And it could be quite challenging in multi-layer perceptron to learn the optimal weights as the number of unrelated features and the size of feature's embedding increase.  
 
 Convolutional Neural Network(CNN) recently has achieved great progress in the area of computer vision and natural language processing . The main advanteges of CNN is that the convolution kernel with shared weights in the convolution kernel can capture important local patterns and pooling is used to reduce the input demension. Shared weight means less parameters which usually lead to simplified optimization difficulties for find optimal combination weights. The nature of CNN matches our initial intention of discovering important feature interactions from a large combination space.  However, unlike sentences or images, different arrangement of features does not change meaning of a sample in the area of Click-Through Rate Prediction. For example, whether \textbf{(User.Name, User.ID, User.Age, User.Gender)} or \textbf{(User.Gender, User.ID, User.Age, User.Name)} is actually the same to portray a given user. Due to this, CNN is criticised of only learning the feature interactions between neighbor features, which also limited the use of CNN in this area.
 
 \begin{figure}[t]
  \includegraphics[width=0.48\textwidth]{CNN+Pooling+MLP.pdf}
  \caption{How CNN+Pooling+MLP captures non-neighbor interactions to generate new features}
  \label{fig:CNN+Pooling+MLP}
 \end{figure}

 In this paper, CNN+Pooling+Recombination is proposed to overcome the weakness of CNN, which is able to capture neighbor and non-neighbor feature interactions. Figure~\ref{fig:CNN+Pooling+MLP} shows an example of how CNN+Poooling+Recombination works. As it shows, the structure not only leverages the benifits of Convolution layer and Pooling Layer to learn feature interactions in a neighboring region, but also has the ability to capture the interactions of non-neighbor features. Moreover, with the height in the convolution kernel increases, it is possible to learn high-order feature interactions.

 In the following parts, we will detail the structure seperately:
 
 
 \subsubsection{Embedding Layer}
 In most CTR Prediction tasks, data are collected in a multi-field categorical form. And each data instance is transformed into a high-dimensional sparse(binary) vector via one-hot encoding~\cite{He2014Practical}.For example,
\textbf{(Gender=Male, ID=123, Age=18, Name=Mary)} can be representated as:
 \begin{equation}
  \underbrace{(0,1)}_{\text{Gender=Male}}\underbrace{ (0,...1,0,0)}_{\text{ID=123}}\underbrace{(0,1,...0,0)}_{\text{Age=18}}\underbrace{(1,0,0,..,0)}_{\text{Name=Mary}}
 \end{equation}

 Next, each one entry $i (1 \le i \le n)$ will be representated by a low dimensional vector $e_i \in R^{1*k}$, where $n$ is the number of fields and $k$ is embedding size. 
 Then, all embedding vector $e_i( 1 \le i \le n)$ will be concatenated as a embedding matrix $E \in R^{n*k}$.   
 In this paper, since the embedding matrix $E$ will be used in both feature genenration and DNNs, to reduce the inconsistency in the direction of gradients, we introduce another embedding  matrix $E' \in R^{n*k}$ for accepting gradient updates from DNN while  $E$ accepts gradient updates from feature genenration.\label{embedding}
 
 
 
 \subsubsection{Convolution Layer}
 After the embedding layer, we can get the embedding matrix $E = (e_1^T, e_2^T,...e_n^T)^T \in R^{n*k}$ of raw features, where $n$ is the number of fields and $k$ is embedding size. The convolution layer is obtained by convolving a matrix $\mathcal{W} \in R^{H*1*f}$ with non-linear activation functions($H$ is the height of convolution matrix and $f$ is the number of feature maps). Suppose the output of Convolution Layer is $F \in R^{n*k*f}$:
\begin{align}
 F_{i,j,m} &= tanh(\sum_{h=1}^H  E_{i-h+1,j}*\mathcal{W}_{h,0,m})\\
 tanh(x) &= \frac{exp(x)-exp(-x)}{exp(x)+exp(-x)}
\end{align}
Note: the above equation excludes padding while actual model uses it. 
 \subsubsection{Pooling Layer}
 After getting the result $F \in R^{n*k*f}$ of Convolution Layer, max pooling is applied to reduce the  number of  paramenters. In our model, $p*1$ is the preferred kernel. Suppose the output in this layer is $\mathbb{F} \in R^{(n/p)*k*f}$:
 \begin{equation}
  \mathbb{F}_{i,j,m} = max(F_{i*p,j,m},F_{i*p+1,j,m},..., F_{i*p+p-1,j,m})
 \end{equation}
 \subsubsection{Recombination Layer}
 After Convolution Layer and Pooling Layer, $\mathbb{F}$ already contains information in the neighboring fields. Due to that important feature interactions is usually sparse and the arrangement of raw features is quite random, some feature interactions can be losed if using $\mathbb{F}$ as the feature interaction results and generating features. Therefore, we introduce a fully connected layer to recombine the interactions from different positions.  Suppose the weights is $\mathbb{W}\in R^{(n/p*k*f) * (N *k)}$ and the bias is ${b} \in R^{(N*k)}$ where $n$ is the field num, $p$ is the pooling kernel size, $k$ is the embed size, $f$ is the number of feature maps and $N$ is the number of new features.  The new features can be represented as $\mathbb{N} \in R^{N*k}$:
 \begin{align}
  &\mathbb{N} = tanh(\mathbb{F}*\mathbb{W} + {b}) 
 \end{align}

 So far, new features are generated among patterns from different Convolution+Pooling results. Furthermore, the Convolution+Pooling+Recombination operations can be repeated many times to yield
 different orders of feature interactions.
 Recall the whole process of Convolution+Pooling+Recombination, Convolution Layer enumurates some possible feature interactions and Pooling Layer filters useless iteractions while Recombination Layer recombines the information in each corner to generate new features. 
 
Old feature and new features can be concatenated as：
\begin{align}
\mathbb{E}&=(E'^T,\mathbb{N}^T)^T 
\end{align}
where $E'$ is the embedding matrix for DNN(see Section ~\ref{embedding}). The augmented feature set can be further leveraged by different Deep Models.

Unlike traditional models only use Deep Neural Network to learn implicit and explicit feature interaction and make final predictions, our method try to identify some important patterns to generate new feature first to reduce the learning difficulties in DNN. This is also the major difference from traditional models.
\subsection{FM and Deep Component}
After the feature generation process by CNN, raw features and new features are concatenated as $\mathbb{E}=(e_1^T,e_2^T,...,e_{N+n}^T)^T \in R^{(N+n)*k}$ where $N$ is the number of new features, $n$ is the number of raw features and $k$ is embedding size. The second part adopts the structure of IPNN model~\cite{pin}, which involves a Factorization Machine~\cite{Rendle2011Factorization} and a Multi-Layer Perceptron(MLP) to make a final predictions. The main reason for choosing IPNN rather than other models(such as xDeepFM, deepFM, and PIN) is that IPNN outperforms other models except PIN in many datasets~\cite{pin} and IPNN is more suitable than PIN when the number of input features is big since IPNN use inner-product to model pairwise interactions and PIN use Micro-Network to model them.
\subsubsection{Factorization Machine Component}
Factorization Machine is proposed in ~\cite{Rendle2011Factorization} to learn feature interactions for recommendation. FM models pairwise(order-2) feature interactions as inner product of feature's embeddings~\cite{deepfm}. In our model, we use the inner product of different features to get explicit feature interactions. The output of FM component $R_{fm}$ can be reformulated as:
\begin{equation}
    R_{fm} = (<\mathbb{E}_{1},\mathbb{E}_2>,<\mathbb{E}_i, \mathbb{E}_j>,...<\mathbb{E}_{N+n-1},\mathbb{E}_{N+n}>)
\end{equation}
The total interactions in FM component is $\frac{(N+n)*(N+n-1)}{2}$. 
\subsubsection{Deep Component}
As we get the FM results and embedding matrix of raw features and generated features, the two results is fed into Multi-Layer-Perceptron to learn implicit feature Interactions. Suppose input for the i-th hidden layer is $I_i$ and the output for the i-th hidden layer is $O_i$:
\begin{align}
 &I_0 = (R_{fm}, \mathbb{E})\\
 &O_i = relu(I_{i}*W_i+b_i) \\
 &I_{i+1} = O_{i}
\end{align}
where $W_i$ is the weight matrix for layer-$i$ and $b$ is the bias. For the last layer, we will make final predictions:
\begin{equation}
 y = sigmoid(I_i*W_i+b_i)
\end{equation}

\subsubsection{Batch Normalization}
Batch Normalization(BN) is proposed in~\cite{BN} to solve covariate shift and accelerate DNN training and it works quite well in our FGCNN model.

BN normalizes activations $w^Tx$ using statistics within a mini-batch
\begin{equation}
 BN(w^Tx) = \frac{w^Tx-avg_i(w^Tx)}{std_i(w^Tx)} *g +b
\end{equation} where $g$ and $b$ scale and shift the normalized values. 

In the FGCNN model, Batch Normalization is applied before each activation function to accelerate model training.
\subsubsection{Objective Function}
The objective function in the   FGCNN model is to minimize cross entropy, which is defined as:
\begin{equation}
 \mathcal{L}(y,\sigma(\hat{y})) = -y log(\sigma{\hat(y)})-(1-y)log(1-\sigma(\hat{y}))
\end{equation}
where $y \in \{0,1\}$ is the label and $\sigma(\hat{y}) \in (0,1)$ is the predicted probability of $y=1$.


\subsection{Complexity Analysis}
We analyse our proposed FGCNN model to study the model complexity. The notations that will be used are summerized in Table~\ref{notations}. \textcolor{red}{summarize the complixities}
\begin{table}[h]
\caption{Notations}
\label{notations}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|l|l|}
\hline
Parameter & Meaning \\ \hline
$k$ & embed size \\ \hline
$n$ & field num \\ \hline
$l$ & num of convolution layers \\ \hline
$m$ & number of hidden layers \\ \hline
$h_i$ & height of conv kernel in the i-th conv layer \\ \hline
$p$ & pooling height(width=1) \\ \hline
$f_i$ & feature map num in the i-th conv layer \\ \hline
$N_i$ & new feature num in the i-th recombination layer \\ \hline
$H_i$ & hidden neurons in the i-th Hidden layer \\ \hline

\end{tabular}}
\end{table}
\subsubsection{Space Complexities}
In the i-th convolution layer, there are total $h_if_{i-1}f_i$ parameters for conv matrix. And in the i-th pooling layer, the number of neurons in pooling output is $n/p^ikf_i$. Therefore, for the i-th recombination Layer to generate $N_i$ new features, the parameter for the weight matrix is $n/p^ikf_i N_ik$(since the number of bias is relatively small, we do not discuss it here). In the convolution+pooling+recombination Layer, the number of total parameters $p_1$is :
\begin{equation}
p_1 = \sum_{i=1}^{l} h_if_{i-1}f_i+ n/p^ik^2f_iN_i
\end{equation}
After the feature generating process, we can get $T = n+\sum_{i=0}^{l} N_i$ in total.
Notice that $l$ is usually less than 5 and $k^2$ is often bigger than $f_{i-1}$ meanwhile $f_i/p^i$ is usually a small number, the total parameters in the feature generating process is $p_1 = O(\sum_{i=0}^{l-1} n/p^ik^2f_i N_i) = O(\sum_{i=0}^{l-1}nk^2N_i) = O(nk^2T)$.

 For the first hidden layer, the number of parameters in the weight matrix is $(T(T-1)/2+Tk)H_i$. In the i-th layer, the number of parameters is $H_(i-1)H_i$. Total parameters in the FM and Deep Component is 
\begin{equation}
 p_2 = \frac{T(T-1)+2Tk}{2}H_0 + \sum_{i=1}^{m} H_iH_{i-1}
\end{equation}
$p_2$ can be simplified as  $O(T^2H_0+\sum_{i=1}^mH_iH_{i-1})$. Therefore, the space complexities of FGCNN is $O(T^2H_0+nk^2T+\sum_{i=1}^mH_iH_{i-1})$, which is dominated by the number of generated features, the number of hidden neurons and the size of embedding.
\subsubsection{Time Complexities}
In the i-th convolution layer, the output demension is $n/p^ikf_i$ and each point is calculated from $h_if_{i-1}$ data points. Therefore, the time complexity in the i-th convolution layer is $n/p^ikf_ih_if_{i-1} = O(nkf_ih_i)$ . In the pooling layer, we just need to scan the output of convolution layer. So the time complexity in the i-th pooling layer is $n/p^ikf_i$. In the i-th recombination layer,  the time complexity is $n/p^ikf_iN_ik = O(nkN_ik)$. The total time complexity during the feature generating process is
\begin{equation}
 t_1 = \sum_{i=1}^l O(nkf_ih_i) + O(nkN_i*k) = O(nTk^2)+ \sum_{i=1}^l O(nkf_ih_i)
\end{equation} where $T = n+\sum_{i=0}^{l} N_i$

In the FM layer, the time complexity to calculate pairwise inner product is $\frac{T(T-1)k}{2}$. In the first hidden layer, the number of input neurons is $T(T-1)/2+Tk$ while the number of output units is $H_0$. Therefore, the time complexity of the first hidden layer is $O(T^2H_0)$. For the other hidden layers, the time complexity is $O(H_iH_{i-1})$. So, the total complexity in the FM and Deep Component is
\begin{equation}
 t_2 = O(T^2H_0)+\sum_{i=1} O(H_iH_{i-1}) = O(T^2H_0+\sum_{i=1} H_iH_{i-1})
\end{equation}
The total time complexity for FGCNN model is $t_1+t_2 = O(T^2H_0+nTk^2+\sum_{i=1}^lnkf_ih_i+\sum_{i=1}H_iH_{i-1})$ which is dominated by the number of generated feature, the number of neurons in first hidden layer, embed size and  convolutional parameters. 


==> model_1025_huifeng.tex <==
\section{Feature Generation by Convolution Neural Network Model}

\subsection{overview}

In this section, we will introduce the proposed Feature Generation by Convolutional Neural Network (FGCNN in short) model.
The notations that will be used are summerized in Table~\ref{notations}.
\begin{table}[!t]
\caption{Notations}
\label{notations}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|c|l|}
\hline
Parameter & Meaning \\ \hline
$k$ & embedding size \\ \hline
$n$ & the number of fields\\ \hline
$l$ & the number of convolution layers \\ \hline
$m$ & the number of hidden layers \\ \hline
$h^i$ & the height of convolutional kernel in the i-th convolutional layer \\ \hline
$p^i$ & pooling height(width=1) of i-th convolution layer \\ \hline
$E^i$ & the input of the i-th convolutional layer \\ \hline
$f^i$ & the number of feature maps in the i-th convolutional layer \\ \hline
$FC^i$ & the output of the i-th convolutional layer \\ \hline
$N^i$ & the number of new features in the i-th recombination layer \\ \hline
$FP^i$ & the output of the i-th pooling layer \\ \hline
$H_i$ & the neurons in the i-th hidden layer \\ \hline

\end{tabular}}
\end{table}
As shown in Figure ~\ref{fig:model_overview}, the model consists of three components: \textcolor{red}{Feature Embedding}, \textcolor{red}{\textit{Feature Generation}} and \textcolor{red}{\textit{Deep  Predictive Learning}}. Specifically, the second component focuses on identifying useful local and global patterns to generate new features as a complementary for raw features, while the third part works on capturing feature interactions based on the augmented feature space implicitly and explicitly through a deep predictive learning model. The details of these components are introduced in the following.

\subsection{Feature Embedding}\label{embedding}
In computer vision and natural language processing, the input data are usually images and sentences, which are known to be dense, so DNNs can be applied directly on the raw features. However, in most CTR Prediction tasks, the input are sparse and collected in a multi-field categorical form, which is widely used in related works~\cite{xdeepfm,pin,deepfm}. Each data instance is transformed into a high-dimensional sparse(binary) vector via one-hot encoding~\cite{He2014Practical}. For example,
\textbf{(Gender=Male, ID=123, Age=18, Name=Mary)} can be representated as:
 \begin{equation}
  \underbrace{(0,1)}_{\text{Gender=Male}}\underbrace{ (0,...1,0,0)}_{\text{ID=123}}\underbrace{(0,1,...0,0)}_{\text{Age=18}}\underbrace{(1,0,0,..,0)}_{\text{Name=Mary}}
 \end{equation}

An embedding layer is applied to compress the raw features to the dense real-value vectors. The feature embedding is used as the field embedding if the field is univalent. Take the above instance as an example, the embedding of feature ``Male'' is taken as the embedding of field ``Gender''. Similar with \cite{xdeepfm}, if the field is multivalent, the sum of feature embedding is used as the field embedding.

Specifically, each entry $i (1 \le i \le n)$ will be represented as a low dimensional vector $e_i \in R^{1*k}$, where $n$ is the number of fields and $k$ is embedding size.
Then, all embedding vector $e_i( 1 \le i \le n)$ will be concatenated as a embedding matrix $E=(e_1^T, e_2^T, ..., e_n^T)^T$, where $E \in R^{n*k}$.
In this paper, the embedding matrix $E$ will be used in both feature generation and deep predictive learning. To reduce the inconsistency in the direction of gradients when updating parameters, another embedding  matrix $E' \in R^{n*k}$  is introduced and fed into deep predictive learning model. In other words, $E'$ for deep predictive learning model while $E$ for feature generation component.
\subsection{Feature Generation}
In practice, the ability of learning sophisticated feature interactions is critical for CTR models. Although MLP is able to approximate any specific feature interaction theoretically, it is difficult to learn in practice because the combination space of raw features is too sparse. It is challenging for MLP to identify important feature interactions while disregarding useless combinations. For the purpose of capturing more meaningful feature interaction, Wide \& Deep model utilizes the manually designed features as a complementary of raw features. As a result, both offline AUC and online CTR are improved. However, it is impractical because designing manually features is expensive and requires domain knowledge. Therefore, we wonder whether we can design a feature generation model to automatically identify some cross features as feature engineering does.

Due to the ability of feature representation, deep learning promotes the progress in many fields related to machine learning. However, simply using fully connected neural network can not works well for feature combination identification. Since the optimal combinations is sparse and it is hard to learn the weights of unrelated features (usually the weights of their embedding) as zero during optimization. For example, we want to use the embedding of four features -\textbf{(User.Name, User.ID, User.Age, User.Gender)} to predict whether a user will download a game Application. In practice, only the combination of \textbf{Age} and \textbf{Gender(Age$<$30 and gender$=$Male) }could contribute to the prediction.


Recently, Convolutional Neural Network (CNN) has achieved great progress in the area of computer vision and natural language processing. CNN has many advantages, two of which are more important: (1) the convolutional kernel with shared weights can capture important local patterns; (2) the pooling technique is used to reduce the input dimension and select meaningful features. In addition, shared weight means less parameters which usually lead to easier learning process and lower optimization difficulty. So CNN is suitable for discovering important feature interactions from a large combination space, which is matching our initial intention. Unfortunately, unlike sentences and images, different arrangement of features does not change the meaning of a sample in the area of CTR prediction. For example, whether \textbf{(User.Name, User.ID, User.Age, User.Gender)} or \textbf{(User.Gender, User.ID, User.Age, User.Name)} is actually the same to portray a given user. Therefore, CNN is criticised of only learning the feature interactions between neighbor features, which also limited the use of CNN in this area.


 \begin{figure}[t]
  \includegraphics[width=0.48\textwidth]{CNN+Pooling+MLP.pdf}
  \caption{How CNN+Pooling+MLP captures non-neighbor interactions to generate new features}
  \label{fig:CNN+Pooling+MLP}
 \end{figure}

In order to overcome this limitation to take the advantage of CNN to capture neighbor and non-neighbor feature interactions, a CNN+Pooling+Recombination structure is proposed in this paper. Figure~\ref{fig:CNN+Pooling+MLP} shows an example of how CNN+Poooling+Recombination works. As it shows, the structure not only leverages the benefits of convolution layer and pooling layer to learn feature interactions in a neighboring region, but also has the ability to capture the interactions of non-neighbor features. Moreover, with the height in the convolution kernel increases, it is possible to learn high-order feature interactions.

 In the following parts, we will detail the structure separately:





 \subsubsection{Convolution Layer}
 After the embedding layer, we can get the embedding matrix $E = (e_1^T, e_2^T,...e_n^T)^T \in R^{n*k}$ of raw features, where $n$ is the number of fields and $k$ is embedding size. For convenience, rename the embedding matrix as $E^{1}$.
 To capture the local neighbor feature interactions, the convolution layer is obtained by convolving a matrix $\mathcal{W} \in R^{H*1*f^{1}}$ with non-linear activation functions($H$ is the height of convolution matrix and $f^1$ is the number of feature maps in the first convolution layer). Suppose the output of the first Convolution Layer is denoted as $FC^{1} \in R^{n*k*f^1}$, we can get:
\begin{align}
 FC^{1}_{i,j,f^{1}_{o_1}} &= tanh(\sum_{h=1}^H  E^{1}_{i-h+1,j}*\mathcal{W}_{h,0,f^{1}_{o_1}})\\
 tanh(x) &= \frac{exp(x)-exp(-x)}{exp(x)+exp(-x)}
\end{align}
where $f^{1}_{o_1}$ denotes the $o_1-{th}$ kernel in the first convolution layer. Note: the above equation excludes padding while actual model uses it.
 \subsubsection{Pooling Layer}
 After getting the result $FC^1$ of the first Convolution Layer, max pooling is applied to seize the most important feature interactions and reduce the number of  parameters. In our model, $p^1*1$ is the preferred kernel of the first pooling layer. Suppose the output in this layer is $\mathbb{FP}^1 \in R^{(n/p^1)*k*f}$:
 \begin{equation}
  \mathbb{FP}^1_{i,j,f^1_{o_1}} = max(FC^1_{i*p^1,j,f^1_{o_1}},..., FC^1_{i*p^1+p^1-1,j,f^1_{o_1}})
 \end{equation}
 \subsubsection{Recombination Layer}
 After Convolution Layer and Pooling Layer, $\mathbb{FP}^1$ already contains information in the neighboring fields. Due to that important feature interactions is usually sparse and the arrangement of raw features is quite random, some feature interactions might be ignored if using $\mathbb{FP}^1$ as the feature interaction results and generating features. Therefore, we introduce a fully connected layer to recombine the interactions from different positions. Specifically, set the weight matrix as $\mathbb{W}^1\in R^{(n/p^1*k*f^1) * (N^1 *k)}$ and the bias as ${b^1} \in R^{(N^1*k)}$, where $n$ is the field num and $p^1$ is the size of pooling kernel in the first pooling layer, $k$ is the embedding size, $f^1$ is the number of feature maps in first convolution layer and $N^1$ is the number of new features after one time convolution and pooling.  The new features can be represented as $\mathbb{N}^1 \in R^{N^1*k}$:
 \begin{align}
  &\mathbb{N}^1 = tanh(\mathbb{FP}^1*\mathbb{W}^1 + {b^1})
 \end{align}
\subsubsection{Concatenation}
 So far, new features are generated among patterns from different Convolution+Pooling results. Furthermore, the Convolution+Pooling+Recombination operations can be repeated many times to yield different orders of feature interactions. Recall the whole process of Convolution+Pooling+Recombination, Convolution Layer enumerates some possible feature interactions and Pooling Layer filters useless interactions while Recombination Layer recombines the information in each corner to generate new features. If we set the number of convolution layers as $l$, new features $\mathbb{N} \in R^{N*k}$, where $N=\sum_{i=1}^{l}{N^i}$, are generated by Feature Generation component:
 \textcolor{red}{pls. modify the mistake in the following equation}
 \begin{align}
\mathbb{N}&= (\mathbb{N}^1, \mathbb{N}^2, ..., \mathbb{N}^l)
 \end{align}
Particularly,
\begin{align}
 \mathbb{N}^l &= tanh(\mathbb{FP}^l*\mathbb{W}^l + {b^l})
 \end{align}
 \begin{align}
  \mathbb{FP}^l_{i,j,f^l_{o_l}} &= max(FC^{l}_{i*p^l,j,f^l_{o_l}},..., FC^l_{i*p^l+p^l-1,j,f^l_{o_l}})
  \end{align}
  \begin{align}
 FC^{l}_{i,j,f^l_{o_l}} &= tanh(\sum_{o_{l-1}=1}^{f^{l-1}}\sum_{h=1}^H  E^{l}_{i-h+1,j,f^{l-1}_{o_{l-1}}}*\mathcal{W}_{h,0,f^{l}_{o_l}})
\end{align}
where $\mathbb{W}_l$ is the weight matrix and ${b_l}$ is bias in the $l_{th}$ recombination layer, $\mathbb{FP}^l$ is the output of $l_{th}$ pooling layer, $FC^{l}$ is the output of $l_{th}$ convolution layer, $f^l_{o_l}$ is the $o_l$-th kernel in $l$-th convolution layer, and $E^{l}$ is $\mathbb{FP}^{l-1}$.
Then, old feature and new features can be concatenated as£º
\begin{align}
\mathbb{E}&=(E'^T,\mathbb{N}^T)^T
\end{align}
where $E'$ is the embedding matrix for DNN(see Section ~\ref{embedding}). The augmented feature set can be further leveraged by different Deep Models.

Unlike traditional models only use Deep Neural Network to learn implicit and explicit feature interaction and make final predictions, our method try to identify some important patterns to generate new feature first to reduce the learning difficulties in DNN. This is also the major difference from traditional models.
\subsection{Deep Predictive Learning}
After the feature generation process by CNN, raw features and new features are concatenated as the augmented embedding matrix $\mathbb{E} \in R^{(N+n)*k}$ where $N$ is the number of new features, $n$ is the number of raw features and $k$ is embedding size. In order to learn the feature interactions implicitly and explicitly, deep predictive learning model adopts the structure of IPNN model~\cite{pin}, which involves a Factorization Machine~\cite{Rendle2011Factorization} and a Multi-Layer Perceptron(MLP) to make a final predictions.
In fact, IPNN outperforms other models except PIN in many datasets~\cite{pin}. The motivation behind our selection is that IPNN is more efficient than PIN since IPNN use inner-product to model pairwise interactions and PIN use Micro-Network to model them.
\subsubsection{Factorization Machine Component}
Factorization Machine is proposed in ~\cite{Rendle2011Factorization} to learn feature interactions for recommendation. FM models pairwise (order-2) feature interactions as inner product of feature's embeddings~\cite{deepfm}. In our model, we use the inner product of different features to get explicit feature interactions. The output of FM component $R_{fm}$ can be reformulated as:
\begin{equation}
    R_{fm} = (<\mathbb{E}_{1},\mathbb{E}_2>,<\mathbb{E}_i, \mathbb{E}_j>,...<\mathbb{E}_{N+n-1},\mathbb{E}_{N+n}>)
\end{equation}
where $\mathbb{E}_{i}$ is the embedding of the $i$-th vector, $<a,b>$ means the inner product of vector a and b and the number of interactions in FM component is $\frac{(N+n)*(N+n-1)}{2}$.
\subsubsection{Deep Component}
As we get the FM results and the augmented embedding matrix $\mathbb{E}$, the two results are fed into Multi-Layer-Perceptron to learn implicit feature Interactions. Suppose input for the i-th hidden layer is $I_i$ and the output for the i-th hidden layer is $O_i$:
\begin{align}
 &I_0 = (R_{fm}, flatten(\mathbb{E}))\\
 &O_i = relu(I_{i}*W_i+b_i) \\
 &I_{i+1} = O_{i}
\end{align}
where $W_i$ is the weight matrix for layer-$i$ and $b$ is the bias. For the last layer, we will make final predictions:
\begin{equation}
 y = sigmoid(I_i*W_i+b_i)
\end{equation}

\subsubsection{Batch Normalization}
Batch Normalization(BN) is proposed in~\cite{BN} to solve covariant shift and accelerate DNN training and it works quite well in our FGCNN model.

BN normalizes activations $w^Tx$ using statistics within a mini-batch
\begin{equation}
 BN(w^Tx) = \frac{w^Tx-avg_i(w^Tx)}{std_i(w^Tx)} *g +b
\end{equation} where $g$ and $b$ scale and shift the normalized values.

In the FGCNN model, Batch Normalization is applied before each activation function to accelerate model training.
\subsubsection{Objective Function}
The objective function in the   FGCNN model is to minimize cross entropy, which is defined as:
\begin{equation}
 \mathcal{L}(y,\sigma(\hat{y})) = -y log(\sigma{\hat(y)})-(1-y)log(1-\sigma(\hat{y}))
\end{equation}
where $y \in \{0,1\}$ is the label and $\sigma(\hat{y}) \in (0,1)$ is the predicted probability of $y=1$.


\subsection{Complexity Analysis}
In this section, we analyse the space and time complexities of the proposed FGCNN model.  \textcolor{red}{summarize the complexities}
\subsubsection{Space Complexities}
The space complexities include three aspects, namely feature embedding, feature generation and deep predictive learning. In the feature embedding component, there are $2nk$ parameters.

In the feature generation component, there are $h^if^{i-1}f^i$ parameters for convolution matrix in $i$-th convolution layer and $n/p^ikf_i$ neurons in the output of $i$-th pooling layer. In addition, the number of parameters in $i$-th recombination layer is $n/p^ikf^iN^ik$ (since the number of bias is relatively small, we do not discuss it here). Therefore, the total parameters of feature generation component is:
$\sum_{i=1}^{l} h^if^{i-1}f^i+ n/p^ik^2f^iN^i$.

After the feature generating process, we can get $T = n+N$ feature embeddings in total.
Generally, $l$ is less than 5 and $k^2$ is bigger than $f^{i-1}$ meanwhile $f^i/p^i$ is a small number, the space complexity $s_1$ of the feature generating process can be represented as the following formulation:
\begin{equation}
s_1=O(\sum_{i=0}^{l-1} n/p^ik^2f_i N_i) = O(\sum_{i=0}^{l-1}nk^2N_i) = O(nk^2T).
\end{equation}

 For the first hidden layer, the number of parameters in the weight matrix is $(T(T-1)/2+Tk)H_i$. In the $i$-th hidden layer, the number of parameters is $H_(i-1)H_i$. So the space complexity of the deep predictive learning component is:
\begin{equation}\label{eq:p-dpl}
s_2=O(\frac{T(T-1)+2Tk}{2}H_0 + \sum_{i=1}^{m} H_iH_{i-1}),
\end{equation}
where Eq.~(\ref{eq:p-dpl}) can be simplified as  $O(T^2H_0+\sum_{i=1}^mH_iH_{i-1})$. Therefore, the space complexities of FGCNN is $O(T^2H_0+nk^2T+\sum_{i=1}^mH_iH_{i-1})$, which is dominated by the number of generated features, the number of hidden neurons and the size of embedding.
\subsubsection{Time Complexities}
In the $i$-th convolution layer, the output dimension is $n/p^ikf_i$ and each point is calculated from $h_if_{i-1}$ data points. Therefore, the time complexity of the i-th convolution layer is $n/p^ikf_ih_if_{i-1} = O(nkf_ih_i)$ . In the pooling layer, we only need scan the output of convolution layer. So the time complexity of the i-th pooling layer is $n/p^ikf_i$. In the i-th recombination layer,  the time complexity is $n/p^ikf_iN_ik = O(nkN_ik)$. The total time complexity during the feature generating process is
\begin{align}
\begin{split}
 t_1 &= \sum_{i=1}^l O(nkf_ih_i) + O(nkN_i*k) \\ 
 &= O(nTk^2)+ \sum_{i=1}^l O(nkf_ih_i)
 \end{split}
\end{align}

In the FM layer, the time complexity to calculate pairwise inner product is $\frac{T(T-1)k}{2}$. In the first hidden layer, the number of input neurons is $T(T-1)/2+Tk$ while the number of output units is $H_0$. Therefore, the time complexity of the first hidden layer is $O(T^2H_0)$. For the other hidden layers, the time complexity is $O(H_iH_{i-1})$. So, the total complexity in the FM and Deep Component is
\begin{equation}
\begin{split}
 t_2 &= O(T^2H_0)+\sum_{i=1} O(H_iH_{i-1}) \\
 &= O(T^2H_0+\sum_{i=1} H_iH_{i-1})
 \end{split}
\end{equation}
The total time complexity for FGCNN model is $t_1+t_2 = O(T^2H_0+nTk^2+\sum_{i=1}^lnkf_ih_i+\sum_{i=1}H_iH_{i-1})$ which is dominated by the number of generated features, the number of neurons in the first hidden layer, embedding size and convolutional parameters.

